Kernel Dependence Network

We propose a greedy strategy to spectrally train a deep network for multi-class classification. Each layer is defined as a composition of linear weights with the feature map of a Gaussian kernel acting as the activation function. At each layer, the linear weights are learned by maximizing the dependence between the layer output and the labels using the Hilbert Schmidt Independence Criterion (HSIC). By constraining the solution space on the Stiefel Manifold, we demonstrate how our network construct (Kernel Dependence Network or KNet) can be solved spectrally while leveraging the eigenvalues to automatically find the width and the depth of the network. We theoretically guarantee the existence of a solution for the global optimum while providing insight into our network's ability to generalize.

==> appen2/ad_Hsequence.tex <==
\begin{appendices} 
\section{Proof for Theorem \ref{thm:hsequence}}
\label{app:thm:hsequence}

\textbf{Theorem \ref{thm:hsequence}: }
\textit{
For any $\hsic_0$, $L>1$ and $\delta>0$ there exists a sequence of kernel feature maps $\{\fm_l\}_{l=1}^L$ parameterized by $\{W_l\}_{l=1}^L$ and $\{\sigma_{l}\}_{l=1}^L$ such that:
}
\begin{enumerate}[label=\Roman*]
    \item )
    in finite $L$ we can get arbitrary close to convergence value where:
    \begin{equation}
        \label{app:eq:app:finite_conv}
        \hsic^{*} - \hsic_L \le \delta,
    \end{equation}
    \item )
    as $l \rightarrow \infty$, the sequence converges to the global optimal where
    \begin{equation}
        \label{app:eq:app:converge_to_global}
        \lim_{l \rightarrow \infty}  \hsic_l = \hsic^*,
    \end{equation}
    \item )
    The convergence is monotonic where
    \begin{equation}
    \label{app:eq:app:ineq}
    \hsic_{l} > \hsic_{l-1} \quad \forall l.
    \end{equation}
\end{enumerate}

\subsection{Proof for I}
\begin{lemma}
Given any $\hsic_0$, $\delta > 0$, and 2 layers, there exists a $\sigma_0 > 0 $ and $\sigma_1 > 0$ such that
\begin{equation}
        \hsic^{*} - \hsic_l \le \delta.
        \label{app:eq:proof_I}
\end{equation}
\end{lemma}

\begin{proof} $\hspace{1pt}$

\begin{adjustwidth}{0.5cm}{0.0cm}
\textbf{Assumptions. }
\begin{enumerate}
    \item 
        Without a loss of generality, we prove here for the binary case of 2 classes. The extension to 3 classes and beyond can be found at \citelemma{app:lemma:3class_lowerbound}.
    \item  
        We here assume to use only 2 layers, with $\sigma_0$ as the $\sigma$ for the 1st layer Gaussian kernel, and $\sigma_1$ is used for the 2nd layer. Since 2 layer is the minimum requirement, any finite number of layers is also satisfied.
\end{enumerate}
\end{adjustwidth}



\begin{adjustwidth}{0.5cm}{0.0cm}
\textbf{Observation 1. }

Note that the objective $\hsic$ is
\begin{equation}
    \hsic^* = 
    \max_W
    \sums \Gij \ISMexp - \sumsc |\Gij| \ISMexp.
\end{equation}
Since the Gaussian kernel is bounded between 0 and 1, the theoretical maximum of $\hsic^*$ is obviously when the kernel is 1 for $\cS$ and 0 for $\cS^c$ with the theoretical maximum as $\hsic^* = \sums \Gij$. Therefore \eq{app:eq:proof_I} inequality is equivalent to 
\begin{equation}
        \sums \Gij - \hsic_l \le \delta.
\end{equation}
\end{adjustwidth}


\begin{adjustwidth}{0.5cm}{0.0cm}
\textbf{Observation 2. }

According to \citelemma{lemma:Lbound_LHS}, there exists a lower bound for $\hsic_l$ that is a function of $\sigma_0$ and $\sigma_1$ denoted as $\lb\Lsigma$. Therefore, we have the following logic 
\begin{equation}
        \sums \Gij - \lb\Lsigma \le \delta \implies
        \sums \Gij - \hsic_l \le \delta.
\end{equation}
That is, proving $\sums \Gij - \lb\Lsigma \le \delta$ is sufficient to prove the lemma. Moreoever, \citelemma{lemma:Lbound_LHS} demonstrates the following properties for $\lb\Lsigma$:
\begin{enumerate}
    \item 
    As $\sigma_0 \rightarrow 0$, the lower bound approaches a specific function $\lb^*(\sigma_1)$
    \begin{equation}
        \lim_{\sigma_{0} \rightarrow 0}
        \lb\Lsigma = \lb^*(\sigma_1)  =  
        \sum_{i,j \in \cS} \Gij
        -
        \sum_{i,j \in \cS^c} |\Gij| 
        e^{-\frac{1}{2\sigma_{l}^2}}        
    \end{equation}    
    %\item
    %    $\lb\Lsigma$ is a decreasing function with respect to $\sigma_0$ and $\sigma_1$.    
    \item
    As $\sigma_1 \rightarrow 0$, $\lb^*(\sigma_1)$ approaches to $\hsic^*$
    \begin{equation}
        \lim_{\sigma_1 \rightarrow 0}
        \lb^*(\sigma_1) = \sums \Gij = \hsic^*.
    \end{equation}
\end{enumerate}
Therefore, by decreasing $\sigma_0$ and $\sigma_1$, we can reach arbitrarily close to the global optimal. 
\begin{equation}
    \sums \Gij - 
    \lim_{\sigma_0 \rightarrow 0} 
    \lim_{\sigma_1 \rightarrow 0}
    \lb\Lsigma = \sums \Gij - \sums \Gij = 0.
\end{equation}
\end{adjustwidth}


\begin{adjustwidth}{0.5cm}{0.0cm}
\textbf{Observation 3. }

If we choose a $\sigma_0$ such that 
\begin{equation}
    \lb^*(\sigma_1) - \lb\Lsigma \le \frac{\delta}{2}
    \quad \text{and} \quad
    \hsic^* - \lb^*(\sigma_1) \le \frac{\delta}{2}
\end{equation}
then we have identified the condition where $\sigma_0 > 0$ and $\sigma_1 > 0$ such that
\begin{equation}
    \sums \Gij - \lb\Lsigma \le \delta.
\end{equation}
\end{adjustwidth}

\end{proof}

\begin{adjustwidth}{0.5cm}{0.0cm}
\textbf{Note. }

Although this proof has shown that it's theoretically possible to reach the global optimal with 2 layers, the $\sigma_0$ and $\sigma_1$ required to accomplish this task might be very small. This causes the Gaussian kernel to be a shap mapping. Instead, of trying to jump to the global optimal $\hsic^*$ with 2 layers, by using more layers, each layer can simply aim for monotonic improvement using a larger $\sigma_0$ and $\sigma_1$, thereby resulting in a sequence of smooth layers.
\end{adjustwidth}
$\newline$

\subsection{Proof for II}

\begin{adjustwidth}{0.0cm}{0.0cm}
\begin{lemma}
    There exists a sequence of kernel feature maps $\{\fm_l\}_{l=1}^L$ parameterized by $\{W_l\}_{l=1}^L$ and $\{\sigma_{l}\}_{l=1}^L$ such that
    \begin{equation}
        \lim_{l \rightarrow \infty}  \hsic_l = \hsic^*.
    \end{equation}
\end{lemma}
\end{adjustwidth}

Before, the proof, we use the following figure to illustrate the relationship between \KS $\{\phi_{l^\circ}\}_{l=1}^L$ that generates the \RS $\{\hsic_l\}_{l=1}^L$. By solving a network greedily, we separate the network into $L$ separable problems. At each additional layer, we rely on the weights learned from the previous layer. At each network, we find $\sigma_{l-1}$, $\sigma_l$, and $W_l$ for the additional network.
        \begin{figure}[h]
        \center
            \includegraphics[width=7cm]{img/kchain_layers.png}
            \caption{Relating \KS to \RS.}
            \label{app:fig:all_layers}
        \end{figure} 
        
\begin{proof} $\hspace{1pt}$
\begin{adjustwidth}{0.5cm}{0.0cm}
We first note that from the proof in I, we have previously proven that given 2 layers and any $\delta > 0$, we can achieve
\begin{equation}
    \hsic^{*} - \hsic_{l} \leq \delta.
\end{equation}
This implies that based on Fig.~\ref{app:fig:all_layers}, at any given layer, we could reach arbitrarily close to $\hsic^*$. Therefore, if we construct a Kernel sequence $\{\hsic_{l}\}_{l=1}^\infty$, where $\delta_{l} = \frac{\hsic^* - \hsic_0}{l}$ such that 
\begin{equation}
    \forall l>0: \hsic^{*} - \hsic_{l} \leq \delta_{l}
\end{equation}
then this construction is sufficient to show that 
\begin{equation}
   \lim_{l \rightarrow \infty}  \hsic_l = \hsic^*
\end{equation}

 because as $l \rightarrow \infty$, we have the condition
 \begin{equation}
     \hsic^* - \hsic_l \le 0.
 \end{equation}
\end{adjustwidth}
\end{proof}

\subsection{Proof for III}
\begin{lemma}
    There exists a $\sigma_{l-1}$ and $\sigma_l$ such that convergence is monotonic where
    \begin{equation}
    \hsic_{l} > \hsic_{l-1} \quad \forall l.
    \end{equation}
\end{lemma}
\begin{proof}
 Given the proof from II, each layer we have
\begin{equation}
    \hsic^* - \hsic_l \le \frac{\hsic^* - \hsic_0}{l}.     
\end{equation} 
Since $\frac{\hsic^* - \hsic_0}{l}$ decreases as $l$ increase, then at each layer, we have the condition
\begin{equation}
    \hsic_{l+1} > \hsic_l.
\end{equation}

\end{proof}

\subsection{Proof the existence of Lower bound $\lb\Lsigma$}
\begin{lemma} \label{lemma:Lbound_LHS}
There exists a lower bound $\lb\Lsigma$ for $\hsic_l$ that is a function of $\sigma_{0}$ and $\sigma_1$ such that 
\begin{enumerate}
    \item
    As $\sigma_0 \rightarrow 0$, $\lb\Lsigma$ approaches to a specific function where
    \begin{equation}
        \lim_{\sigma_{0} \rightarrow 0}
        \lb\Lsigma = \lb^*(\sigma_1)  =  
        \sum_{i,j \in \cS} \Gij
        -
        \sum_{i,j \in \cS^c} |\Gij| 
        e^{-\frac{1}{2\sigma_{l}^2}}        
    \end{equation}
    %\item  
    %    $\lb\Lsigma$ is a decreasing function with respect to $\sigma_0$ and $\sigma_1$.   
    \item
        As $\sigma_1 \rightarrow 0$, $\lb\Lsigma$ approaches to the global optimal $\hsic^*$ where
        \begin{equation}
            \lim_{\sigma_1} \lb^*(\sigma_1) = \sums \Gij
            = \hsic^*.
        \end{equation}
\end{enumerate}
\end{lemma}

\begin{adjustwidth}{0.5cm}{0.0cm}
\textbf{Notations and Assumtions. }
\begin{enumerate}
    \item
        Assume that no two samples $i \ne j$ overlap each other.
    \item 
        Without a loss of generality, we prove here for the binary case of 2 classes. The logical extension can be found at \citelemma{app:lemma:3class_lowerbound}.
    \item
        To simplify the notation, here, we denote $W_l$ simply as $W$.
    \item  
        Given the figure below, assume that we are using only 2 layers since this is the minimally sufficient amount of layers. The input of the data is $X$ with each sample as $x_i$, and the output of the 1st layer are denoted as $r_i$ as samples from $\cS^1$ and $t_i$ as samples from $\cS^2$. $\psi_{\sigma_0}$ is the feature map of the 1st \rbfk using $\sigma_0$ and $\psi_{\sigma_1}$ corresponds to the 2nd layer. 
        \begin{figure}[h]
        \center
            \includegraphics[width=7cm]{img/TwoLayer.png}
            \caption{Figure of a 2 layer network.}
            \label{app:fig:two_layer_f}
        \end{figure} 
        
\end{enumerate}
\end{adjustwidth}


\begin{proof} $\hspace{1pt}$

\begin{adjustwidth}{0.5cm}{0.0cm}
Given Fig.~\ref{app:fig:two_layer_f}, the equation for $\hsic_0$ is 
\begin{align}
    \hsic_0 
        & = \sums \Gij 
        e^{-\frac{(x_i - x_j)^TW W^T (x_i - x_j)}{2 \sigma_0^2}}
        -
        \sumsc |\Gij| 
        e^{-\frac{(x_i - x_j)^TW W^T (x_i - x_j)}{2 \sigma_0^2}}    \\
        & = 
        \sums \Gij
            \langle 
                \psi_{\sigma_0}(x_i), 
                \psi_{\sigma_0}(x_j)
            \rangle
            \sumsc |\Gij|
            \langle 
                \psi_{\sigma_0}(x_i), 
                \psi_{\sigma_0}(x_j)
            \rangle
\end{align}
Notice that as $\sigma_0 \rightarrow 0$, we have the condition
\begin{equation}
    %\label{eq:converged_kernel}
    \lim_{\sigma_0 \rightarrow 0} 
    \langle 
        \psi_{\sigma_0}(x_i), 
        \psi_{\sigma_0}(x_j)
    \rangle   
    =  
    \begin{cases} 
    0 \quad \forall i \ne j
    \\
    1 \quad \forall i = j
    \end{cases}.
\end{equation}
In other words, as $\sigma_0 \rightarrow 0$, the samples $r_i$ and $t_i$ in the RKHS of a Gaussian kernel approaches orthogonal to all other samples. Given this observation, it also implies that the $\sigma_0$ controls the size of the maximum sample pair $x_i^*, x_j^*$ defined as 
\begin{equation}
    \langle 
        \psi_{\sigma_0}(x_i^*), 
        \psi_{\sigma_0}(x_j^*)
    \rangle  
    \ge 
     \langle 
        \psi_{\sigma_0}(x_i), 
        \psi_{\sigma_0}(x_j)
    \rangle      
    \quad
    \forall i,j \ne i^*, j^*,
\end{equation}
or equivalently
\begin{equation}
    \langle 
        r_i^*, 
        r_j^*
    \rangle  
    \ge 
     \langle 
        r_i,
        r_j
    \rangle      
    \quad
    \forall i,j \ne i^*, j^*.
\end{equation}

Therefore, given a $\sigma_0$, it controls the upper bound of the inner product. We denote this upper bound as $\ub = \langle r_i^*, r_j^* \rangle$ with the relationship
\begin{equation}
    \lim_{\sigma_0 \rightarrow 0} 
    \ub = 0.
\end{equation}
Having defined these notations, we can now write the equation for $\hsic_1$ as 
\begin{align}
    \hsic_1 & = 
    \max_W
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW W^T(r_i-r_j)}{2\sigma_{1}^2}}
    }_\text{1st term}
     +
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^2} \Gij 
    e^{-\frac{(t_i-t_j)^TW W^T(t_i-t_j)}{2\sigma_{1}^2}}
    }_\text{2st term}   \\
    & -
    \underbrace{
    \sum_{i,j \in \mathcal{S}^c} |\Gij| 
    e^{-\frac{(r_i-t_j)^TW W^T(r_i-t_j)}{2\sigma_{1}^2}} 
    }_\text{3rd term}. 
\end{align}
Our goal is to identify a lower bound for $\hsic_1$. First, instead of using an optimal $W^*$, we let $W$ be a suboptimal solution where $W_s = \sum_i r_i$. We claim that $W_s$ is suboptimal because \citelemma{app:lemma:W_not_optimal} showed that $\partial \hsic/\partial W_s \ne 0$.  Althought $W_s$ is suboptimal, it simplifies the proof and bypasses the maximization process. This also produces a smaller $\hsic_s$ where $\hsic_s \le \hsic_1$ which is helpful in identifying a lower bound. Next, we use $W_s$ and multiply each term out to obtain the lowest possible value. We can find the lowest bound by finding the upper and lower bound of the exponent for terms 1, 2 and 3. Specifically, we need to
\begin{enumerate}
    \item find the upper bound of 
    $(r_i-r_j)^TW_l W_l^T(r_i-r_j)$ for 1st term.
    \item find the upper bound of 
    $(t_i-t_j)^TW_l W_l^T(t_i-t_j)$ for 2nd term.   
    \item find the lower bound of 
    $(r_i-t_j)^TW_l W_l^T(r_i-t_j)$ for 3rd term.
\end{enumerate}

Note that any $\langle r_i, r_j \rangle$ is upper and lower bounded by $\ub$ and 0. We can use this to derived the lower bound.

\textbf{1st Term lower bound. } If we look at each term carefully, we have
\begin{equation}
      r_{i}^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^T r_{i}
      + r_{j}^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^Tr_{j} - r_{i}^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^Tr_{j} -r_{j}^T (\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^Tr_{i}.
\end{equation}
By using $\ub$ as its upper bound and 0 as the lower bound of $r_i^Tr_j$, we have
\begin{align}
 (r_{i}^T r_{i} + (n-1)\ub)^2 &+ (r_{j}^T r_{j} + (n-1)\ub)^2 & - (r_{i}^T r_{i})^2   & -r_{j}^T r_{j} r_{j}^T r_{j}   \\ 
 (1 + (n-1)\ub)^2 &+ (1 + (n-1)\ub)^2 & -1  & -1 
\end{align}
\begin{equation}
    2(1+(n-1)\ub)^2 - 2
\end{equation}
Therefore, the 1st term is lower bounded by 
\begin{equation}
      \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW W^T(r_i-r_j)}{2\sigma_1^2}} \geq 
    \sum_{i,j \in \cS^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\ub)^2 - 2 }{2\sigma_1^2}}.
\end{equation}
\textbf{2st Term lower bound. }
We next try to maximize the exponent of the 2nd term. Again, by using $\ub$ and 0 as its upper and lower bound of $r_i^Tr_j$, we have
\begin{align}
      t_{i}^T(\sum_{i\in \cS^1}r_{i}) (\sum_{i\in \cS^1}r_{i})^T t_{i}
      &
      + t_{j}^T(\sum_{i\in \cS^1}r_{i}) (\sum_{i\in \cS^1}r_{i})^Tt_{j} 
      & - t_{i}^T(\sum_{i\in \cS^1}r_{i}) (\sum_{i\in \cS^1}r_{i})^Tt_{j} 
      &
      - t_{j}^T (\sum_{i\in \cS^1}r_{i}) (\sum_{i\in \cS^1}r_{i})^Tt_{i} \\
      (n\ub)^2 
      &
      + (n\ub)^2 
      & - 0 & - 0.
\end{align}
Which yields a bound of
\begin{align}
 2(n\ub)^2.
\end{align}
Therefore, the 2nd term is lower bounded by 
\begin{equation}
     \sum_{i,j \in \cS^2} \Gamma_{i,j} 
    e^{-\frac{(t_i-t_j)^TW W^T(t_i-t_j)}{2\sigma_1^2}} \geq 
    \sum_{i,j \in \cS^2} \Gamma_{i,j} 
    e^{-\frac{2(n\ub)^2 }{2\sigma_1^2}}.
\end{equation}

\end{adjustwidth}



\begin{adjustwidth}{0.5cm}{0.0cm}
\textbf{3rd Term lower bound. }
We again repeat the same process for the 3rd term. Note that here, instead of trying to maximize the exponent, we need to minimize them.
\begin{equation}
    (r_i-t_j)^T(\sum_{i\in \cS^1}r_{i}) (\sum_{i\in \cS^1}r_{i})^T(r_i-t_j)
\end{equation}
\end{adjustwidth}

\begin{align}
      &r_{i}^T(\sum_{i\in \cS^1}r_{i}) (\sum_{i\in \cS^1}r_{i})^T r_{i}
      + t_{j}^T(\sum_{i\in \cS^1}r_{i}) (\sum_{i\in \cS^1}r_{i})^Tt_{j} - r_{i}^T(\sum_{i\in \cS^1}r_{i}) (\sum_{i\in \cS^1}r_{i})^Tt_{j} -t_{j}^T (\sum_{i\in \cS^1}r_{i}) (\sum_{i\in \cS^1}r_{i})^Tr_{i}\\
      &(1)^2
      + 0 
      - n\ub(1+(n-1)\ub)
      - n\ub(1+(n-1)\ub)\\
      &1 - 2n\ub(1+(n-1)\ub)
\end{align}

\begin{adjustwidth}{0.5cm}{0.0cm}
Therefore, the 3rd term is also lower bounded such that 
\begin{equation}
   -\sum_{i,j \in \cS^c} |\Gij| 
   e^{-\frac{(r_i-t_j)^TW W^T(r_i-t_j)}{2\sigma_{1}^2}} 
   \leq 
   - \sum_{i,j \in \cS^c} |\Gij| 
   e^{-\frac{1 - 2n\ub(1+(n-1)\ub))}{2\sigma_{1}^2}}.
\end{equation}

\textbf{Complete lower bound. } Give the lower bound of all 3 terms, we have a joint lower bound for $\lb\Lsigma$. \blue{Here, we have proven the existence of a lower bound. }

\end{adjustwidth}

\begin{equation}
    \lb\Lsigma = 
    \sum_{i,j \in \cS^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\ub)^2 - 2 }{2\sigma_1^2}}
    + 
    \sum_{i,j \in \cS^1} \Gamma_{i,j} 
    e^{-\frac{2(n\ub)^2 }{2\sigma_1^2}}    
    -
   \sum_{i,j \in \cS^c} |\Gij| 
   e^{-\frac{1 - 2n\ub(1+(n-1)\ub))}{2\sigma_{1}^2}}. 
\end{equation}


\begin{adjustwidth}{0.5cm}{0.0cm}
From this equation, we see that a lower bound $\lb\Lsigma$ as a function of $\sigma_{0}$ exists. Additionally, note that
\begin{equation}
    \lim_{\sigma_{0} \rightarrow 0} 
    \ub = 0.
\end{equation}
and therefore
 \begin{align}
    \lim_{\sigma_{0} \rightarrow 0}
    \lb\Lsigma = \lb^*(\sigma_1) & =  
    \sum_{i,j \in \cS^1} \Gij
    + 
    \sum_{i,j \in \cS^2} \Gij
    -
   \sum_{i,j \in \cS^c} |\Gij| 
   e^{-\frac{1}{2\sigma_{1}^2}} \\
   & = 
   \sum_{i,j \in \cS} \Gij
    -
   \sum_{i,j \in \cS^c} |\Gij| 
   e^{-\frac{1}{2\sigma_{1}^2}} 
\end{align}
    \blue{Here, we have proven condition 1, i.e., the limit of $\lb\Lsigma$ as $\sigma_0 \rightarrow 0$.}
   Given this lower bound, $\lb(\ub)$ is a decreasing function with respect to $\ub$ This can be seen easily by taking the derivative with respect to $\ub$ and showing that the derivative is always < 0. 
\end{adjustwidth}

\begin{equation}
    L(\ub) = 
    \sum_{i,j \in \cS^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\ub)^2 - 2 }{2\sigma_1^2}}
    + 
    \sum_{i,j \in \cS^2} \Gamma_{i,j} 
    e^{-\frac{2(n\ub)^2 }{2\sigma_1^2}}    
    -
   \sum_{i,j \in \cS^c} |\Gij| 
   e^{-\frac{1 - 2n\ub(1+(n-1)\ub))}{2\sigma_{1}^2}}. 
\end{equation}  

\begin{adjustwidth}{0.5cm}{0.0cm}
Taking derivative for each term with respect to $\ub$ we obtain the following:
\end{adjustwidth}

\begin{equation}
    \frac{\partial}{\partial \ub}
    \sum_{i,j \in \cS^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\ub)^2 - 2 }{2\sigma_1^2}} 
    = 
    \sum_{i,j \in \cS^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\cS)^2 - 2 }{2\sigma_1^2}}   
    \left[
    - \frac{2(1+(n-1)\cS)(n-1)}{\sigma_1^2}
    \right] 
    \le 0 
\end{equation} 

\begin{equation}    
    \frac{\partial}{\partial \ub}
    \sum_{i,j \in \cS^2} \Gamma_{i,j} 
    e^{-\frac{2(n\ub)^2 }{2\sigma_1^2}}    
    = 
    \sum_{i,j \in \cS^2} \Gamma_{i,j} 
    e^{-\frac{2(n\ub)^2 }{2\sigma_1^2}}       
    \left[
    -\frac{(n\ub)^2}{\sigma_1^2}
    \right]
    \le 0 
\end{equation}
\begin{equation}
   \frac{\partial}{\partial \ub}
   -\sum_{i,j \in \cS^c} |\Gij| 
   e^{-\frac{1 - 2n\ub(1+(n-1)\ub))}{2\sigma_{1}^2}}
   = 
   -\sum_{i,j \in \cS^c} |\Gij| 
   e^{-\frac{1 - 2n\ub(1+(n-1)\ub))}{2\sigma_{1}^2}}
   \le 0.
\end{equation}

\begin{adjustwidth}{0.5cm}{0.0cm}
It can be seen that all 3 terms are negative. This implies that as $\ub$ increases, $\lb(\ub)$ is a decreasing function. Conversely, as $\ub \rightarrow 0$,  $\lb(\ub)$ is an increasing $\uparrow$ function. This implies the following set of logics
\begin{align}
    \sigma_0 \uparrow & \implies \ub \uparrow \\
    \sigma_0 \downarrow & \implies \ub \downarrow \\
    \sigma_0 \downarrow \implies \ub \downarrow & \implies \lb\Lsigma \uparrow
\end{align}
Here, we have proven that $\lb\Lsigma$ is an decreasing function with respect to $\sigma_0$.
Conversely, as $\sigma_0$ decrease, $\lb\Lsigma$ increases. 
Also, looking at $\lb^*(\sigma_1)$ we have 
\begin{equation}
    \lb^*(\sigma_1) = 
    \sum_{i,j \in \cS} \Gij
    -
   \sum_{i,j \in \cS^c} |\Gij| 
   e^{-\frac{1}{2\sigma_{1}^2}} 
\end{equation}

It is obvious that $\lb^*(\sigma_1)$ is an increasing function as $\sigma_1$ decreases. In fact, as $\sigma_1 \rightarrow 0$, $\lb^*(\sigma_1)$ approaches $\hsic^* = \sums \Gij$. \blue{From this logic the 2nd condition is also proven}.
\end{adjustwidth}

\end{proof}





\end{appendices} 

==> appen2/ae_3_class_extension.tex <==
\subsection{Extending Inequality Proof to 3 Classes}
\begin{lemma} \label{app:lemma:3class_lowerbound}
There exists a lower bound $\lb\Lsigma$ for $\hsic_l$ that is a function of $\sigma_{0}$ and $\sigma_1$ such that 
\begin{enumerate}
    \item
    As $\sigma_0 \rightarrow 0$, $\lb\Lsigma$ approaches to a specific function where
    \begin{align}
    \lim_{\sigma_{0} \rightarrow 0}
    \lb\Lsigma = \lb^*(\sigma_1) 
    & =
    \underbrace{ 
    \sums \Gij 
    }_\text{1st, 2nd, 3rd terms}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    e^{-\frac{2}{2\sigma_{1}^2}} 
    }_\text{4th term}
    \\
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{1}^2}} 
    }_\text{5th term}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{1}^2}} 
    }_\text{6th term}.        
    \end{align}
    %\item  
    %    $\lb\Lsigma$ is a decreasing function with respect to $\sigma_0$ and $\sigma_1$.   
    \item
        As $\sigma_1 \rightarrow 0$, $\lb^*(\sigma_1)$ approaches to the global optimal $\hsic^*$ where
        \begin{equation}
            \lim_{\sigma_1 \rightarrow 0} \lb^*(\sigma_1) = \sums \Gij
            = \hsic^*.
        \end{equation}
\end{enumerate}
\end{lemma}



\textbf{Notations and Assumptions of the Proof. }
\begin{enumerate}
  \item We assume to only have 3 classes where the set of sample pairs from the 1st, 2nd and 3rd classes are denoted as $\mathcal{S}^1$, $\mathcal{S}^2$ and $\mathcal{S}^3$. Given the extension to 3 classes, a similar proof can be used for 4 classes and beyond.
  \item To emphasize  the different classes, we denote samples from different classes as
  $r_i \in \cS^1$,  $t_i \in \cS^2$,  $q_i \in \cS^3$
  \item To simplify the notation, we let $W = W_l$ in the proof.
  \item We let $\sigma_{0}$ and $\sigma_1$ be the $\sigma$ values used for the previous and current layer respectively.
  \item For 3 classes we need to use the mean direction of 2 classes. In general, for $c$ classes, we need to use the mean direction for $c-1$ classes.
  \begin{equation}
        \label{app:eq:multiple_class_W}
        W = \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right].
  \end{equation}
  Note that since we are looking for the lower bound, using a suboptimal $W_s$, is guaranteed to have a equal or lower value. 
\end{enumerate}

\textbf{Proof of the 3 class extension Lemma}
The strategy of proving 3 class is identical to the 2 class. However, instead of deriving the lower bound equation, we can assume its existence from 2 class prove and derive directly $\lb^*(\sigma_1)$ function. Everything, we did for the 2 class regarding to $\ub$ is still valid here. For this proof, we want to first show that as $\sigma_{0} \rightarrow 0$, we have 
\begin{align}
   \lim_{\sigma_{0} \rightarrow 0} 
   \lb\Lsigma = &
    \underbrace{ 
    \sums \Gij 
    }_\text{1st, 2nd, 3rd terms}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    e^{-\frac{2}{2\sigma_{1}^2}} 
    }_\text{4th term}
    \\
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{1}^2}} 
    }_\text{5th term}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{1}^2}} 
    }_\text{6th term}.       
\end{align}

\begin{proof}
To find the limit of the lower bound, we let $\sigma_{0} = 0$ and input $W$ from \eq{app:eq:multiple_class_W} into the following equation
\begin{align}
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW W^T(r_i-r_j)}{2\sigma_{1}^2}}
    }_\text{1st term}
    & +
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^2} \Gij 
    e^{-\frac{(t_i-t_j)^TW W^T(t_i-t_j)}{2\sigma_{1}^2}}
    }_\text{2nd term} 
    \\
    +
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^3} \Gamma_{i,j} 
    e^{-\frac{(q_i-q_j)^TW W^T(q_i-q_j)}{2\sigma_{1}^2}}
    }_\text{3rd term} 
    & - 
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    e^{-\frac{(r_i-t_j)^TW W^T(r_i-t_j)}{2\sigma_{1}^2}} 
    }_\text{4th term}
    \\
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{(r_i-q_j)^TW W^T(r_i-q_j)}{2\sigma_{1}^2}} 
    }_\text{5th term}
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{(t_i-q_j)^TW W^T(t_i-q_j)}{2\sigma_{1}^2}} 
    }_\text{6th term}. 
    \label{ineq:exist_lower_bound_3_classes}
\end{align}


\textbf{1st Term. } If we look at the exponent of the 1st term carefully, we have
\begin{align}
    (r_i-r_j)^TW W^T(r_i-r_j)\\
    (r_i-r_j)^T
    \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right] 
        \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right]^T   
        (r_i-r_j) \\
        \left[
        \begin{bmatrix}
        1 & 0
        \end{bmatrix} - 
        \begin{bmatrix}
        1 & 0
        \end{bmatrix}       
        \right]
         \left[
        \begin{bmatrix}
        1 \\ 0
        \end{bmatrix} - 
        \begin{bmatrix}
        1 \\ 0
        \end{bmatrix}       
        \right] = 0
\end{align}

\textbf{2nd Term. } If we look at the exponent of the 2nd term carefully, we have
\begin{align}
    (t_i-t_j)^TW W^T(t_i-t_j)\\
    (t_i-t_j)^T
    \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right] 
        \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right]^T   
        (t_i-t_j) \\
        \left[
        \begin{bmatrix}
        0 & 1
        \end{bmatrix} - 
        \begin{bmatrix}
        0 & 1
        \end{bmatrix}       
        \right]
         \left[
        \begin{bmatrix}
        0 \\ 1
        \end{bmatrix} - 
        \begin{bmatrix}
        0 \\ 1
        \end{bmatrix}       
        \right] = 0
\end{align}

\textbf{3rd Term. } If we look at the exponent of the 3rd term carefully, we have
\begin{align}
    (q_i-q_j)^TW W^T(q_i-q_j)\\
    (q_i-q_j)^T
    \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right] 
        \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right]^T   
        (q_i-q_j) \\
        \left[
        \begin{bmatrix}
        0 & 0
        \end{bmatrix} - 
        \begin{bmatrix}
        0 & 0
        \end{bmatrix}       
        \right]
         \left[
        \begin{bmatrix}
        0 \\ 0
        \end{bmatrix} - 
        \begin{bmatrix}
        0 \\ 0
        \end{bmatrix}       
        \right] = 0
\end{align}

\textbf{4th Term. } If we look at the exponent of the 4th term carefully, we have
\begin{align}
    (r_i-t_j)^TW W^T(r_i-t_j)\\
    (r_i-t_j)^T
    \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right] 
        \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right]^T   
        (r_i-t_j) \\
        \left[
        \begin{bmatrix}
        1 & 0
        \end{bmatrix} - 
        \begin{bmatrix}
        0 & 1
        \end{bmatrix}       
        \right]
         \left[
        \begin{bmatrix}
        1 \\ 0
        \end{bmatrix} - 
        \begin{bmatrix}
        0 \\ 1
        \end{bmatrix}       
        \right] = 2
\end{align}

\textbf{5th Term. } If we look at the exponent of the 5th term carefully, we have
\begin{align}
    (r_i-q_j)^TW W^T(r_i-q_j)\\
    (r_i-q_j)^T
    \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right] 
        \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right]^T   
        (r_i-q_j) \\
        \left[
        \begin{bmatrix}
        1 & 0
        \end{bmatrix} - 
        \begin{bmatrix}
        0 & 0
        \end{bmatrix}       
        \right]
         \left[
        \begin{bmatrix}
        1 \\ 0
        \end{bmatrix} - 
        \begin{bmatrix}
        0 \\ 0
        \end{bmatrix}       
        \right] = 1
\end{align}

\textbf{6th Term. } If we look at the exponent of the 6th term carefully, we have
\begin{align}
    (t_i-q_j)^TW W^T(t_i-q_j)\\
    (t_i-q_j)^T
    \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right] 
        \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right]^T   
        (t_i-q_j) \\
        \left[
        \begin{bmatrix}
        0 & 1
        \end{bmatrix} - 
        \begin{bmatrix}
        0 & 0
        \end{bmatrix}       
        \right]
         \left[
        \begin{bmatrix}
        0 \\ 1
        \end{bmatrix} - 
        \begin{bmatrix}
        0 \\ 0
        \end{bmatrix}       
        \right] = 1
\end{align}

We next put all 6 terms together
\begin{align}
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^1} \Gij 
    }_\text{1st term}
    +
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^2} \Gij 
    }_\text{2nd term} 
    +
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    }_\text{3rd term} 
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    e^{-\frac{2}{2\sigma_{1}^2}} 
    }_\text{4th term}
    \\
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{1}^2}} 
    }_\text{5th term}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{1}^2}} 
    }_\text{6th term} \\
    \lim_{\sigma_{0} \rightarrow 0}
    \lb\Lsigma 
    = \lb^*(\sigma_1) & = 
    \underbrace{ 
    \sums \Gij 
    }_\text{1st, 2nd, 3rd terms}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    e^{-\frac{2}{2\sigma_{1}^2}} 
    }_\text{4th term}
    \\
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{1}^2}} 
    }_\text{5th term}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{1}^2}} 
    }_\text{6th term}.    
\end{align}
\blue{Here, we have proven Condition 1 of the lemma.} Next, the 2nd condition also reveals itself as we decrease $\sigma_1$. At its limit we that
\begin{equation}
    \lim_{\sigma_1 \rightarrow 0}
    \lb^*(\sigma_1) = \hsic^* = \sums \Gij.
\end{equation}
\end{proof}




==> appen2/af_geometric_proof.tex <==
\begin{appendices} 
\section{Proof for Theorem \ref{thm:geometric_interpret}}
\label{app:thm:geometric_interpret}

\textbf{Theorem \ref{thm:geometric_interpret}: }
\textit{
As $l \rightarrow \infty$ and  $\hsic_l \rightarrow \hsic^*$, 
the following properties are satisfied: }

\begin{enumerate}[label=\Roman*]
    \item 
    %Given $S_{w}^{l}, S^{l}_{b}$ to be the scatter matrices of transformed data through the sequences of kernels of first $l$ layer in IDS, then:
    the scatter ratio approaches 0 where
    \begin{equation}
    \lim_{l \rightarrow \infty} \frac{\Tr(S_w^{l})}{\Tr(S_b^{l})} =   0
\end{equation}

\item the \KS converges to the following kernel:
\begin{equation}
    %\lim_{l \rightarrow \infty} 
    %\hsic_l = \hsic^* \implies 
    \lim_{l \rightarrow \infty} 
    \kf(x_{i},x_{j})^{l} = 
    \kf^* =  
    \begin{cases} 
    0 \quad \forall i,j \in \mathcal{S}^c
    \\
    1 \quad \forall i,j \in \mathcal{S}
    \end{cases}.
\end{equation}
\end{enumerate}

\begin{proof}













We start by proving condition II starting from the $\hsic$ objective using a \rbfk
\begin{align}
    \max_{W} 
    \sums \Gij \kf_W(r_i, r_j) 
    -
    \sumsc |\Gij| \kf_W(r_i, r_j)\\
    \max_{W} 
    \sums \Gij  \ISMexp
    -
    \sumsc |\Gij| \ISMexp   
\end{align}
Given that $\hsic_l \rightarrow \hsic^*$,
and the fact that $0 \leq \kf_W \leq 1$,
this implies that the following condition must be true:
\begin{equation}
   \hsic^{*} = \sums \Gij =  
    \sums \Gij (1) 
    -
    \sumsc |\Gij| (0).
\end{equation}

Based on \eq{eq:cond1}, our construction at each layer ensures to satisfy 
\begin{equation}
    \hsic^{*} - \hsic_{l} \leq \delta_{l}.
\end{equation}
Substituting the definition of $\hsic^*$ and $\hsic_l$, we have
\begin{align}
    \sums \Gij (1) 
    -\left[\sums \Gij  \kf_W(r_i, r_j) 
    -
    \sumsc |\Gij| \kf_W(r_i, r_j) \right] \leq \delta_{l}
    \\
     \sums \Gij  (1-\kf_W(r_i, r_j)) 
    +
    \sumsc |\Gij| \kf_W(r_i, r_j)  \leq \delta_{l}.
    \label{eq:kernel_inequal}
\end{align}
Since every term within the summation in \eq{eq:kernel_inequal} is positive, this implies
\begin{align}\label{eq:limit kernal behaviour}
     1-\kf_W(r_i, r_j) \leq \delta_{l} \quad i,j \in \mathcal{S}
     \\
     \kf_W(r_i, r_j) \leq \delta_{l}\quad  i,j \in \mathcal{S}^{c}.
     \label{eq:limit kernal behaviour2}
\end{align}

So as $l \rightarrow \infty$ and  $\delta_{l} \rightarrow 0$, every component getting closer to limit Kernel, i.e, taking the limit from both sides and using the fact that is proven is theorem 1 $\lim_{l\rightarrow \infty} \delta_{l} = 0$ leads to
\begin{align}
   \lim_{l\rightarrow \infty}  1 \leq \kf_W(r_i, r_j)  \quad i,j \in \mathcal{S}
     \\
     \lim_{l\rightarrow \infty}\kf_W(r_i, r_j) \leq 0 \quad  i,j \in \mathcal{S}^{c}
\end{align}
%Since $\kf$ is a Gaussian kernel, it is impossible for 
%\begin{align}
%   \lim_{l\rightarrow \infty}  1 < \kf_W(r_i, r_j)  \quad i,j \in \mathcal{S}
%     \\
%     \lim_{l\rightarrow \infty}\kf_W(r_i, r_j) < 0 \quad  i,j \in \mathcal{S}^{c},
%\end{align}
both terms must instead be strictly equality. Therefore, we see that at the limit point $\kf_W$ would have the form 
\begin{equation}
     \kf^* =  
    \begin{cases} 
    0 \quad \forall i,j \in \mathcal{S}^c
    \\
    1 \quad \forall i,j \in \mathcal{S}
    \end{cases}.   
\end{equation}

\textbf{First Property}:

Using \eq{eq:limit kernal behaviour} and \eq{eq:limit kernal behaviour2} we have:

\begin{align}
         1-\delta_{l}\leq  \ISMexp  \quad i,j \in \mathcal{S}
     \\
     \ISMexp \leq \delta_{l}\quad  i,j \in \mathcal{S}^{c}.
\end{align}

As  $\lim_{l\rightarrow \infty} \delta_{l} = 0$, taking the limit from both side leads to:


% \begin{align}
%          \ln\frac{1}{1-\delta_{l}} \geq   (r_i - r_j)^T W W^T(r_i - r_j)  \quad i,j \in \mathcal{S}
%      \\
%       (r_i - r_j)^T W W^T(r_i - r_j) \geq \ln{\frac{1}{\delta_{l}}}\quad  i,j \in \mathcal{S}^{c}
% \end{align}



 
\begin{equation}
    \begin{cases} 
    \ISMexp = 1 \quad \forall i,j \in \mathcal{S}\\
    \ISMexp = 0 \quad \forall i,j \in \mathcal{S}^c
    \end{cases}.   
\end{equation}
If we take the log of the conditions, we get
\begin{equation}
    \begin{cases} 
     \frac{1}{2\sigma^2}
    (r_i - r_j)^T W W^T(r_i - r_j) =0 
    \quad \forall i,j \in \mathcal{S}\\   
    \frac{1}{2\sigma^2}
    (r_i - r_j)^T W W^T(r_i - r_j) = \infty
    \quad \forall i,j \in \mathcal{S}^c
    \end{cases}.   
\end{equation}
This implies that as $l \rightarrow \infty$ we have
\begin{equation}
    \lim_{l \rightarrow \infty}
    \sums
    \frac{1}{2\sigma^2}
    (r_i - r_j)^T W W^T(r_i - r_j) 
    = 
    \lim_{l \rightarrow \infty}
    \Tr(S_w) = 0.
\end{equation}
\begin{equation}
    \lim_{l \rightarrow \infty}
    \sumsc \frac{1}{2\sigma^2}
    (r_i - r_j)^T W W^T(r_i - r_j) 
    = 
    \lim_{l \rightarrow \infty}
    \Tr(S_b)
    =
    \infty,
\end{equation}
This yields the ratio
\begin{equation}
    \lim_{\hsic_l \rightarrow \hsic^*} \frac{\Tr(S_w)}{\Tr(S_b)} = \frac{0}{\infty} = 0.
\end{equation}

\end{proof}

% \blue{This proof is shallow}

% Using the construction from Theorem 1, we defined $W_s = \frac{1}{\sqrt{\zeta}} \sum_{\alpha} r_{\alpha}$, using this we can compute an upper bound for $\Tr(S_w^{l})$ and a lower bound for 
% $\Tr(S_b^{l})$, hence an upper bound for $\frac{\Tr(S_w^{l})}{\Tr(S_b^{l})}$ and then we'll show this upper bound approaches 





\end{appendices}

==> appen2/ag_general_lowerbound.tex <==
\begin{appendices} 
\section{Derivation for the Lower Bound of $\hsic$}
\label{app:general_lowerbound}

\textbf{Assumptions and Notations. }
\begin{enumerate}
    \item  Here we show that this bound can be established given 2 layers.  
    \item  $\sigma_0$ is the $\sigma$ value of the previous layer
    \item  $\sigma_1$ is the $\sigma$ value of the current layer
    \item  $c$ is the number of classes
    \item  $n$ is total number of samples
    \item  $n_i$ is number of samples in the $i^{th}$ class
    
    \item  $\sigma_0$ is number of samples in the $i^{th}$ class
    
    \item  $\cS$ is a set of all $i,j$ sample pairs where $r_i$ and $r_j$ belong to the same class.
    \item  $\cS^c$ is a set of all $i,j$ sample pairs where $r_i$ and $r_j$ belong to different same classes.
    \item  $\cS^{\beta}$ is a set of all $i,j$ sample pairs that belongs to the same $\beta^{th}$ classes.
    \item  $r_i^{\alpha}$ is the $i^{th}$ sample in the $\alpha^{th}$ class among $c$ classes.
    \item  We assume no $r_i \ne r_j$ pair are equal $\forall i \ne j$. 
    \item  Among all $r_i \ne r_j$ pairs, there exists an optimal $r_i^*, r_j^*$ pair where  
    $\langle r_i^*, r_j^* \rangle \ge \langle r_i, r_j \rangle$ $\forall r_i \ne r^*_i$ and $r_j \ne r^*_j$. We denote this maximum inner product as 
    \begin{equation}
        \ub = \langle r_i^*, r_j^* \rangle.
    \end{equation}
    \item In \kc, each $r_i$ sample is assumed to be a sample in the RKHS of the \rbfk, therefore all inner products are bounded such that
    \begin{equation}
        0 \le \langle r_i, r_j \rangle 
        \le
        \ub.
    \end{equation}
    \item We let $W$ be 
    \begin{equation}
        W_s = \frac{1}{\sqrt{\zeta}} \W.
    \end{equation}
    Instead of using an optimal $W^*$, we use a suboptimal $W_s$ where each dimension is simply the average direction of each class: $\frac{1}{\sqrt{\zeta}}$ is a normalizing constant the ensures $W^TW=I$. By using $W_s$, this implies that the $\hsic$ we obtain is already a lower bound compare $\hsic$ obtained by $W^*$. But, we will use this suboptimal $W_s$ to identify an even lower bound.
    \item  We let the objective $\hsic$ be
    \begin{equation}
        \hsic = 
        \underbrace{
        \sums \Gij \ISMexpC{}{}}_{\within}
        -
        \underbrace{
        \sumsc |\Gij| \ISMexpC{}{}}_{\between}
    \end{equation}
    where we let $\within$ be the summation of terms associated with the within cluster pairs, and let $\between$ be the summation of terms associated with the between cluster pairs.
\end{enumerate}

\begin{proof} $\hspace{1pt}$
\begin{adjustwidth}{0.5cm}{0.0cm}
    Due to the length of this proof, the equation is divided into smaller parts organized into multiple sections.
    
    \textbf{For sample pairs in $\cS$. } The first portion of the function can be split into multiple classes where
    \begin{equation}
    \within = 
    \underbrace{
    \sum_{\cS^1} \Gij \ISMexpC{(1)}{(1)}
    }_\text{$\within_1$}
    + ... + 
    \underbrace{
    \sum_{\cS^c} \Gij \ISMexpC{(c)}{(c)}}_\text{$\within_c$}
    \end{equation}
    Realize that to find the lower bound, the key is to determine the maximum possible values for each exponent term. Since every one of them are the same, we can simply look at the numerator of the exponent from $\within_1$. Given $W_s$ as $W$, our goal is identify the maximum possible value for
    \begin{equation}
        \underbrace{
        \rij{1}{1}^TW}_{\Pi_1}
        \underbrace{
        W^T\rij{1}{1}}_{\Pi_2}. 
    \end{equation}
    Zoom in further by looking only at $\Pi_1$, we have 
    the following relationships
    \begin{equation}
       \Pi_1 = 
        \underbrace{
            r_i^{(1)^T} W}_{\xi_1}
        - 
        \underbrace{r_j^{(1)^T} W}_{\xi_2} 
    \end{equation}
    \begin{align}
        \xi_1 & = r_i^{(1)^T} \W \\
        & = r_i^{(1)^T} 
            \begin{bmatrix}
                (r_1^{(1)} + ... + r_{n_1}^{(1)}) &
                ... &
                (r_1^{(c)} + ... + r_{n_1}^{(c)})
            \end{bmatrix}
    \end{align}
    \begin{align}
        \xi_2 & = r_j^{(1)^T} \W \\
        & = r_j^{(1)^T} 
            \begin{bmatrix}
                (r_1^{(1)} + ... + r_{n_1}^{(1)}) &
                ... &
                (r_1^{(c)} + ... + r_{n_1}^{(c)})
            \end{bmatrix}
    \end{align}   
    By knowing that the inner product is constrained between $[0,\ub]$, we know the maximum possible value for $\xi_1$ and the minimum possible value for $\xi_2$ to be
     \begin{align}
        \xi_1 & = 
            \begin{bmatrix}
                1 + (n_1 - 1)\ub &
                n_2 \ub &
                n_3 \ub &
                ... &
                n_c \ub
            \end{bmatrix} \\
         \xi_2 & = 
            \begin{bmatrix}
                1 &
                0 &
                0 &
                ... &
                0
            \end{bmatrix}. 
    \end{align}   
    Which leads to  
    \begin{equation}
        \Pi_1 = 
        \xi_1 - \xi_2 = 
            \begin{bmatrix}
                (n_1 - 1)\ub &
                n_2 \ub &
                n_3 \ub &
                ... &
                n_c \ub
            \end{bmatrix}
    \end{equation}
    Since $\Pi_1 \Pi_2 = \Pi_1 \Pi_1^T$, we have 
    \begin{align}
        \Pi_1 \Pi_2 & = 
            (n_1 - 1)^2\ub^2 + 
            n_2^2 \ub^2 +
            n_3^2 \ub^2 +
                ... +
            n_c^2 \ub^2 \\
        & = 
            [(n_1 - 1)^2+ 
            n_2^2 +
            n_3^2 +
                ... +
            n_c^2] \ub^2
    \end{align}
    The lower bound for just the $\within_1$ term emerges as 
    \begin{equation}
        \within_1 \ge 
        \sum_{\cS^1} \Gij e^{
        - \frac{ 
            [(n_1 - 1)^2+ 
            n_2^2 +
            n_3^2 +
                ... +
            n_c^2] \ub^2 }{2 \zeta \sigma_1^2}}. 
    \end{equation}
    To further condense the notation, we define the following
    \begin{equation}
        \mathscr{N}_g = 
            \frac{1}{2 \zeta}
            [n_1^2+ 
            n_2^2 +
            ... +
            (n_g - 1) + 
            ... + 
            n_c^2].
    \end{equation}
    Therefore, the lower bound for $\within_1$ can be simplified as 
    \begin{equation}
        \within_1 \ge \sum_{\cS^1} \Gij e^{-\frac{\mathscr{N}_1 \ub^2}{\sigma_1^2}}
    \end{equation}
    and the general pattern for any $\within_g$ becomes
    \begin{equation}
         \within_g \ge \sum_{\cS^i} \Gij e^{-\frac{\mathscr{N}_g \ub^2}{\sigma_1^2}}. 
    \end{equation}
    The lower bound for the entire set of $\cS$ then becomes
    \begin{equation}
        \sums \Gij \ISMexpC{}{} = 
        \within_1 + ... + \within_c \ge 
        \underbrace{
        \sum_{g=1}^c \sum_{\cS^g} \Gij
        e^{-\frac{\mathscr{N}_g \ub^2}{\sigma_1^2}}}_{\text{Lower bound}}.
    \end{equation}
    
    \textbf{For sample pairs in $\cS^c$. } 
    
    We now derived the lower bound for the sample pairs in $\cS^c$.  
    \begin{align}
    \between & = 
    \underbrace{
    \sum_{i \in \cS^1} 
    \sum_{j \in \cS^2}
    |\Gij| \ISMexpC{(1)}{(2)}
    }_\text{$\between_{1,2}$} \\
    & + 
    \underbrace{
    \sum_{i \in \cS^1} 
    \sum_{j \in \cS^3}
    |\Gij| \ISMexpC{(1)}{(3)}
    }_\text{$\between_{1,3}$} \\
    & + ... \\
    & +
    \underbrace{
    \sum_{i \in \cS^c} 
    \sum_{j \in \cS^{c-1}} 
    |\Gij| \ISMexpC{(c)}{}}_\text{$\between_{c,c}$}
    \end{align}
    Using the similar approach, note that $\between$ is a negative value, so we need to maximize this term to obtain a lower bound. Consequently, the key is to determine the \textbf{minimum} possible values for each exponent term. Since every one of them will behave very similarly, we can simply look at the numerator of the exponent from $\between_{1,2}$ and then arrive to a more general conclusion. Given $W_s$ as $W$, our goal is identify the \textbf{minimize} possible value for
    \begin{equation}
        \underbrace{
        \rij{1}{2}^TW}_{\Pi_1}
        \underbrace{
        W^T\rij{1}{2}}_{\Pi_2}. 
    \end{equation}
  
    Zoom in further by looking only at $\Pi_1$, we have 
    the following relationships
    \begin{equation}
       \Pi_1 = 
        \underbrace{
            r_i^{(1)^T} W}_{\xi_1}
        - 
        \underbrace{r_j^{(2)^T} W}_{\xi_2} 
    \end{equation}
    \begin{align}
        \xi_1 & = r_i^{(1)^T} \W \\
        & = r_i^{(1)^T} 
            \begin{bmatrix}
                (r_1^{(1)} + ... + r_{n_1}^{(1)}) &
                ... &
                (r_1^{(c)} + ... + r_{n_1}^{(c)})
            \end{bmatrix}
    \end{align}
    \begin{align}
        \xi_2 & = r_j^{(2)^T} \W \\
        & = r_j^{(2)^T} 
            \begin{bmatrix}
                (r_1^{(1)} + ... + r_{n_1}^{(1)}) &
                ... &
                (r_1^{(c)} + ... + r_{n_1}^{(c)})
            \end{bmatrix}
    \end{align}   
    By knowing that the inner product is constrained between $[0,\ub]$, we know the \textbf{minimum} possible value for $\xi_1$ and the \textbf{maximum} possible value for $\xi_2$ to be
     \begin{align}
        \xi_1 & = 
            \begin{bmatrix}
                1 &
                0 &
                0 &
                ... &
                0
            \end{bmatrix} \\
         \xi_2 & = 
            \begin{bmatrix}
                n_1\ub &
                1 + (n_2 - 1) \ub &
                n_3 \ub &
                ... &
                n_c \ub
            \end{bmatrix} 
    \end{align}   
    Which leads to  
    \begin{equation}
        \Pi_1 = 
        \xi_1 - \xi_2 = 
            \begin{bmatrix}
                1 - n_1\ub &
                -(1 + (n_2 - 1) \ub) &
                -n_3 \ub &
                ... &
                -n_c \ub
            \end{bmatrix}
    \end{equation}
    Since $\Pi_1 \Pi_2 = \Pi_1 \Pi_1^T$, we have     
    \begin{align}
        \Pi_1 \Pi_2 & = 
            (1- n_1 \ub)^2 + 
            (1 + (n_2-1)\ub)^2 + 
            n_3^2 \ub^2 +
                ... +
            n_c^2 \ub^2.
    \end{align}
    The lower bound for just the $\between_{1,2}$ term emerges as 
    \begin{equation}
        -\between_{1,2} \ge 
        - \sum_{\cS^1} |\Gij| e^{
        - \frac{ 
            (1- n_1\ub)^2 + 
            (1 + (n_2-1)\ub)^2 + 
            n_3^2 \ub^2 +
                ... +
            n_c^2 \ub^2}
            {2 \zeta \sigma_1^2}}. 
    \end{equation}
    To further condense the notation, we define the following function
    \begin{align}
        \mathscr{N}_{g_1, g_2}(\ub) & = 
            \frac{1}{2 \zeta}
            [ n_1^2 \ub^2 + n_2^2 \ub^2 + ... \\ 
            & +  (1- n_{g_1}\ub)^2 + ... + 
            (1 + (n_{g_2}-1)\ub)^2 \\
            & + ...  + n_c^2 \ub^2].
    \end{align}
    Note that while for $\cS$, the $\ub$ term can be separated out. But here, we cannot, and therefore $\mathscr{N}$ here must be a function of $\ub$.  Therefore, the lower bound for $\between_{1,2}$ can be simplified into
    \begin{equation}
        - \between_{1,2} \ge - \sum_{\cS^1} |\Gij| e^{-\frac{\mathscr{N}_{1,2}(\ub)}{\sigma_1^2}}
    \end{equation}
    and the general pattern for any $\between_{g_1, g_2}$ becomes
    \begin{equation}
         \between_{g_1,g_2} \ge \sum_{\cS^i} \Gij e^{-\frac{\mathscr{N}_{g_1,g_2}(\ub)}
         {\sigma_1^2}}. 
    \end{equation}    
    The lower bound for the entire set of $\cS^c$ then becomes
    \begin{align}
        -\sumsc |\Gij| \ISMexpC{}{} & = 
        - \between_{1,2} 
        - \between_{1,3} 
        - ... - 
        \between_{c-1, c} \\
        & \ge 
        - \underbrace{
        \sum_{g_1 \ne g_2}^c 
        \sum_{i \in \cS^{g_1}} 
        \sum_{j \in \cS^{g_2}} 
        |\Gij|
        e^{-\frac{\mathscr{N}_{g_1,g_2} (\ub)}{\sigma_1^2}}}_{\text{Lower bound}}.
    \end{align}    
    
    
\end{adjustwidth}
\end{proof}


\end{appendices}

==> appen2/ag_not_optimal.tex <==
\subsection{Show that $W = \sum_i r_i$ is Not the Optimal Solution}
\begin{lemma}
\label{app:lemma:W_not_optimal} Given $\epsilon$ as a normalizing constant for  $W = \epsilon \sum_i r_i$ such that $W^TW=I$, then $W$ is not the optimal solution for the HSIC objective.
\end{lemma}

\begin{proof}
    We here provide a proof for 2 classes. We let the sample from $\cS^1$ be $r_i$ and samples from $\cS^2$ be $t_i$. We start with the Lagrangian
    \begin{equation}
        \mathcal{L} = 
        - \sum_{\cS^1} \Gij \ISMexp.
        - \sum_{\cS^2} \Gij 
        e^{-\frac{(t_i - t_j)^T W W^T(t_i - t_j)}{2 \sigma^2}}
        + \sum_{\cS^c} \Gij e^{-\frac{(r_i - t_j)^T W W^T(r_i - t_j)}{2 \sigma^2}}.
    \end{equation}
    To simplify the formulation, we can simply assume that $W$ is always scaled to satisfy $W^TW = I$. If we now take the derivative with respect to the Lagrange, we get
    \begin{align}
        \nabla \mathcal{L} = &
        - \sum_{\cS^1} \Gij \ISMexp
        (r_i - r_j)(r_i - r_j)^TW\\
        & - \sum_{\cS^2} \Gij 
        e^{-\frac{(t_i - t_j)^T W W^T(t_i - t_j)}{2 \sigma^2}}
        (t_i - t_j)(t_i - t_j)^TW\\
        &  + \sum_{\cS^c} \Gij e^{-\frac{(r_i - t_j)^T W W^T(r_i - t_j)}{2 \sigma^2}}.   
        (r_i - t_j)(r_i - t_j)^TW.
    \end{align}
    Now, we put $W = \sum_i r_i$ into the gradient of the Lagrangian and we can clearly see that it is not always equal to 0.
    \begin{align}
        \nabla \mathcal{L}((\epsilon \sum_{\alpha} r_\alpha)) = &
        - \sum_{\cS^1} \Gij e^{-\frac{(r_i - r_j)^T (\epsilon\sum_{\alpha} r_\alpha) (\epsilon\sum_{\alpha} r_\alpha)^T(r_i - r_j)}{2 \sigma^2}}
        (r_i - r_j)(r_i - r_j)^T(\epsilon\sum_{\alpha} r_\alpha)\\
        & - \sum_{\cS^2} \Gij 
        e^{-\frac{(t_i - t_j)^T (\epsilon\sum_{\alpha} r_\alpha) (\sum_{\alpha} r_\alpha)^T(t_i - t_j)}{2 \sigma^2}}
        (t_i - t_j)(t_i - t_j)^T (\epsilon\sum_{\alpha} r_\alpha)\\
        &  + \sum_{\cS^c} \Gij e^{-\frac{(r_i - t_j)^T (\epsilon\sum_{\alpha} r_\alpha) (\epsilon\sum_{\alpha} r_\alpha)^T(r_i - t_j)}{2 \sigma^2}}   
        (r_i - t_j)(r_i - t_j)^T(\epsilon\sum_{\alpha} r_\alpha) \ne 0.
    \end{align}
\end{proof}

==> appen2/ai_regularizer.tex <==
\begin{appendices} 
\section{Proof for Theorem \ref{thm:regularizer}}
\label{app:thm:regularizer}

\textbf{Theorem \ref{thm:regularizer}: }
\textit{\eq{eq:similarity_hsic} objective is equivalent to }
\begin{equation}
        \sum_{i,j}
        \Gij \ISMexp
        (r_i^TWW^Tr_j)
        -
        \sum_{i}
        D_i(W)
        ||W^Tr_i||_2.
\end{equation}

\begin{proof}
Let $A_{i,j} = (r_i - r_j)(r_i - r_j)^T$. Given the Lagranian of the HSIC objective as 
\begin{equation}
    \mathcal{L} = -\sum_{i,j} \Gij \ISMexp - \Tr[\Lambda(W^TW - I)].
\end{equation}
Our layer wise HSIC objective becomes 
\begin{equation}
    \min_W -\sum_{i,j} \Gij \ISMexp - \Tr[\Lambda(W^TW - I)].
    \label{obj:hsic}
\end{equation}
We take the derivative of the Lagrangian, the expression becomes
   \begin{equation} \label{eq:gradient_of_lagrangian}
    \nabla_W \mathcal{L} ( W, \Lambda) = \sum_{i, j} \frac{\Gamma_{i,
      j}}{\sigma^2} e^{- \frac{\Tr (W^T A_{i, j} W)}{2 \sigma^2}} A_{i, j} W
      - 2 W \Lambda. 
    \end{equation}
Setting the gradient to 0, and consolidate some scalar values into $\hat{\Gamma}_{i,j}$, we get the expression
   \begin{align} 
    \left[
    \sum_{i, j} \frac{\Gamma_{i,
      j}}{2\sigma^2} e^{- \frac{\Tr (W^T A_{i, j} W)}{2 \sigma^2}} A_{i, j} 
     \right]
      W
      & =  W \Lambda \\
      \left[\frac{1}{2}
      \sum_{i,j} \hat{\Gamma}_{i,j} A_{i,j}
      \right] W
      & = W \Lambda \\
      \mathcal{Q} W
      & = W \Lambda.      
    \end{align}
From here, we see that the optimal solution is an eigenvector of $\mathcal{Q}$. Based on ISM, it further proved that the optimal solution is not just any eigenvector, but the eigenvectors associated with the smallest values of $\mathcal{Q}$. From this logic, ISM solves objective~(\ref{obj:hsic}) with a surrogate objective
\begin{equation}
    \min_W \quad
        \Tr \left( W^T
        \left[\frac{1}{2}
        \sum_{i,j} \hat{\Gamma}_{i,j} A_{i,j}
        \right] W \right) \quad \st W^TW=I.
    \label{obj:min_2}
\end{equation}
Given $D_{\hat{\Gamma}}$ as the degree matrix of $\hat{\Gamma}$ and $R = [r_1, r_2, ...]^T$, ISM further shows that Eq.~(\ref{obj:min_2}) can be written into
\begin{align}
    \min_W \quad
        \Tr \left( W^T R^T
        \left[
        D_{\hat{\Gamma}} - \hat{\Gamma}
        \right] R W \right) &\quad \st W^TW=I \\
     \max_W \quad
        \Tr \left( W^T R^T
        \left[
        \hat{\Gamma} - 
        D_{\hat{\Gamma}}
        \right] R W \right) &\quad \st W^TW=I \\       
     \max_W \quad
        \Tr \left( W^T R^T
        \hat{\Gamma}  
        R W \right) 
        -
        \Tr \left( W^T R^T
        D_{\hat{\Gamma}}  
        R W \right) 
        &\quad \st W^TW=I \\              
     \max_W \quad
        \Tr \left( 
        \hat{\Gamma}  
        R W W^T R^T\right) 
        -
        \Tr \left( 
        D_{\hat{\Gamma}}  
        R W W^T R^T\right) 
        &\quad \st W^TW=I \\                     
     \max_W \quad
        \sum_{i,j}
        \hat{\Gamma}_{i,j}
        [R W W^T R^T]_{i,j}
        -
        \sum_{i,j}
        D_{\hat{\Gamma}_{i,j}}
        [R W W^T R^T]_{i,j}       
        &\quad \st W^TW=I. 
\end{align}
Since the jump from \eq{obj:min_2} can be intimidating for those not familiar with the literature, we included a more detailed derivation in App.~\ref{app:matrix_derivation}.

Note that the degree matrix $D_{\hat{\Gamma}}$ only have non-zero diagonal elements, all of its off diagonal are 0. Given $[RWW^TR^T]_{i,j} = (r_i^TWW^Tr_j)$, the objective becomes
\begin{equation}
     \max_W \quad
        \sum_{i,j}
        \hat{\Gamma}_{i,j}
        (r_i^TWW^Tr_j)
        -
        \sum_{i}
        D_i(W)
        ||W^Tr_i||_2
        \quad \st W^TW=I.     
\end{equation}
Here, we treat $D_{i}$ as a penalty weight on the norm of the $W^Tr_i$ for every sample. 
\end{proof}


To better understand the behavior of $D_i(W)$, note that $\hat{\Gamma}$ matrix looks like
\begin{equation}
    \hat{\Gamma} = \frac{1}{\sigma^2} \begin{bmatrix}
       \begin{bmatrix}
       \Gamma_{\mathcal{S}} \ISMexp
        \end{bmatrix}
       &  
       \begin{bmatrix}
       -|\Gamma_{\mathcal{S}^c}| \ISMexp
       \end{bmatrix}
       &
       ... \\
       \begin{bmatrix}
       -|\Gamma_{\mathcal{S}^c}| \ISMexp
       \end{bmatrix}
       &      
       \begin{bmatrix}
       \Gamma_{\mathcal{S}} \ISMexp
        \end{bmatrix}      
       &            
       ... \\
       ... &
       ... &
       ...
    \end{bmatrix}.
\end{equation}
The diagonal block matrix all $\Gij$ elements that belong to $\cS$ and the off diagonal are elements that belongs to $\cS^c$. Each penalty term is the summation of its corresponding row. Hence, we can write out the penalty term as
\begin{equation}
    D_i(W_l) = 
    \frac{1}{\sigma^2}
    \sum_{j \in \cS|i}
    \Gij \kf_{W_l}(r_i,r_j)
    -
    \frac{1}{\sigma^2}
    \sum_{j \in \cS^c|i}
    |\Gij| \kf_{W_l}(r_i,r_j).
\end{equation}
From this, it shows that as $W$ improve the objective, the penalty term is also increased. In fact, at its extreme as $\hsic_l \rightarrow \hsic^*$, all the negative terms are gone and all of its positive terms are maximized and this matrix approaches 
\begin{equation}
    \hat{\Gamma}^* = \frac{1}{\sigma^2} \begin{bmatrix}
       \begin{bmatrix}
       \Gamma_{\mathcal{S}} 
        \end{bmatrix}
       &  
       \begin{bmatrix}
       0
       \end{bmatrix}
       &
       ... \\
       \begin{bmatrix}
       0
       \end{bmatrix}
       &      
       \begin{bmatrix}
       \Gamma_{\mathcal{S}} 
        \end{bmatrix}      
       &            
       ... \\
       ... &
       ... &
       ...
    \end{bmatrix}.
\end{equation}
From the matrix $\hat{\Gamma}^*$ and the definition of $D_i(W_l)$, we see that as $\mathcal{K}_W$ from $\mathcal{S}$ increase, 

Since $D_i(W)$ is the degree matrix of $\hat{\Gamma}$, we see that as $\hsic_l \rightarrow \hsic^*$, we have
\begin{equation}
   D^*_i(W) > D_i(W). 
\end{equation}
\end{appendices} 

==> appen2/zz_hold.tex <==


\newpage

\textbf{Aria's thought pattern of the proof:}

The goal is to build a sequence of networks that has the properties statement in the thm1. 


First we proof the following the second statement:

\textbf{Theorem \ref{thm:hsequence}: }
\textit{For any $\hsic_0$, $L>1$ and $\delta>0$ there exists a sequence of kernel feature maps $\{\fm_l\}_{l=1}^L$ parameterized by $\{W_l\}_{l=1}^L$ and $\{\sigma_{l}\}_{l=1}^L$ such that:
}
     II) in finite $L$ we can get arbitrary close to convergence value where:
        \begin{equation}
        \label{eq:app:finite_conv}
        \hsic^{*} - \hsic_L \le \delta
    \end{equation}

\begin{proof}
\begin{lemma}
Choosing $\{W_l\}_{l=1}^L = \sum_{i\in \mathcal{S}^1}$ and any $\{\sigma_{l}\}_{l=1}^{L-2}> 0 $, there exist a $\sigma_{L-1}$ and $\sigma_{L}$, where: \begin{equation}
        \label{eq:app:finite_conv}
        \hsic^{*} - \hsic_L \le \delta
    \end{equation}
    \end{lemma}
    \begin{proof}
    
    Given the formulation of $\hsic_{L}$ as follows: 
    
      \begin{equation}
    \hsic_{l} = \underbrace{ 
    \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma_{l}^2}}
    }_\text{1st term}
    -
    \underbrace{
    \sum_{i,j \in \mathcal{S}^c} |\Gij| 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma_{l}^2}} 
    }_\text{2nd term}
    \label{hsic equation}
\end{equation}
    
    There exist a lower bound $L(\sigma_{L-1}, \sigma_{L})$, define as follows, (\textbf{the details of derivation in another lemma}):
    
    \begin{equation}
    L(\sigma_{L-1},\sigma_{L}) = 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\mathcal{E}(\sigma_{L-1}))^2 - 2 }{2\sigma_L^2}}
    + 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2(n\mathcal{E}(\sigma_{L-1}))^2 }{2\sigma_L^2}}    
    -
   \sum_{i,j \in \mathcal{S}^c} |\Gij| 
   e^{-\frac{1 - 2n\mathcal{E}(\sigma_{L-1})(1+(n-1)\mathcal{E}(\sigma_{L-1})))}{2\sigma_{L}^2}}. 
\end{equation}
Where $\mathcal{E}(\sigma_{L-1}) = <r_{i},r_{j}> = e^\frac{-|.|^2}{2\sigma_{l-1} ^2}$ \textbf{We can more details here, or we can introduce in the beginning}.
This lower bound is a global lower bound to $\hsic_{L}$ for a given $\sigma_{L-1}$,$\sigma_{L}$. i.e. $\hsic_{L}(\sigma_{L-1}$,$\sigma_{L}) \geq L(\sigma_{L-1}$,$\sigma_{L})$. Furthermore it can be seen that this lower bound is a continuous function of $\sigma_{L-1}$,$\sigma_{L}$. In addition, $L(\sigma_{L-1}$,$\sigma_{L})$ is a decreasing function of $\sigma_{L-1}$:     

   Given this lower bound, it is a decreasing function with respect to $\sigma_{l-1}$, and consequently $\mathcal{E}(\sigma_{l-1})$. This can be seen easily by taking the derivative with respect to $\mathcal{E}$ and showing that the derivative is always < 0.
   
\begin{equation}
    L(\mathcal{E}) = 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\mathcal{E})^2 - 2 }{2\sigma_l^2}}
    + 
    \sum_{i,j \in \mathcal{S}^2} \Gamma_{i,j} 
    e^{-\frac{2(n\mathcal{E})^2 }{2\sigma_l^2}}    
    -
   \sum_{i,j \in \mathcal{S}^c} |\Gij| 
   e^{-\frac{1 - 2n\mathcal{E}(1+(n-1)\mathcal{E}(\sigma_{l-1})))}{2\sigma_{l}^2}}. 
\end{equation}  

Taking derivative for each term with respect to $\mathcal{E}$ we obtain the following:
%\begin{equation}
%    \frac{\partial}{\partial \mathcal{E}}
%    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
%    e^{-\frac{2(1+(n-1)\mathcal{E})^2 - 2 }{2\sigma_l^2}} 
%    = 
%    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
%    e^{-\frac{2(1+(n-1)\mathcal{E})^2 - 2 }{2\sigma_l^2}}   
%    \left[
%    - \frac{2(1+(n-1)\mathcal{E})(n-1)}{\sigma_l^2}
%    \right] 
%    \le 0
%\end{equation}  

\begin{align}
    \frac{\partial}{\partial \mathcal{E}}
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\mathcal{E})^2 - 2 }{2\sigma_l^2}} 
    & = 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\mathcal{E})^2 - 2 }{2\sigma_l^2}}   
    \left[
    - \frac{2(1+(n-1)\mathcal{E})(n-1)}{\sigma_l^2}
    \right] 
    & \le 0 \\
    \frac{\partial}{\partial \mathcal{E}}
    \sum_{i,j \in \mathcal{S}^2} \Gamma_{i,j} 
    e^{-\frac{2(n\mathcal{E})^2 }{2\sigma_l^2}}    
    & = 
    \sum_{i,j \in \mathcal{S}^2} \Gamma_{i,j} 
    e^{-\frac{2(n\mathcal{E})^2 }{2\sigma_l^2}}       
    \left[
    -\frac{(n\mathcal{E})^2}{\sigma_l^2}
    \right]
    & \le 0  \\
   \frac{\partial}{\partial \mathcal{E}}
   -\sum_{i,j \in \mathcal{S}^c} |\Gij| 
   e^{-\frac{1 - 2n\mathcal{E}(1+(n-1)\mathcal{E}(\sigma_{l-1})))}{2\sigma_{l}^2}}
   & = 
   -\sum_{i,j \in \mathcal{S}^c} |\Gij| 
   e^{-\frac{1 - 2n\mathcal{E}(1+(n-1)\mathcal{E}(\sigma_{l-1})))}{2\sigma_{l}^2}}
   & \le 0.
\end{align}
It can be seen that all 3 terms are negative. This implies that as $\mathcal{E}$ increases, $L(\mathcal{E})$ is a decreasing function. Conversely, as $\mathcal{E} \rightarrow 0$,  $L(\mathcal{E})$ is an increasing function. As $\sigma_{L-1} \rightarrow 0$ the limit behavior continuously approaches to the following:

According to \citelemma{lemma:Lbound_LHS}, there exists a lower bound for the LHS of (\ref{ineq:kchain_inequality}) that is also a function of $\sigma_{L-1}$ which we denote as $L(\sigma_{L-1})$. As shown by the lemma, as $\sigma_{L-1}$ decreases $L(\sigma_{L-1})$ increases towards a limit point $L^*$. Formally, we have
\begin{equation}
    \lim_{\sigma_{L-1} \rightarrow 0} 
    L(\sigma_{L-1}) = L^*
\end{equation}
where
\begin{equation}
    L^* = \sums \Gij - \sumsc \Gij
    e^{-\frac{1}{2\sigma_L^2}}.
    \label{eq:lower_limit}
\end{equation}.

Notice that $L^{*} = \hsic^{*} - \sumsc \Gij
    e^{-\frac{1}{2\sigma_L^2}}$. hence by condoling $\sigma_{L}$, we can get arbitrary close to $\hsic^{*}$.
    
    
Now for $\delta > 0 $, choose $\sigma_{L-1}$ such that $L^{*}(\sigma_{L}) - L(\sigma_{L-1},\sigma_{L}) \leq \delta / 2$. and choose a $\sigma_{L}$ such that $\mathcal{H}^{*} - L^* \leq \delta/2$, hence by summing these two up we have:

$$\hsic^{*} - L^* \leq \delta /2$$.
Which conclude this lemma's proof. 
    \end{proof}
    
    
Note that for a given $L > 2$ the control over two last layer is enough to make $\hsic_{L}$ arbitrary close to $\hsic^{*}$. Hence for any given $L$ there exist a sequence with $W$ as mean over one of the classes in RKHS. This proof is generelized to more than 2 classes in \textbf{Lemma}.  
    
    
    
    
\end{proof}

Now we use the aforementioned construction to make a sequence of network with $l$ layers that has the I and III properties:

I)  as $l \rightarrow \infty$, the sequence converges to the global optimal where
    \begin{equation}
        \label{eq:app:converge_to_global}
        \lim_{l \rightarrow \infty}  \hsic_l = \hsic^*,
    \end{equation}
    
    III) The convergence is monotonic where
    \begin{equation}
    \label{eq:app:ineq}
    \hsic_{l} > \hsic_{l-1} \quad \forall l.
    \end{equation}.
    
\textbf{I)}: We have to construct a Kernel sequence $\{\hsic_{l}\}_{l=1}^\infty$, where for any $\delta>0$, $\exists l < \infty$ such that $$\hsic^{*} - \hsic_{l} \leq \delta $$. 
Fromm the II condition, this construction is trivial, we just set $\delta_{l} = \frac{1}{l}$. Hence we prove the following: 

$$\forall l>0: \hsic^{*} - \hsic_{l} \leq \delta_{l}$$

This construction is enough to show that $ \lim_{l \rightarrow \infty}  \hsic_l = \hsic^*$, because for any arbitrary $\delta>0$ there exist an $l$ such that $\delta > 1\l$.

From II, constructing this sequence of kernel can be controlled by $\sigma_{l-1},\sigma_{l}$ so that $\hsic^{*} - \hsic_{l} \leq \delta_{l}$, hence: $$\lim_{l \rightarrow \infty}  \hsic_l = \hsic^{*}$$.

III) Furthermore this construction satisfies the following: 

$ \hsic^{*} - \hsic_{l} \leq \frac{1}{l} , \forall l>0: \hsic^{*} - \hsic_{l+1} \leq \frac{1}{l+1} \rightarrow \hsic_{l+1} - \hsic_{l} < \frac{1}{l} - \frac{1}{l+1}$, hence $\hsic_{l+1} > \hsic_{l}$.

Which concludes the proof of the theorem..




\newpage

\textbf{Organization of the Proof. }

\begin{enumerate}[label=\Roman*. ]
    \item
        \eq{eq:app:ineq} is first proven in 
        \citelemma{lemma:ineq_lemma}.
   \item 
        Without a loss of generality, we first assume to only have 2 classes where the set of sample pairs from the 1st and 2nd classes are denoted as $\mathcal{S}^1$ and $\mathcal{S}^2$. The generalization to 3 classes can be found at \citelemma{lemma:extension_3_class}.       
    \item
        We next prove \eq{eq:app:converge_to_global}
        and \eq{eq:app:finite_conv}
        in \citelemma{app:lemma:conv_to_global}. This proof is only understandable given the logical steps of 
        \citelemma{lemma:ineq_lemma}.
    \item  
        Due to the length of the proof, it is difficult to find a mistake. For this reason, we simulated the proof step by step in python. The results and the details of this simulation can be found at.
    \end{enumerate}


\textbf{Notations and Assumptions of the Proof. }
\begin{enumerate}
  \item $n$ is the number of samples.
  \item $\mathcal{S}$ is the set of $i,j$ sample pairs that belongs to the same class.
  \item $\mathcal{S}^c$ is the set of $i,j$ sample pairs that belongs to different classes. 
  \item Since $\Gamma = HK_YH$, $\sum_{i,j} \Gij = 0$.
  \item To simplify the notation, we let $W = W_l$ in the proof.
  \item We let $\sigma_{l-1}$ and $\sigma_l$ be the $\sigma$ values used for the previous and current layer respectively.
  \item Instead of finding the optimal $W$,  
  we let $W_l = \sum_{i\in \mathcal{S}^1}r_{i}$. The reason why we use this instead of an optimal $W_l$ is that if there exists an non-optimal $W_l$ that satisfies the inequality, then there must also exists an optimal $W_l$ that satisfies the inequality. We emphasize that the goal here is to prove the existence of $W_l$ that satisfies the inequality.
\end{enumerate}





\setcounter{lemma}{0}
\begin{lemma}
\label{lemma:ineq_lemma}
Given $r_{i} =  \fm_{l-1} \circ ... \circ \fm_1 (x_{i})$ and $\fm_l = \af \circ \mathcal{W}_l$, there exist a sequence of $\{\sigma_{l}\}_{l\geq 1}$, $\sigma_l > 0$ such that
  \begin{equation}
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma_{l}^2}}
    }_\text{1st term}
    -
    \underbrace{
    \sum_{i,j \in \mathcal{S}^c} |\Gij| 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma_{l}^2}} 
    }_\text{2nd term}
    \quad \geq 
    \sum_{i,j \in \mathcal{S}\cup \mathcal{S}^{c}} \Gamma_{i,j} 
    r_{i}^{T}r_{j}
    \label{ineq:kchain_inequality}
\end{equation}
\end{lemma}

\begin{proof}
According to \citelemma{lemma:Ubound_RHS}, there exists an upper bound for the RHS of (\ref{ineq:kchain_inequality}) that is a function of $\sigma_{l-1}$ which we denote as $U(\sigma_{l-1})$. Additionally, \citelemma{lemma:Ubound_RHS} shows that as $\sigma_{l-1}$ decreases $U(\sigma_{l-1})$ also decrease towards 0. Formally, we have
\begin{equation}
    \lim_{\sigma_{l-1} \rightarrow 0} 
    U(\sigma_{l-1}) = 0. 
\end{equation}
According to \citelemma{lemma:Lbound_LHS}, there exists a lower bound for the LHS of (\ref{ineq:kchain_inequality}) that is also a function of $\sigma_{l-1}$ which we denote as $L(\sigma_{l-1})$. As shown by the lemma, as $\sigma_{l-1}$ decreases $L(\sigma_{l-1})$ increases towards a limit point $L^*$. Formally, we have
\begin{equation}
    \lim_{\sigma_{l-1} \rightarrow 0} 
    L(\sigma_{l-1}) = L^*
\end{equation}
where
\begin{equation}
    L^* = \sums \Gij - \sumsc \Gij
    e^{-\frac{1}{2\sigma_l^2}}.
    \label{eq:lower_limit}
\end{equation}
Instead of proving the inequality (\ref{ineq:kchain_inequality}) directly, we can use the upper and lower bounds instead, i.e., (\ref{ineq:kchain_inequality}) is satisfied when the following inequality is satisfied:
\begin{equation}
    L(\sigma_{l-1}) \ge U(\sigma_{l-1}).
\end{equation}
Assuming that $\sigma_{l-1}$ is randomly initialized at $\sigma_{l-1}^{(0)}$, $L(\sigma_{l-1}^{(0)})$ may or may not be greater than $U(\sigma_{l-1}^{(0)})$. We wish to know that even in the event that $L(\sigma_{l-1}^{(0)}) < U(\sigma_{l-1}^{(0)})$, if we decrease $\sigma_{l-1} \rightarrow 0$, is there a $\sigma_{l-1}^* > 0$ such that 
\begin{equation}
    L(\sigma_{l-1}^{*}) \ge U(\sigma_{l-1}^{*}).
    \label{ineq:lowUpbound}
\end{equation}

As $\sigma_{l-1}^{(0)} \rightarrow 0$, there are 3 possible cases as shown in Fig.~\ref{fig:bound_limits}.

\begin{figure}[!ht]
\center
    \includegraphics[width=13cm,height=6cm]{img/sigma_trends.png}
    \caption{3 cases as $\sigma_{l-1} \rightarrow 0$.}
    \label{fig:bound_limits}
\end{figure} 

Note that case 3 is the only possible case where $\exists \sigma_{l-1} > 0$ such that Inequality~(\ref{ineq:lowUpbound}) is satisfied. Also note that given $U(0) = 0$,  case 3 is only possible if $L^*$ is strictly greater than $U(0)=0$, i.e., $L^* > 0$. 
Therefore, using (\ref{eq:lower_limit}), we must show that 
\begin{equation}
    \sums \Gij - \sumsc |\Gij|
    e^{-\frac{1}{2\sigma_l^2}} > 0.
\end{equation}
Using Assumption 5, we know that $\sum_{i,j} \Gij = 0$, and therefore $\sums \Gij = \sumsc |\Gij|$. Therefore, we can have the following derivation:
\begin{align}
     \sums \Gij - \sumsc |\Gij|
    e^{-\frac{1}{2\sigma_l^2}} &> 0 \\
      \sums \Gij &> \sumsc |\Gij|
    e^{-\frac{1}{2\sigma_l^2}}\\   
    \sums \Gij &> e^{-\frac{1}{2\sigma_l^2}} \sumsc |\Gij|\\      
    1 &> e^{-\frac{1}{2\sigma_l^2}}       
    \label{ineq:conclusion}
\end{align}
Note that as long as $\sigma_l \ne \infty$, the strict inequality of (\ref{ineq:conclusion}) will always hold. Therefore, there exists a $\sigma_{l-1}^* > 0$ such that Inequality~(\ref{ineq:kchain_inequality}) is true.  Also note that it is only necessary to set $\sigma_{l-1}$, we do not need to tune $\sigma_l$.
\end{proof}

\subsection{Proof the existence of upper bound $U(\sigma_{l-1})$}
\begin{lemma} \label{lemma:Ubound_RHS}
There exists an upper bound $U(\sigma_{l-1})$ that is a function of $\sigma_{l-1}$ such that 
\begin{equation}
    \sum_{i,j \in \mathcal{S}\cup \mathcal{S}^{c}} \Gamma_{i,j}  r_{i}^{T}r_{j} \le U(\sigma_{l-1}). 
\end{equation}
\end{lemma}

\begin{proof}
By looking at all sample pairs, $\exists r_i^*r_j^*$ such that 
\begin{equation}
    r_i^{*^T}r_j^* \ge r_i^Tr_j \quad \forall i,j.
\end{equation}
This leads us to the following inequalities
\begin{equation}
    \sums \Gij r_i^Tr_j - \sumsc |\Gij| r_i^Tr_j \le
    \sums \Gij r_i^{*^T}r_j^* - \sumsc |\Gij| r_i^Tr_j
    \le
    \sums \Gij r_i^{*^T}r_j^*
    \label{ineq:upb_show}
\end{equation}
Therefore, we see that $\sums \Gij r_i^{*^T}r_j^*$ is an upper bound for $\sum_{i,j \in \mathcal{S}\cup \mathcal{S}^{c}} \Gamma_{i,j}  r_{i}^{T}r_{j}$. Since $r_i^*$ and $r_j^*$ are elements in RKHS from the last layer, we have 
\begin{equation}
    \langle r_{i}^*,r_{j}^* \rangle 
    = e^\frac{-|.|^2}{2\sigma_{l-1} ^2}
\end{equation}
Therefore, $\langle r_{i}^*,r_{j}^* \rangle$ is specifically a function of $\sigma_{l-1}$ which we will denote as 
    $\langle r_{i}^*(\sigma_{l-1}),r_{j}^*(\sigma_{l-1}) \rangle$. Combining this observation with Inequality~(\ref{ineq:upb_show}), we have 
\begin{align}
   \sum_{i,j \in \mathcal{S}\cup \mathcal{S}^{c}} \Gamma_{i,j}  r_{i}^{T}r_{j} 
   & \le 
   \sums \Gij 
   \langle r_{i}^*(\sigma_{l-1}),r_{j}^*(\sigma_{l-1}) \rangle \\
   &\le U(\sigma_{l-1}).
   \label{ineq:showing_upper_bound_conclusion}
\end{align} 
From (\ref{ineq:showing_upper_bound_conclusion}), we see that there exists an upper bound that is a function of $\sigma_{l-1}$. Additionally, note that as we decrease $\sigma_{l-1}$ the bound decreases and approaches 0.
\begin{equation}
    \lim_{\sigma_{l-1} \rightarrow 0}
    \sums \Gij 
    \langle r_{i}^*(\sigma_{l-1}),r_{j}^*(\sigma_{l-1}) \rangle
    =
    \lim_{\sigma_{l-1} \rightarrow 0}
    \sums \Gij 
    e^\frac{-|.|^2}{2\sigma_{l-1} ^2} = 0.
\end{equation} 
\end{proof}




\subsection{Proof the existence of Lower bound $L(\sigma_{l-1})$}
\begin{lemma} \label{lemma:Lbound_LHS}
There exists a lower bound $L(\sigma_{l-1})$ that is a function of $\sigma_{l-1}$ such that 
\begin{equation}
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW W^T(r_i-r_j)}{2\sigma_{l}^2}}
    }_\text{1st term}
    +
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^2} \Gij 
    e^{-\frac{(t_i-t_j)^TW W^T(t_i-t_j)}{2\sigma_{l}^2}}
    }_\text{2st term}   
    -
    \underbrace{
    \sum_{i,j \in \mathcal{S}^c} |\Gij| 
    e^{-\frac{(r_i-t_j)^TW W^T(r_i-t_j)}{2\sigma_{l}^2}} 
    }_\text{3rd term}
    \ge L(\sigma_{l-1}). 
    \label{ineq:exist_lower_bound}
\end{equation}
\end{lemma}

Note that to further emphasize and highlight the 2 classes, we let the samples from $\mathcal{S}^1$ be $r_i$ and samples from $\mathcal{S}^2$ be $t_i$.

\begin{proof}
We can find the lower bound for (\ref{ineq:exist_lower_bound}) by finding the upper and lower bound of the exponent for terms 1, 2 and 3. Specifically, we need to
\begin{enumerate}
    \item find the upper bound of 
    $(r_i-r_j)^TW_l W_l^T(r_i-r_j)$ for 1st term.
    \item find the upper bound of 
    $(t_i-t_j)^TW_l W_l^T(t_i-t_j)$ for 2nd term.   
    \item find the lower bound of 
    $(r_i-t_j)^TW_l W_l^T(r_i-t_j)$ for 3rd term.
\end{enumerate}

From \citelemma{lemma:Ubound_RHS}, we see that all 
$\langle r_i, r_j \rangle$ sample pairs from the last layer are functions of $\sigma_{l-1}$. Additionally, each pair is upper bounded by its largest pair where
\begin{equation}
  \langle r_i, r_j \rangle \le   
  \langle r_i^*(\sigma_{l-1}), 
  r_j ^*(\sigma_{l-1}) 
  \rangle.
\end{equation}
To simplify the notation, we here denote this upper bound on the inner product as $\mathcal{E}(\sigma_{l-1})$ where
\begin{equation}
    \mathcal{E}(\sigma_{l-1}) = 
    \langle r_i^*(\sigma_{l-1}),  r_j ^*(\sigma_{l-1}) 
  \rangle.
\end{equation}
We next note that from our assumption $W = \sum_{i\in \mathcal{S}^1}^n r_{i}$, therefore, an upper bound of the 1st term \begin{equation}
  (r_i-r_j)^TW W^T(r_i-r_j)  
\end{equation}
becomes
\begin{align}
   (r_i-r_j)^TW W^T(r_i-r_j) &=  
   (r_i-r_j)^T(\sum_{\eta \in \mathcal{S}^1}^n r_\eta) (\sum_{\eta \in \mathcal{S}^1}^n r_\eta )^T(r_i-r_j).
%   &=  
%   \left[
%    (r_i-r_j)^T(\sum_{\eta \in \mathcal{S}^1}^n r_\eta) 
%    \right]^2 \\
%    &=  
%   \left[
%    (r_i-r_j)^T(r_1 + r_2 + ...) 
%    \right]^2 \\  
%    &=  
%   \left[
%    r_i^Tr_i
%    (r_i-r_j)^T(r_1 + r_2 + ...) 
%    \right]^2 \\     
\end{align}
\textbf{1st Term lower bound. } If we look at each term carefully, we have
\begin{equation}
      r_{i}^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^T r_{i}
      + r_{j}^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^Tr_{j} - r_{i}^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^Tr_{j} -r_{j}^T (\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^Tr_{i}.
\end{equation}
By using $\mathcal{E}(\sigma_{l-1})$ as it upper bound and 0 as the lower bound of $r_i^Tr_j$, we have
\begin{align}
 (r_{i}^T r_{i} r_{i}^T r_{i} + (n-1)\mathcal{E}(\sigma_{l-1}))^2 +& (r_{j}^T r_{j} r_{j}^T r_{j} + (n-1)\mathcal{E}(\sigma_{l-1}))^2 & -r_{i}^T r_{i} r_{i}^T r_{i} & -0 & -r_{j}^T r_{j} r_{j}^T r_{j} & +0  \\ 
 (1 + (n-1)\mathcal{E}(\sigma_{l-1}))^2 +& (1 + (n-1)\mathcal{E}(\sigma_{l-1}))^2 & -1 & -0 & -1 &+  0
\end{align}
\begin{equation}
    2(1+(n-1)\mathcal{E}(\sigma_{l-1}))^2 - 2
\end{equation}
Therefore, the 1st term is lower bounded by 
\begin{equation}
      \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW W^T(r_i-r_j)}{2\sigma_l^2}} \geq 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\mathcal{E}(\sigma_{l-1}))^2 - 2 }{2\sigma_l^2}}.
\end{equation}
\textbf{2st Term lower bound. }
We next look at the exponential terms from the 2nd term. Again, by using $\mathcal{E}(\sigma_{l-1})$ and 0 as its upper and lower bound of $r_i^Tr_j$, we have
\begin{align}
      t_{i}^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^T t_{i}
      &
      + t_{j}^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^Tt_{j} 
      & - t_{i}^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^Tt_{j} 
      &
      - t_{j}^T (\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^Tt_{i} \\
      (n\mathcal{E}(\sigma_{l-1}))^2 
      &
      + (n\mathcal{E}(\sigma_{l-1}))^2 
      & - 0 & - 0.
\end{align}
Which yields a bound of
\begin{align}
 2(n\mathcal{E}(\sigma_{l-1}))^2.
\end{align}
Therefore, the 2nd term is lower bounded by 
\begin{equation}
     \sum_{i,j \in \mathcal{S}^2} \Gamma_{i,j} 
    e^{-\frac{(t_i-t_j)^TW W^T(t_i-t_j)}{2\sigma_l^2}} \geq 
    \sum_{i,j \in \mathcal{S}^2} \Gamma_{i,j} 
    e^{-\frac{2(n\mathcal{E}(\sigma_{l-1}))^2 }{2\sigma_l^2}}.
\end{equation}

\textbf{3rd Term lower bound. }
We again repeat the same process for the 3rd term. Note that here, instead of trying to find the largest combination, we want the smallest combination.
\begin{align}
    (r_i-t_j)^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^T(r_i-t_j)\\
      r_{i}^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^T r_{i}
      + t_{j}^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^Tt_{j} - r_{i}^T(\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^Tt_{j} -t_{j}^T (\sum_{i\in \mathcal{S}^1}r_{i}) (\sum_{i\in \mathcal{S}^1}r_{i})^Tr_{i}\\
      (1)^2
      + 0 
      - n\mathcal{E}(\sigma_{l-1})(1+(n-1)\mathcal{E}(\sigma_{l-1}))
      - n\mathcal{E}(\sigma_{l-1})(1+(n-1)\mathcal{E}(\sigma_{l-1}))\\
      1 - 2n\mathcal{E}(\sigma_{l-1})(1+(n-1)\mathcal{E}(\sigma_{l-1}))
\end{align}
Therefore, the 3rd term is also lower bounded such that 
\begin{equation}
   -\sum_{i,j \in \mathcal{S}^c} |\Gij| 
   e^{-\frac{(r_i-t_j)^TW W^T(r_i-t_j)}{2\sigma_{l}^2}} 
   \leq 
   - \sum_{i,j \in \mathcal{S}^c} |\Gij| 
   e^{-\frac{1 - 2n\mathcal{E}(\sigma_{l-1})(1+(n-1)\mathcal{E}(\sigma_{l-1})))}{2\sigma_{l}^2}}.
\end{equation}

\textbf{Complete lower bound. } Give the lower bound of all 3 terms, we have a lower bound for $L(\sigma_{l-1})$.
\begin{equation}
    L(\sigma_{l-1}) = 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\mathcal{E}(\sigma_{l-1}))^2 - 2 }{2\sigma_l^2}}
    + 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2(n\mathcal{E}(\sigma_{l-1}))^2 }{2\sigma_l^2}}    
    -
   \sum_{i,j \in \mathcal{S}^c} |\Gij| 
   e^{-\frac{1 - 2n\mathcal{E}(\sigma_{l-1})(1+(n-1)\mathcal{E}(\sigma_{l-1})))}{2\sigma_{l}^2}}. 
\end{equation}
From this equation, we see that a lower bound $L$ as a function of $\sigma_{l-1}$ exists. Additionally, note that
\begin{equation}
    \lim_{\sigma_{l-1} \rightarrow 0} 
    \mathcal{E}(\sigma_{l-1}) = 0.
\end{equation}
and therefore
 \begin{align}
    \lim_{\sigma_{l-1} \rightarrow 0}
    L(\sigma_{l-1}) = L^* & =  
    \sum_{i,j \in \mathcal{S}^1} \Gij
    + 
    \sum_{i,j \in \mathcal{S}^2} \Gij
    -
   \sum_{i,j \in \mathcal{S}^c} |\Gij| 
   e^{-\frac{1}{2\sigma_{l}^2}} \\
   & = 
   \sum_{i,j \in \mathcal{S}} \Gij
    -
   \sum_{i,j \in \mathcal{S}^c} |\Gij| 
   e^{-\frac{1}{2\sigma_{l}^2}} 
\end{align}

   Given this lower bound, it is a decreasing function with respect to $\sigma_{l-1}$, and consequently $\mathcal{E}(\sigma_{l-1})$. This can be seen easily by taking the derivative with respect to $\mathcal{E}$ and showing that the derivative is always < 0.
   
\begin{equation}
    L(\mathcal{E}) = 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\mathcal{E})^2 - 2 }{2\sigma_l^2}}
    + 
    \sum_{i,j \in \mathcal{S}^2} \Gamma_{i,j} 
    e^{-\frac{2(n\mathcal{E})^2 }{2\sigma_l^2}}    
    -
   \sum_{i,j \in \mathcal{S}^c} |\Gij| 
   e^{-\frac{1 - 2n\mathcal{E}(1+(n-1)\mathcal{E}(\sigma_{l-1})))}{2\sigma_{l}^2}}. 
\end{equation}  

Taking derivative for each term with respect to $\mathcal{E}$ we obtain the following:
%\begin{equation}
%    \frac{\partial}{\partial \mathcal{E}}
%    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
%    e^{-\frac{2(1+(n-1)\mathcal{E})^2 - 2 }{2\sigma_l^2}} 
%    = 
%    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
%    e^{-\frac{2(1+(n-1)\mathcal{E})^2 - 2 }{2\sigma_l^2}}   
%    \left[
%    - \frac{2(1+(n-1)\mathcal{E})(n-1)}{\sigma_l^2}
%    \right] 
%    \le 0
%\end{equation}  

\begin{align}
    \frac{\partial}{\partial \mathcal{E}}
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\mathcal{E})^2 - 2 }{2\sigma_l^2}} 
    & = 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2(1+(n-1)\mathcal{E})^2 - 2 }{2\sigma_l^2}}   
    \left[
    - \frac{2(1+(n-1)\mathcal{E})(n-1)}{\sigma_l^2}
    \right] 
    & \le 0 \\
    \frac{\partial}{\partial \mathcal{E}}
    \sum_{i,j \in \mathcal{S}^2} \Gamma_{i,j} 
    e^{-\frac{2(n\mathcal{E})^2 }{2\sigma_l^2}}    
    & = 
    \sum_{i,j \in \mathcal{S}^2} \Gamma_{i,j} 
    e^{-\frac{2(n\mathcal{E})^2 }{2\sigma_l^2}}       
    \left[
    -\frac{(n\mathcal{E})^2}{\sigma_l^2}
    \right]
    & \le 0  \\
   \frac{\partial}{\partial \mathcal{E}}
   -\sum_{i,j \in \mathcal{S}^c} |\Gij| 
   e^{-\frac{1 - 2n\mathcal{E}(1+(n-1)\mathcal{E}(\sigma_{l-1})))}{2\sigma_{l}^2}}
   & = 
   -\sum_{i,j \in \mathcal{S}^c} |\Gij| 
   e^{-\frac{1 - 2n\mathcal{E}(1+(n-1)\mathcal{E}(\sigma_{l-1})))}{2\sigma_{l}^2}}
   & \le 0.
\end{align}
It can be seen that all 3 terms are negative. This implies that as $\mathcal{E}$ increases, $L(\mathcal{E})$ is a decreasing function. Conversely, as $\mathcal{E} \rightarrow 0$,  $L(\mathcal{E})$ is an increasing function.
\end{proof}


\subsection{Extending Inequality Proof to 3 Classes}
\begin{lemma}
\label{lemma:extension_3_class}
Given $r_{i} =  f_{l-1} \circ ... \circ f_1 (x_{i})$ and $f_l = \Psi \circ \mathcal{W}_l$, there exist a sequence of $\{\sigma_{l}\}_{l\geq 1}$, $\sigma_l > 0$ such that
  \begin{equation}
    \max_{W_l} \quad
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma_{l}^2}}
    }_\text{1st term}
    -
    \underbrace{
    \sum_{i,j \in \mathcal{S}^c} |\Gij| 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma_{l}^2}} 
    }_\text{2nd term}
    \quad \geq 
    \sum_{i,j \in \mathcal{S}\cup \mathcal{S}^{c}} \Gamma_{i,j} 
    r_{i}^{T}r_{j}
    \label{ineq:kchain_inequality_3_classes}
\end{equation}
\end{lemma}

\textbf{Notations and Assumptions of the Proof. }
\begin{enumerate}
  \item $n$ is the number of samples.
  \item $\mathcal{S}$ is the set of $i,j$ sample pairs that belongs to the same class.
  \item $\mathcal{S}^c$ is the set of $i,j$ sample pairs that belongs to different classes. 
  \item We assume to only have 3 classes where the set of sample pairs from the 1st, 2nd and 3rd classes are denoted as $\mathcal{S}^1$, $\mathcal{S}^2$ and $\mathcal{S}^3$.
  \item To emphasize  the different classes, we denote samples from different classes as
  $r_i \in \cS^1$,  $t_i \in \cS^2$,  $q_i \in \cS^3$
  \item Since $\Gamma = HK_YH$, $\sum_{i,j} \Gij = 0$.
  \item To simplify the notation, we let $W = W_l$ in the proof.
  \item We let $\sigma_{l-1}$ and $\sigma_l$ be the $\sigma$ values used for the previous and current layer respectively.
  \item We assume
  \begin{equation}
        W = \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right].
  \end{equation}
  The reason why we use this instead of an optimal $W$ is that if there exists an non-optimal $W$ that satisfies the inequality, then there must also exists an optimal $W$ that satisfies the inequality. We emphasize that the goal here is to prove the existence of $W$ that satisfies the inequality.
\end{enumerate}

\textbf{Proof of the 3 class extension Lemma}
\begin{proof}
The strategy of proving 3 class is identical to the 2 class: we show that at the limit where $\sigma_{l-1} \rightarrow 0$, the lower bound limit $L^*$ is strictly greater than the Upper bound limit $U^*$ where
\begin{equation}
    L^* > U^*.
\end{equation}
For the RHS, \citelemma{lemma:Ubound_RHS} for the 2 class case  still applies to the 3 class, therefore, we have  
\begin{equation}
    \lim_{\sigma_{l-1} \rightarrow 0} 
    U(\sigma_{l-1}) = U^* = 0. 
\end{equation}

For the LHS, we show from \citelemma{lemma:Lbound_3_class_LHS} that as
$\sigma_{l-1} \rightarrow 0$, the $L^*$ becomes
\begin{align}
   \lim_{\sigma_{l-1} \rightarrow 0} 
   L(\sigma_{l-1}) = L^* 
   & = 
    \underbrace{ 
    \sums \Gij 
    }_\text{1st, 2nd, 3rd terms}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    e^{-\frac{2}{2\sigma_{l}^2}} 
    }_\text{4th term}
    \\
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{l}^2}} 
    }_\text{5th term}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{l}^2}} 
    }_\text{6th term}.       
\end{align}

Therefore, we need to show that 
\begin{equation}
    \underbrace{ 
    \sums \Gij 
    }_\text{1st, 2nd, 3rd terms}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    e^{-\frac{2}{2\sigma_{l}^2}} 
    }_\text{4th term}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{l}^2}} 
    }_\text{5th term}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{l}^2}} 
    }_\text{6th term} > 0. 
\end{equation}
\begin{equation}
    \underbrace{ 
    \sums \Gij 
    }_\text{1st, 2nd, 3rd terms}
    >
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    e^{-\frac{2}{2\sigma_{l}^2}} 
    }_\text{4th term}
    +
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{l}^2}} 
    }_\text{5th term}
    +
    \underbrace{
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{l}^2}} 
    }_\text{6th term}. 
\end{equation}
Here, we need to realize that since $\Gamma = HK_YH$, $\sum_{i,j} \Gij = 0$ and therefore we know that 
\begin{equation}
    \sums \Gij =
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    +
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    +
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
\end{equation}
Since 
\begin{equation}
    e^{-\frac{2}{2\sigma_{l}^2}} <
    e^{-\frac{1}{2\sigma_{l}^2}} \le 1
\end{equation}
the RHS term must always be smaller, and hence the inequality is satisfied.

\end{proof}


\subsection{The limit of 3 Classes Lower bound.}
\begin{lemma} \label{lemma:Lbound_3_class_LHS}
As $\sigma_{l-1} \rightarrow 0$, we have 
\begin{align}
   \lim_{\sigma_{l-1} \rightarrow 0} 
   L(\sigma_{l-1}) = &
    \underbrace{ 
    \sums \Gij 
    }_\text{1st, 2nd, 3rd terms}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    e^{-\frac{2}{2\sigma_{l}^2}} 
    }_\text{4th term}
    \\
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{l}^2}} 
    }_\text{5th term}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{l}^2}} 
    }_\text{6th term}.       
\end{align}
\end{lemma}

\begin{proof}
To find the limit of the lower bound, we let $\sigma_{l-1} = 0$ and input $W$ into the following equation
\begin{align}
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW W^T(r_i-r_j)}{2\sigma_{l}^2}}
    }_\text{1st term}
    & +
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^2} \Gij 
    e^{-\frac{(t_i-t_j)^TW W^T(t_i-t_j)}{2\sigma_{l}^2}}
    }_\text{2nd term} 
    \\
    +
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^3} \Gamma_{i,j} 
    e^{-\frac{(q_i-q_j)^TW W^T(q_i-q_j)}{2\sigma_{l}^2}}
    }_\text{3rd term} 
    & - 
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    e^{-\frac{(r_i-t_j)^TW W^T(r_i-t_j)}{2\sigma_{l}^2}} 
    }_\text{4th term}
    \\
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{(r_i-q_j)^TW W^T(r_i-q_j)}{2\sigma_{l}^2}} 
    }_\text{5th term}
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{(t_i-q_j)^TW W^T(t_i-q_j)}{2\sigma_{l}^2}} 
    }_\text{6th term}. 
    \label{ineq:exist_lower_bound_3_classes}
\end{align}


\textbf{1st Term. } If we look at the exponent of the 1st term carefully, we have
\begin{align}
    (r_i-r_j)^TW W^T(r_i-r_j)\\
    (r_i-r_j)^T
    \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right] 
        \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right]^T   
        (r_i-r_j) \\
        \left[
        \begin{bmatrix}
        1 & 0
        \end{bmatrix} - 
        \begin{bmatrix}
        1 & 0
        \end{bmatrix}       
        \right]
         \left[
        \begin{bmatrix}
        1 \\ 0
        \end{bmatrix} - 
        \begin{bmatrix}
        1 \\ 0
        \end{bmatrix}       
        \right] = 0
\end{align}

\textbf{2nd Term. } If we look at the exponent of the 2nd term carefully, we have
\begin{align}
    (t_i-t_j)^TW W^T(t_i-t_j)\\
    (t_i-t_j)^T
    \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right] 
        \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right]^T   
        (t_i-t_j) \\
        \left[
        \begin{bmatrix}
        0 & 1
        \end{bmatrix} - 
        \begin{bmatrix}
        0 & 1
        \end{bmatrix}       
        \right]
         \left[
        \begin{bmatrix}
        0 \\ 1
        \end{bmatrix} - 
        \begin{bmatrix}
        0 \\ 1
        \end{bmatrix}       
        \right] = 0
\end{align}

\textbf{3rd Term. } If we look at the exponent of the 3rd term carefully, we have
\begin{align}
    (q_i-q_j)^TW W^T(q_i-q_j)\\
    (q_i-q_j)^T
    \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right] 
        \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right]^T   
        (q_i-q_j) \\
        \left[
        \begin{bmatrix}
        0 & 0
        \end{bmatrix} - 
        \begin{bmatrix}
        0 & 0
        \end{bmatrix}       
        \right]
         \left[
        \begin{bmatrix}
        0 \\ 0
        \end{bmatrix} - 
        \begin{bmatrix}
        0 \\ 0
        \end{bmatrix}       
        \right] = 0
\end{align}

\textbf{4th Term. } If we look at the exponent of the 4th term carefully, we have
\begin{align}
    (r_i-t_j)^TW W^T(r_i-t_j)\\
    (r_i-t_j)^T
    \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right] 
        \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right]^T   
        (r_i-t_j) \\
        \left[
        \begin{bmatrix}
        1 & 0
        \end{bmatrix} - 
        \begin{bmatrix}
        0 & 1
        \end{bmatrix}       
        \right]
         \left[
        \begin{bmatrix}
        1 \\ 0
        \end{bmatrix} - 
        \begin{bmatrix}
        0 \\ 1
        \end{bmatrix}       
        \right] = 2
\end{align}

\textbf{5th Term. } If we look at the exponent of the 5th term carefully, we have
\begin{align}
    (r_i-q_j)^TW W^T(r_i-q_j)\\
    (r_i-q_j)^T
    \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right] 
        \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right]^T   
        (r_i-q_j) \\
        \left[
        \begin{bmatrix}
        1 & 0
        \end{bmatrix} - 
        \begin{bmatrix}
        0 & 0
        \end{bmatrix}       
        \right]
         \left[
        \begin{bmatrix}
        1 \\ 0
        \end{bmatrix} - 
        \begin{bmatrix}
        0 \\ 0
        \end{bmatrix}       
        \right] = 1
\end{align}

\textbf{6th Term. } If we look at the exponent of the 6th term carefully, we have
\begin{align}
    (t_i-q_j)^TW W^T(t_i-q_j)\\
    (t_i-q_j)^T
    \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right] 
        \left[\sum_{i\in \mathcal{S}^1}r_{i}, 
        \sum_{i\in \mathcal{S}^2}t_{i} \right]^T   
        (t_i-q_j) \\
        \left[
        \begin{bmatrix}
        0 & 1
        \end{bmatrix} - 
        \begin{bmatrix}
        0 & 0
        \end{bmatrix}       
        \right]
         \left[
        \begin{bmatrix}
        0 \\ 1
        \end{bmatrix} - 
        \begin{bmatrix}
        0 \\ 0
        \end{bmatrix}       
        \right] = 1
\end{align}

We next put all 6 terms together
\begin{align}
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^1} \Gij 
    }_\text{1st term}
    +
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^2} \Gij 
    }_\text{2nd term} 
    +
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    }_\text{3rd term} 
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    e^{-\frac{2}{2\sigma_{l}^2}} 
    }_\text{4th term}
    \\
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{l}^2}} 
    }_\text{5th term}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{l}^2}} 
    }_\text{6th term} \\
    \lim_{\sigma_{l-1} \rightarrow 0}
    L(\sigma_{l-1})
    =
    \underbrace{ 
    \sums \Gij 
    }_\text{1st, 2nd, 3rd terms}
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^2} |\Gij| 
    e^{-\frac{2}{2\sigma_{l}^2}} 
    }_\text{4th term}
    \\
    & -
    \underbrace{
    2\sum_{i \in \mathcal{S}^1, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{l}^2}} 
    }_\text{5th term}
    -
    \underbrace{
    2\sum_{i \in \mathcal{S}^2, j \in \mathcal{S}^3} |\Gij| 
    e^{-\frac{1}{2\sigma_{l}^2}} 
    }_\text{6th term}.    
\end{align}

\end{proof}


\begin{lemma}
\label{app:lemma:conv_to_global}.
For any $\hsic_0$, $L>1$ and $\delta>0$ there exists a sequence of kernel feature maps $\{\fm_l\}_{l=1}^L$ parameterized by $\{W_l\}_{l=1}^L$ and $\{\sigma_{l}\}_{l=1}^L$ such that as $l \rightarrow \infty$, the sequence converges to the global optimal where
    \begin{equation}
        \lim_{l \rightarrow \infty}  \hsic_l = \hsic^*,
    \end{equation}
\end{lemma}

\begin{figure}[h]
\center
    \includegraphics[width=6cm,height=3cm]{img/Two_layer_Chain.png}
    \label{app:fig:two_layer}
\end{figure} 

\begin{proof}
From \citelemma{lemma:ineq_lemma}, we know that by decreasing $\sigma_{l-1}$ towards 0, we can achieve arbitrarily close to the the lower bound of $\hsic_l$ where
\begin{equation}
    \lim_{\sigma_{l-1} \rightarrow 0}
    \hsic_l = 
    \sums \Gij - \sumsc |\Gij|
    e^{-\frac{1}{2\sigma_l^2}}. 
\end{equation}

This implies that given the control of 2 layers, by also setting $\sigma_l$ arbitrarily small we can achieve the global maximum HSIC value $\hsic^*$ where
\begin{equation}
    \lim_{\sigma_{l-1} \rightarrow 0}
    \lim_{\sigma_{l} \rightarrow 0}
    \hsic_l = \hsic^* = 
    \sums \Gij. 
\end{equation}
This proof implies that, the minimum number of layers required to achieve global optimum is 2. Therefore, any finite $L>1$ number of layers, $\hsic^*$ can be achieved. 

We emphasize that while this is theoretically possible, setting $\sigma_l$ and $\sigma_{l-1}$ too small promotes a non-smooth mapping, and in practice, it is better to use a slow monotonic improvement of $\hsic_l$ by using multiple layers and a larger $\sigma_l$.

\end{proof}




==> append3/aa_thm1_proof.tex <==
\begin{appendices} 
\section{Proof for Theorem \ref{thm:hsequence}}
\label{app:thm:hsequence}

\textbf{Theorem \ref{thm:hsequence}: }
\textit{
For any $\hsic_0$, there exists a \KS $\{\fm_{l^{\circ}}\}_{l=1}^L$ parameterized by a set of weights $W_l$ and a set of bandwidths $\sigma_l$ such that:
}
\begin{enumerate}[label=\Roman*.]
    \item 
     $\hsic_L$ can approach arbitrarily close to $\hsic^*$ such that for any $L>1$ and $\delta>0$ we can achieve
     \begin{equation}
        \hsic^{*} - \hsic_L \le \delta,
    \end{equation}   
    \item 
    as $L \rightarrow \infty$, the \RS converges to the global optimum, that is 
    \begin{equation}
        \lim_{L \rightarrow \infty}  \hsic_L = \hsic^*,
    \end{equation}       
    \item 
    the convergence is monotonic where 
    \begin{equation}
    \hsic_{l} > \hsic_{l-1} \quad \forall l.
    \end{equation}   
\end{enumerate}

\begin{lemma}
\label{app:lemma:lowerbound}
Given $\sigma_0$ and $\sigma_1$ as the $\sigma$ values from the last layer and the current layer, then there exists a lower bound for $\hsic_l$, denoted as $\lb\Lsigma$ such that 


\begin{equation}
    \hsic_l \ge \lb\Lsigma.
\end{equation}
\end{lemma}

\textbf{Basic Background, Assumptions, and Notations. }
\begin{enumerate}
    \item
    The simulation of this theorem for Adversarial and Random data is also publicly available on \url{https://github.com/anonymous}.
    \item  Here we show that this bound can be established given the last 2 layers.  
    \item  $\sigma_0$ is the $\sigma$ value of the previous layer
    \item  $\sigma_1$ is the $\sigma$ value of the current layer
    \item  $\nclass$ is the number of classes
    \item  $n$ is total number of samples
    \item  $n_i$ is number of samples in the $i^{th}$ class
    \item  $\cS$ is a set of all $i,j$ sample pairs where $r_i$ and $r_j$ belong to the same class.
    \item  $\cS^c$ is a set of all $i,j$ sample pairs where $r_i$ and $r_j$ belong to different same classes.
    \item  $\cS^{\beta}$ is a set of all $i,j$ sample pairs that belongs to the same $\beta^{th}$ classes.
    \item  $r_i^{(\alpha)}$ is the $i^{th}$ sample in the $\alpha^{th}$ class among $\nclass$ classes.
    \item  We assume no $r_i \ne r_j$ pair are equal $\forall i \ne j$. 
    \item  
    Among all $r_i \ne r_j$ pairs, there exists an optimal $r_i^*, r_j^*$ pair where  
    $\langle r_i^*, r_j^* \rangle \ge \langle r_i, r_j \rangle$ $\forall r_i \ne r^*_i$ and $r_j \ne r^*_j$. We denote this maximum inner product as 
    \begin{equation}
        \ub = \langle r_i^*, r_j^* \rangle.
    \end{equation}
    \item In \kc, each $r_i$ sample is assumed to be a sample in the RKHS of the Gaussian kernel, therefore all inner products are bounded such that
    \begin{equation}
        0 \le \langle r_i, r_j \rangle 
        \le
        \ub.
    \end{equation}
    \item We let $W$ be 
    \begin{equation}
        W_s = \frac{1}{\sqrt{\zeta}} \W.
    \end{equation}
    Instead of using an optimal $W^*$ defined as $W^{*} = \argmax_{W} H_{l}(W)$, we use a suboptimal $W_s$ where each dimension is simply the average direction of each class: $\frac{1}{\sqrt{\zeta}}$ is a normalizing constant $\zeta = ||W_{s}||_{2}^{2}$ that ensures $W_{s}^TW_{s}=I$. By using $W_s$, this implies that the $\hsic$ we obtain is already a lower bound compare $\hsic$ obtained by $W^*$. But, we will use this suboptimal $W_s$ to identify an even lower bound. Note that based on the definition $W^{*}$, we have the property $\hsic(W^{*}) \geq \hsic(W) \, \forall W$.

    \item  We note that the objective $\hsic$ is
    \begin{equation}
        \hsic = 
        \underbrace{
        \sums \Gij \ISMexpC{}{}}_{\within}
        -
        \underbrace{
        \sumsc |\Gij| \ISMexpC{}{}}_{\between}
    \end{equation}
    where we let $\within$ be the summation of terms associated with the within cluster pairs, and let $\between$ be the summation of terms associated with the between cluster pairs.
\end{enumerate}
    
    %\blue{In order to talk about the optimal solution 15 should be before the definition of optimal W and again define $\zeta = ||W||_{2}^{2}$}
    
\begin{proof} $\hspace{1pt}$
\begin{adjustwidth}{0.5cm}{0.0cm}
    The equation is divided into smaller parts organized into multiple sections.
    
    \textbf{For sample pairs in $\cS$. } The first portion of the function can be split into multiple classes where
    \begin{equation}
    \within = 
    \underbrace{
    \sum_{\cS^1} \Gij \ISMexpC{(1)}{(1)}
    }_\text{$\within_1$}
    + ... + 
    \underbrace{
    \sum_{\cS^{\nclass}} \Gij \ISMexpC{(\nclass)}{(\nclass)}}_\text{$\within_{\nclass}$}
    \end{equation}
    Realize that to find the lower bound, we need to determine the minimum possible value of each term which translates to \textbf{maximum} possible value of each exponent. Without of loss of generality we can find the lower bound for one term and generalize its results to other terms due to their similarity. Let us focus on the numerator of the exponent from $\within_1$. Given $W_s$ as $W$, our goal is identify the \textbf{maximum} possible value for
    \begin{equation}
        \underbrace{
        \rij{1}{1}^TW}_{\Pi_1}
        \underbrace{
        W^T\rij{1}{1}}_{\Pi_2}. 
    \end{equation}
    Zoom in further by looking only at $\Pi_1$, we have 
    the following relationships
    \begin{equation}
       \Pi_1 = 
        \underbrace{
            r_i^{(1)^T} W}_{\xi_1}
        - 
        \underbrace{r_j^{(1)^T} W}_{\xi_2} 
    \end{equation}
    \begin{align}
        \xi_1 & = \frac{1}{\sqrt{\zeta}} r_i^{(1)^T} \W \\
        & = \frac{1}{\sqrt{\zeta}}
            r_i^{(1)^T} 
            \begin{bmatrix}
                (r_1^{(1)} + ... + r_{n_1}^{(1)}) &
                ... &
                (r_1^{(\nclass)} + ... + r_{n_{\nclass}}^{(\nclass)})
            \end{bmatrix}
    \end{align}
    \begin{align}
        \xi_2 & = 
        \frac{1}{\sqrt{\zeta}}
        r_j^{(1)^T} \W \\
        & = 
        \frac{1}{\sqrt{\zeta}}
        r_j^{(1)^T} 
            \begin{bmatrix}
                (r_1^{(1)} + ... + r_{n_1}^{(1)}) &
                ... &
                (r_1^{(\nclass)} + ... + r_{n_{\nclass}}^{(\nclass)})
            \end{bmatrix}
    \end{align}   
    By knowing that the inner product is constrained between $[0,\ub]$, we know the maximum possible value for $\xi_1$ and the minimum possible value for $\xi_2$ to be
     \begin{align}
        \xi_1 & = 
        \frac{1}{\sqrt{\zeta}}
            \begin{bmatrix}
                1 + (n_1 - 1)\ub &
                n_2 \ub &
                n_3 \ub &
                ... &
                n_{\nclass} \ub
            \end{bmatrix} \\
         \xi_2 & = 
         \frac{1}{\sqrt{\zeta}}
            \begin{bmatrix}
                1 &
                0 &
                0 &
                ... &
                0
            \end{bmatrix}. 
    \end{align}   
    Which leads to  
    \begin{equation}
        \Pi_1 = 
        \frac{1}{\sqrt{\zeta}}
        (\xi_1 - \xi_2) = 
        \frac{1}{\sqrt{\zeta}}
            \begin{bmatrix}
                (n_1 - 1)\ub &
                n_2 \ub &
                n_3 \ub &
                ... &
                n_{\nclass} \ub
            \end{bmatrix}
    \end{equation}
    Since $\Pi_2^{T}  = \Pi_1$ we have 
    \begin{align}
        \Pi_1 \Pi_2 & = 
            \frac{1}{\zeta}
            [
            (n_1 - 1)^2\ub^2 + 
            n_2^2 \ub^2 +
            n_3^2 \ub^2 +
                ... +
            n_{\nclass}^2 \ub^2] \\
        & = 
            \frac{1}{\zeta}
            [(n_1 - 1)^2+ 
            n_2^2 +
            n_3^2 +
                ... +
            n_{\nclass}^2] \ub^2
    \end{align}
    The lower bound for just the $\within_1$ term emerges as 
    \begin{equation}
        \within_1 \ge 
        \sum_{\cS^1} \Gij e^{
        - \frac{ 
            [(n_1 - 1)^2+ 
            n_2^2 +
            n_3^2 +
                ... +
            n_{\nclass}^2] \ub^2 }{2 \zeta \sigma_1^2}}. 
    \end{equation}
    To further condense the notation, we define the following constant
    \begin{equation}
        \mathscr{N}_g = 
            \frac{1}{2 \zeta}
            [n_1^2+ 
            n_2^2 +
            ... +
            (n_g - 1)^2 + 
            ... + 
            n_{\tau}^2].
    \end{equation}
    Therefore, the lower bound for $\within_1$ can be simplified as 
    \begin{equation}
        \within_1 \ge \sum_{\cS^1} \Gij e^{-\frac{\mathscr{N}_1 \ub^2}{\sigma_1^2}}
    \end{equation}
    and the general pattern for any $\within_g$ becomes
    \begin{equation}
         \within_g \ge \sum_{\cS^i} \Gij e^{-\frac{\mathscr{N}_g \ub^2}{\sigma_1^2}}. 
    \end{equation}
    The lower bound for the entire set of $\cS$ then becomes
    \begin{equation}
        \sums \Gij \ISMexpC{}{} = 
        \within_1 + ... + \within_{\nclass} \ge 
        \underbrace{
        \sum_{g=1}^{\nclass} \sum_{\cS^g} \Gij
        e^{-\frac{\mathscr{N}_g \ub^2}{\sigma_1^2}}}_{\text{Lower bound}}.
    \end{equation}
    
    \textbf{For sample pairs in $\cS^c$. } 
    To simplify the notation, we note that
    \begin{align}
        -\between_{g_1,g_2} & = 
            -
            \sum_{i \in \cS^{g_1}} 
            \sum_{j \in \cS^{g_2}}
            |\Gij| \ISMexpC{(g_1)}{(g_2)} \\
            & = -
            \sum_{i \in \cS^{g_1}} 
            \sum_{j \in \cS^{g_2}}
            |\Gij| e^{-\frac
            {\Tr(W^T (\rij{g_1}{g_1})(\rij{g_1}{g_2})^T W)}
            {2 \sigma_1^2}} \\                
            & = -
            \sum_{i \in \cS^{g_1}} 
            \sum_{j \in \cS^{g_2}}
            |\Gij| e^{-\frac{\Tr(W^T A_{i,j}^{(g_1, g_2)} W)}
            {2 \sigma_1^2}} \\           
    \end{align}
    We now derived the lower bound for the sample pairs in $\cS^c$. We start by writing out the entire summation sequence for $\between$.  
    \begin{equation}
    \begin{split}
    \between & = 
    -\underbrace{
    \sum_{i \in \cS^1} 
    \sum_{j \in \cS^2}
    |\Gij| 
    e^{-\frac{\Tr(W^T A_{i,j}^{(1, 2)} W)}
    {2 \sigma_1^2}}
    }_\text{$\between_{1,2}$} 
    - \underbrace{...}_{\between_{g_1 \ne g_2}}
    -\underbrace{
    \sum_{i \in \cS^1} 
    \sum_{j \in \cS^{\nclass}}
    |\Gij| 
    e^{-\frac{\Tr(W^T A_{i,j}^{(1, \nclass)} W)}
    {2 \sigma_1^2}}
    }_\text{$\between_{1,\nclass}$} 
    \\
    & 
    -\underbrace{
    \sum_{i \in \cS^2} 
    \sum_{j \in \cS^1}
    |\Gij| 
    e^{-\frac{\Tr(W^T A_{i,j}^{(2, 1)} W)}
    {2 \sigma_1^2}}
    }_\text{$\between_{2,1}$} 
    - \underbrace{...}_{\between_{g_1 \ne g_2}}
    -\underbrace{
    \sum_{i \in \cS^2} 
    \sum_{j \in \cS^{\nclass}}
    |\Gij| 
    e^{-\frac{\Tr(W^T A_{i,j}^{(2, \nclass)} W)}
    {2 \sigma_1^2}}
    }_\text{$\between_{2,\nclass}$} 
    \\   
    & ... \\
    & 
    -\underbrace{
    \sum_{i \in \cS^\nclass} 
    \sum_{j \in \cS^1}
    |\Gij| 
    e^{-\frac{\Tr(W^T A_{i,j}^{(\nclass, 1)} W)}
    {2 \sigma_1^2}}
    }_\text{$\between_{\nclass,1}$} 
    - \underbrace{...}_{\between_{g_1 \ne g_2}}
    -\underbrace{
    \sum_{i \in \cS^{\nclass-1}} 
    \sum_{j \in \cS^{\nclass}}
    |\Gij| 
    e^{-\frac{\Tr(W^T A_{i,j}^{(\nclass-1, \nclass)} W)}
    {2 \sigma_1^2}}
    }_\text{$\between_{\nclass-1,\nclass}$} 
    \end{split}
    \end{equation}
    
    Using a similar approach with the terms from $\within$, note that $\between$ is a negative value, so we need to maximize this term to obtain a lower bound. Consequently, the key is to determine the \textbf{minimal} possible values for each exponent term. Since every one of them will behave very similarly, we can simply look at the numerator of the exponent from $\between_{1,2}$ and then arrive to a more general conclusion. Given $W_s$ as $W$, our goal is to identify the \textbf{minimal} possible value for
    \begin{equation}
        \underbrace{
        \rij{1}{2}^TW}_{\Pi_1}
        \underbrace{
        W^T\rij{1}{2}}_{\Pi_2}. 
    \end{equation}
  
    Zoom in further by looking only at $\Pi_1$, we have 
    the following relationships
    \begin{equation}
       \Pi_1 = 
        \underbrace{
            r_i^{(1)^T} W}_{\xi_1}
        - 
        \underbrace{r_j^{(2)^T} W}_{\xi_2} 
    \end{equation}
    \begin{align}
        \xi_1 & = 
        \frac{1}{\sqrt{\zeta}}
        r_i^{(1)^T} \W \\
        & = 
        \frac{1}{\sqrt{\zeta}}
        r_i^{(1)^T} 
            \begin{bmatrix}
                (r_1^{(1)} + ... + r_{n_1}^{(1)}) &
                ... &
                (r_1^{(\nclass)} + ... + r_{n_{\nclass}}^{(\nclass)})
            \end{bmatrix}
    \end{align}
    \begin{align}
        \xi_2 & = 
        \frac{1}{\sqrt{\zeta}}
        r_j^{(2)^T} \W \\
        & = 
        \frac{1}{\sqrt{\zeta}}
        r_j^{(2)^T} 
            \begin{bmatrix}
                (r_1^{(1)} + ... + r_{n_1}^{(1)}) &
                ... &
                (r_1^{(\nclass)} + ... + r_{n_{\nclass}}^{(\nclass)})
            \end{bmatrix}
    \end{align}   
    By knowing that the inner product is constrained between $[0,\ub]$, we know the \textbf{minimum} possible value for $\xi_1$ and the \textbf{maximum} possible value for $\xi_2$ to be
     \begin{align}
        \xi_1 & = 
            \frac{1}{\sqrt{\zeta}}
            \begin{bmatrix}
                1 &
                0 &
                0 &
                ... &
                0
            \end{bmatrix} \\
         \xi_2 & = 
            \frac{1}{\sqrt{\zeta}}
            \begin{bmatrix}
                n_1\ub &
                1 + (n_2 - 1) \ub &
                n_3 \ub &
                ... &
                n_{\nclass} \ub
            \end{bmatrix} 
    \end{align}   
    Which leads to  
    \begin{equation}
        \Pi_1 = 
        \frac{1}{\sqrt{\zeta}}
        (\xi_1 - \xi_2) = 
            \frac{1}{\sqrt{\zeta}}
            \begin{bmatrix}
                1 - n_1\ub &
                -(1 + (n_2 - 1) \ub) &
                -n_3 \ub &
                ... &
                -n_{\nclass} \ub
            \end{bmatrix}
    \end{equation}
    Since $\Pi_2^{T}  = \Pi_1$ we have     
    \begin{align}
        \Pi_1 \Pi_2 & = 
            \frac{1}{\zeta}
            [
            (1- n_1 \ub)^2 + 
            (1 + (n_2-1)\ub)^2 + 
            n_3^2 \ub^2 +
                ... +
            n_{\nclass}^2 \ub^2].
    \end{align}
    The lower bound for just the $\between_{1,2}$ term emerges as 
    \begin{equation}
        -\between_{1,2} \ge 
        - \sum_{\cS^1} \sum_{\cS^2} |\Gij| e^{
        - \frac{ 
            (1- n_1\ub)^2 + 
            (1 + (n_2-1)\ub)^2 + 
            n_3^2 \ub^2 +
                ... +
            n_{\nclass}^2 \ub^2}
            {2 \zeta \sigma_1^2}}. 
    \end{equation}
    To further condense the notation, we define the following function
    \begin{equation}
    \begin{split}
        \mathscr{N}_{g_1, g_2}(\ub) & = 
            \frac{1}{2 \zeta}
            [ n_1^2 \ub^2 + n_2^2 \ub^2 + ... \\ 
            & +  (1- n_{g_1}\ub)^2 + ... + 
            (1 + (n_{g_2}-1)\ub)^2 \\
            & + ...  + n_{\tau}^2 \ub^2].
    \end{split}
    \end{equation}
    Note that while for $\cS$, the $\ub$ term can be separated out. But here, we cannot, and therefore $\mathscr{N}$ here must be a function of $\ub$.  Therefore, the lower bound for $\between_{1,2}$ can be simplified into
    \begin{equation}
        - \between_{1,2} \ge - 
        \sum_{\cS^1} 
        \sum_{\cS^2}
        |\Gij| e^{-\frac{\mathscr{N}_{1,2}(\ub)}{\sigma_1^2}}
    \end{equation}
    and the general pattern for any $\between_{g_1, g_2}$ becomes
    \begin{equation}
         -\between_{g_1,g_2} \ge -
         \sum_{\cS^{g1}} 
        \sum_{\cS^{g2}}
         \Gij e^{-\frac{\mathscr{N}_{g_1,g_2}(\ub)}
         {\sigma_1^2}}. 
    \end{equation}    
    The lower bound for the entire set of $\cS^c$ then becomes
    \begin{align}
        -\sumsc |\Gij| \ISMexpC{}{} & = 
        - \between_{1,2} 
        - \between_{1,3} 
        - ... - 
        \between_{\nclass-1, \nclass} \\
        & \ge 
        - \underbrace{
        \sum_{g_1 \ne g_2}^{\nclass}
        \sum_{i \in \cS^{g_1}} 
        \sum_{j \in \cS^{g_2}} 
        |\Gij|
        e^{-\frac{\mathscr{N}_{g_1,g_2} (\ub)}{\sigma_1^2}}}_{\text{Lower bound}}.
    \end{align}    
    
    \textbf{Putting $\cS$ and $\cS^c$ Together. } 
    \begin{align}
        \hsic & = \within + \between    \\
        & \ge
        \underbrace{
        \sum_{g=1}^{\nclass} \sum_{\cS^g} \Gij
        e^{-\frac{\mathscr{N}_g \ub^2}{\sigma_1^2}}}_{\text{Lower bound of } \within}
        - \underbrace{
        \sum_{g_1 \ne g_2}^{\nclass} 
        \sum_{i \in \cS^{g_1}} 
        \sum_{j \in \cS^{g_2}} 
        |\Gij|
        e^{-\frac{\mathscr{N}_{g_1,g_2} (\ub)}{\sigma_1^2}}}_{\text{Lower bound of } \between}.
    \end{align}
    Therefore, we have identified a lower bound that is a function of $\sigma_0$ and $\sigma_1$ where
    \begin{equation}
        \lb\Lsigma = 
        \sum_{g=1}^{\tau} \sum_{\cS^g} \Gij
        e^{-\frac{\mathscr{N}_g \ub^2}{\sigma_1^2}}
        - 
        \sum_{g_1 \ne g_2}^{\tau} 
        \sum_{i \in \cS^{g_1}} 
        \sum_{j \in \cS^{g_2}} 
        |\Gij|
        e^{-\frac{\mathscr{N}_{g_1,g_2} (\ub)}{\sigma_1^2}}.
    \end{equation}
    From the lower bound, it is obvious why it is a function of $\sigma_1$. The lower bound is also a function of $\sigma_{0}$ because $\ub$ is actually a function of $\sigma_0$. To specifically clarify this point, we have the next lemma. 
\end{adjustwidth}
\end{proof}
\hspace{1pt}

\begin{lemma}
\label{app:lemma:ub_goes_to_zero}
The $\ub$ used in \citelemma{app:lemma:lowerbound} is a function of $\sigma_0$ where $\ub$ approaches to zero as $\sigma_{0}$ approaches to zero, i.e.
\begin{equation}
    \lim_{\sigma_0 \rightarrow 0}  
    \ub = 0.
\end{equation}
\end{lemma}

\textbf{Assumptions and Notations. }
\begin{enumerate}
    \item  
        We use Fig.~\ref{app:fig:two_layer_img} to help clarify the notations. We here only look at the last 2 layers.  
    \item  
        We let $\hsic_0$ be the $\hsic$ of the last layer, and $\hsic_1$, the $\hsic$ of the current layer.
    \item
        The input of the data is $X$ with each sample as $x_i$, and the output of the previous layer are denoted as $r_i$. $\psi_{\sigma_0}$ is the feature map of the previous layer using $\sigma_0$ and $\psi_{\sigma_1}$ corresponds to the current layer. 
        \begin{figure}[h]
        \center
            \includegraphics[width=7cm]{img/TwoLayer.png}
            \caption{Figure of a 2 layer network.}
            \label{app:fig:two_layer_img}
        \end{figure}     
    \item  
        As defined from \citelemma{app:lemma:lowerbound}, 
        among all $r_i \ne r_j$ pairs, there exists an optimal $r_i^*, r_j^*$ pair where   $\langle r_i^*, r_j^* \rangle \ge \langle r_i, r_j \rangle$ $\forall r_i \ne r^*_i$ and $r_j \ne r^*_j$. We denote this maximum inner product as 
    \begin{equation}
        \ub = \langle r_i^*, r_j^* \rangle.
    \end{equation}
\end{enumerate}



\begin{proof} \hspace{1pt}
\begin{adjustwidth}{0.5cm}{0.0cm}
Given Fig.~\ref{app:fig:two_layer_img}, the equation for $\hsic_0$ is 
\begin{align}
    \hsic_0 
        & = \sums \Gij 
        e^{-\frac{(x_i - x_j)^TW W^T (x_i - x_j)}{2 \sigma_0^2}}
        -
        \sumsc |\Gij| 
        e^{-\frac{(x_i - x_j)^TW W^T (x_i - x_j)}{2 \sigma_0^2}}    \\
        & = 
        \sums \Gij
            \langle 
                \psi_{\sigma_0}(x_i), 
                \psi_{\sigma_0}(x_j)
            \rangle
            - \sumsc |\Gij|
            \langle 
                \psi_{\sigma_0}(x_i), 
                \psi_{\sigma_0}(x_j)
            \rangle
\end{align}
Notice that as $\sigma_0 \rightarrow 0$, we have 
\begin{equation}
    %\label{eq:converged_kernel}
    \lim_{\sigma_0 \rightarrow 0} 
    \langle 
        \psi_{\sigma_0}(x_i), 
        \psi_{\sigma_0}(x_j)
    \rangle   
    =  
    \begin{cases} 
    0 \quad \forall i \ne j
    \\
    1 \quad \forall i = j
    \end{cases}.
\end{equation}
In other words, as $\sigma_0 \rightarrow 0$, the samples $r_i$ in the RKHS of a Gaussian kernel approaches orthogonal to all other samples. Given this fact, it also implies that the $\sigma_0$ controls the inner product magnitude in RKHS space  of the maximum sample pair $r_i^*, r_j^*$. We define this maximum inner product as
\begin{equation}
    \langle 
        \psi_{\sigma_0}(x_i^*), 
        \psi_{\sigma_0}(x_j^*)
    \rangle  
    \ge 
     \langle 
        \psi_{\sigma_0}(x_i), 
        \psi_{\sigma_0}(x_j)
    \rangle      
\end{equation}
or equivalently
\begin{equation}
    \langle 
        r_i^*, 
        r_j^*
    \rangle  
    \ge 
     \langle 
        r_i,
        r_j
    \rangle      
\end{equation}

Therefore, given a $\sigma_0$, it controls the upper bound of the inner product. Notice that as $\sigma_0 \rightarrow 0$, every sample in RKHS becomes orthogonal. Therefore, the upper bound of $\langle r_i, r_j \rangle$ also approaches 0 when $r_i \ne r_j$. From this, we see the relationship
\begin{equation}
    \lim_{\sigma_0 \rightarrow 0} 
    \ub = \lim_{\sigma_0 \rightarrow 0}  \exp -(|.|/\sigma^{2}_{0}) = 0
\end{equation}, where |.| is bounded and has a minimum and maximum, because we have finite number of samples.
\end{adjustwidth}
\end{proof}





\begin{lemma}
%\label{app:lemma:ub_goes_to_zero}
\label{app:lemma:as_ub_zero_L_approaches}
Given any fixed $\sigma_1 > 0 $, the lower bound $\lb\Lsigma$ is a function with respect to $\sigma_0$ and as $\sigma_0 \rightarrow 0$, $\lb\Lsigma$ approaches the function
    \begin{equation}
        \lb(\sigma_1) = 
        \sum_{g=1}^{\nclass} \sum_{\cS^g} \Gij
        - 
        \sum_{g_1 \ne g_2}^{\nclass}
        \sum_{i \in \cS^{g_1}} 
        \sum_{j \in \cS^{g_2}} 
        |\Gij|
        e^{-\frac{1}{\zeta \sigma_1^2}}.
    \end{equation}
At this point, if we let $\sigma_1 \rightarrow 0$, we have 
    \begin{align}
        \lim_{\sigma_1 \rightarrow 0}
        \lb(\sigma_1) & = \sums \Gij \\
        & = \hsic^*.
    \end{align}
\end{lemma}

\begin{proof} \hspace{1pt}
\begin{adjustwidth}{0.5cm}{0.0cm}
    Given \citelemma{app:lemma:ub_goes_to_zero}, we know that 
     \begin{equation}
        \lim_{\sigma_0 \rightarrow 0} 
        \ub = 0.
    \end{equation}   
    Therefore, having $\sigma_0 \rightarrow 0$ is equivalent to having $\ub \rightarrow 0$. Since 
    \citelemma{app:lemma:lowerbound} provide the equation of a lower bound that is a function of $\ub$,  this lemma is proven by simply evaluating $\lb\Lsigma$ as $\ub \rightarrow 0$. Following these steps, we have
    \begin{align}
        \lb(\sigma_1) & = 
        \lim_{\ub \rightarrow 0}
        \sum_{g=1}^{\nclass} \sum_{\cS^g} \Gij
        e^{-\frac{\mathscr{N}_g \ub^2}{\sigma_1^2}}
        - 
        \sum_{g_1 \ne g_2}^{\nclass} 
        \sum_{i \in \cS^{g_1}} 
        \sum_{j \in \cS^{g_2}} 
        |\Gij|
        e^{-\frac{\mathscr{N}_{g_1,g_2} (\ub)}{\sigma_1^2}}, \\
        & = 
        \sum_{g=1}^{\nclass} \sum_{\cS^g} \Gij
        - 
        \sum_{g_1 \ne g_2}^{\nclass} 
        \sum_{i \in \cS^{g_1}} 
        \sum_{j \in \cS^{g_2}} 
        |\Gij|
        e^{-\frac{1}{\zeta \sigma_1^2}}.
    \end{align}    
At this point, as $\sigma_1 \rightarrow 0$, our lower bound reaches the global maximum 
    \begin{align}
        \lim_{\sigma_1 \rightarrow 0}
        \lb(\sigma_1) & = \sum_{g=1}^{\nclass} \sum_{\cS^g} \Gij
        = \sums \Gij \\
        & = \hsic^*.
    \end{align}
    
%Additionally, $\lb\Lsigma$ is a decreasing function with respect to $\ub$. This can be seen by taking the derivative of $\lb\Lsigma$ with respect to $\ub$. 
%\begin{equation}
%    \frac{\partial}{\partial \ub} 
%        \sum_{g=1}^c \sum_{\cS^g} \Gij
%        e^{-\frac{\mathscr{N}_g \ub^2}{\sigma_1^2}}
%        - 
%        \sum_{g_1 \ne g_2}^c 
%        \sum_{i \in \cS^{g_1}} 
%        \sum_{j \in \cS^{g_2}} 
%        |\Gij|
%        e^{-\frac{\mathscr{N}_{g_1,g_2} (\ub)}{\sigma_1^2}}.    
%\end{equation}
%\begin{equation}
%        - 2
%        \sum_{g=1}^c \sum_{\cS^g} \Gij
%        e^{-\frac{\mathscr{N}_g \ub^2}{\sigma_1^2}}
%        \left(
%        \frac{\mathscr{N}_g}{\sigma_1^2}
%        \right) \ub
%        - 
%        \sum_{g_1 \ne g_2}^c 
%        \sum_{i \in \cS^{g_1}} 
%        \sum_{j \in \cS^{g_2}} 
%        |\Gij|
%        e^{-\frac{\mathscr{N}_{g_1,g_2} (\ub)}{\sigma_1^2}}.    
%\end{equation}
\end{adjustwidth}
\end{proof}

\begin{lemma}
%%\label{app:lemma:ub_goes_to_zero}
%%\label{app:lemma:as_ub_zero_L_approaches}
\label{app:lemma:arbitrarily_close}
Given any $\hsic_{l-2}$, $\delta > 0$, there exists a $\sigma_0 > 0 $ and $\sigma_1 > 0$ such that
\begin{equation}
        \hsic^{*} - \hsic_l \le \delta.
        \label{app:eq:proof_I}
\end{equation}
\end{lemma}
\begin{proof} $\hspace{1pt}$


\begin{adjustwidth}{0.5cm}{0.0cm}
\textbf{Observation 1. }

Note that the objective of $\hsic_l$ is
\begin{equation}
\begin{split}
    \hsic_l = 
    \max_W
    &
    \sums \Gij 
    e^{-\frac{\rij{\cS}{\cS}^T WW^T \rij{\cS}{\cS}}{2\sigma_1^2}} \\
    - & \sumsc |\Gij| 
     e^{-\frac{\rij{\cS^c}{\cS^c}^T WW^T \rij{\cS^c}{\cS^c}}{2\sigma_1^2}}.
\end{split}
\end{equation}
Since the Gaussian kernel is bounded between 0 and 1, the theoretical maximum of $\hsic^*$ is when the kernel is 1 for $\cS$ and 0 for $\cS^c$ with the theoretical maximum as $\hsic^* = \sums \Gij$. Therefore \eq{app:eq:proof_I} inequality is equivalent to 
\begin{equation}
        \sums \Gij - \hsic_l \le \delta.
\end{equation}
\end{adjustwidth}


%\begin{adjustwidth}{0.5cm}{0.0cm}
%\textbf{Observation 2. }
%
%According to \citelemma{app:lemma:lowerbound}, there exists a lower bound for $\hsic_l$ that is a function of $\sigma_0$ and $\sigma_1$ denoted as $\lb\Lsigma$. Therefore, we have the following logic 
%\begin{equation}
%        \sums \Gij - \lb\Lsigma \le \delta \implies
%        \sums \Gij - \hsic_l \le \delta.
%\end{equation}
%That is, proving $\sums \Gij - \lb\Lsigma \le \delta$ is sufficient to prove this lemma. Moreoever, \citelemma{app:lemma:as_ub_zero_L_approaches} demonstrates the following properties for $\lb\Lsigma$:
%\begin{enumerate}
%    \item 
%    As $\sigma_0 \rightarrow 0$, the lower bound approaches a specific function $\lb(\sigma_1)$
%    \begin{equation}
%        \lb(\sigma_1) = 
%        \sum_{g=1}^{\nclass} \sum_{\cS^g} \Gij
%        - 
%        \sum_{g_1 \ne g_2}^{\nclass} 
%        \sum_{i \in \cS^{g_1}} 
%        \sum_{j \in \cS^{g_2}} 
%        |\Gij|
%        e^{-\frac{2}{\sigma_1^2}}.
%    \end{equation}    
%    %\item
%    %    $\lb\Lsigma$ is a decreasing function with respect to $\sigma_0$ and $\sigma_1$.    
%    \item
%    As $\sigma_1 \rightarrow 0$, $\lb^*(\sigma_1)$ approaches to $\hsic^*$
%    \begin{equation}
%        \lim_{\sigma_1 \rightarrow 0}
%        \lb^*(\sigma_1) = \sums \Gij = \hsic^*.
%    \end{equation}
%\end{enumerate}
%Therefore, by decreasing $\sigma_0$ and $\sigma_1$, we can reach arbitrarily close to the global optimal. \blue{this is wrong you don't need observation 2 you can just prove observation 3.}
%\begin{equation}
%    \sums \Gij - 
%    \lim_{\sigma_0 \rightarrow 0} 
%    \lim_{\sigma_1 \rightarrow 0}
%    \lb\Lsigma = \sums \Gij - \sums \Gij = 0.
%\end{equation}
%\end{adjustwidth}


\begin{adjustwidth}{0.5cm}{0.0cm}
\textbf{Observation 2. }

If we choose a $\sigma_0$ such that 


\begin{equation}
    \lb^*(\sigma_1) - \lb\Lsigma \le \frac{\delta}{2}
    \quad \text{and} \quad
    \hsic^* - \lb^*(\sigma_1) \le \frac{\delta}{2}
\end{equation}
then we have identified the condition where $\sigma_0 > 0$ and $\sigma_1 > 0$ such that
\begin{equation}
    \sums \Gij - \lb\Lsigma \le \delta.
\end{equation}
Note that the $\lb^*(\sigma_1)$ is a continuous function of $\sigma_1$. Therefore, a $\sigma_1$ exists such that $\lb^*(\sigma_1)$ can be set arbitraty close to $\hsic^{*}$. Hence, we choose an $\sigma_{1}$ that has the following property:
\begin{equation}
    \hsic^* - \lb^*(\sigma_1) \le \frac{\delta}{2}.
\end{equation}
We next fix $\sigma_{1}$, we also know $\lb\Lsigma$ is a continuous function of $\sigma_{0}$, and it has a limit $\lb^*(\sigma_1)$ as $\sigma_{0}$ approaches to 0, hence there exits a $\sigma_{0}$, where 
\begin{equation}
    \lb^*(\sigma_1) - \lb\Lsigma \le \frac{\delta}{2}
\end{equation}
Then we have:
\begin{equation}
    \lb^*(\sigma_1) - \lb\Lsigma \le \frac{\delta}{2}
    \quad \text{and} \quad
    \hsic^* - \lb^*(\sigma_1) \le \frac{\delta}{2}.
\end{equation}
By adding the two $\frac{\delta}{2}$, we conclude the proof.
\end{adjustwidth}
\end{proof}




%\begin{adjustwidth}{0.0cm}{0.0cm}
%\begin{lemma}
%    \label{app:lemma:approach_optimal_H}
%    There exists a \KS $\{\fm_{l^{\circ}}\}_{l=1}^L$ parameterized by a set of weights $W_l$ and a set of bandwidths $\sigma_l$ such that    
%    \begin{equation}
%        \lim_{l \rightarrow \infty}  \hsic_l = \hsic^*.
%    \end{equation}
%\end{lemma}
%\end{adjustwidth}
%
%Before, the proof, we use the following figure to illustrate the relationship between \KS $\{\phi_{l^\circ}\}_{l=1}^L$ that generates the \RS $\{\hsic_l\}_{l=1}^L$. By solving a network greedily, we separate the network into $L$ separable problems. At each additional layer, we rely on the weights learned from the previous layer. At each network, we find $\sigma_{l-1}$, $\sigma_l$, and $W_l$ for the next network.
%        \begin{figure}[h]
%        \center
%            \includegraphics[width=7cm]{img/kchain_layers.png}
%            \caption{Relating \KS to \RS.}
%            \label{app:fig:all_layers}
%        \end{figure} 
%        
%\begin{proof} $\hspace{1pt}$
%\begin{adjustwidth}{0.5cm}{0.0cm}
%We first note that from \citelemma{app:lemma:arbitrarily_close}, we have previously proven that given 2 layers and any $\delta > 0$, we can achieve
%\begin{equation}
%    \hsic^{*} - \hsic_{l} \leq \delta.
%\end{equation}
%This implies that based on Fig.~\ref{app:fig:all_layers}, at any given layer, we could reach arbitrarily close to $\hsic^*$. Therefore, if we construct a Kernel sequence $\{\hsic_{l}\}_{l=1}^\infty$, where $\delta_{l} = \frac{\hsic^* - \hsic_0}{l}$ such that 
%\begin{equation}
%    \forall l>0: \hsic^{*} - \hsic_{l} \leq \delta_{l}
%\end{equation}
%then this construction is sufficient to show that 
%\begin{equation}
%   \lim_{l \rightarrow \infty}  \hsic_l = \hsic^*
%\end{equation}
%
% because as $l \rightarrow \infty$, we have the condition
% \begin{equation}
%     \hsic^* - \hsic_l \le 0.
% \end{equation}
%\end{adjustwidth}
%\end{proof}
%
%\begin{lemma}
%    There exists a $\sigma_{l-1}$ and $\sigma_l$ such that convergence is monotonic where
%    \begin{equation}
%    \hsic_{l} > \hsic_{l-1} \quad \forall l.
%    \end{equation}
%\end{lemma}
%\begin{proof}
% Given the proof from \citelemma{app:lemma:approach_optimal_H}, each layer we have
%\begin{equation}
%    \hsic^* - \hsic_l \le \frac{\hsic^* - \hsic_0}{l}.     
%\end{equation} 
%Since $\frac{\hsic^* - \hsic_0}{l}$ decreases as $l$ increase, then at each layer, we have the condition
%\begin{equation}
%    \hsic_{l+1} > \hsic_l.
%\end{equation}
%
%\end{proof}

\begin{lemma}
    \label{app:lemma:approach_optimal_H1}
    There exists a \KS $\{\fm_{l^{\circ}}\}_{l=1}^L$ parameterized by a set of weights $W_l$ and a set of bandwidths $\sigma_l$ such that    
    \begin{equation}
        \lim_{l \rightarrow \infty}  \hsic_l = \hsic^* , \quad \hsic_{l+1} > \hsic_l \quad \forall l
    \end{equation}
\end{lemma}


Before, the proof, we use the following figure, Fig.~\ref{app:fig:all_layers}, to illustrate the relationship between \KS $\{\phi_{l^\circ}\}_{l=1}^L$ that generates the \RS $\{\hsic_l\}_{l=1}^L$. By solving a network greedily, we separate the network into $L$ separable problems. At each additional layer, we rely on the weights learned from the previous layer. At each network, we find $\sigma_{l-1}$, $\sigma_l$, and $W_l$ for the next network. We also note that since we only need to prove the existence of a solution, this proof is done by \textit{\textbf{Proof by Construction}}, i.e, we only need to show an example of its existence. Therefore, this proof consists of us constructing a \RS which satisfies the lemma.
        \begin{figure}[h]
        \center
            \includegraphics[width=7cm]{img/kchain_layers.png}
            \caption{Relating \KS to \RS.}
            \label{app:fig:all_layers}
        \end{figure} 

\begin{proof} \hspace{1pt}
\begin{adjustwidth}{0.5cm}{0.0cm}
We first note that from \citelemma{app:lemma:arbitrarily_close}, we have previously proven given any $\hsic_{l-2}$, $\delta > 0$, there exists a $\sigma_0 > 0 $ and $\sigma_1 > 0$ such that
\begin{equation}
    \hsic^{*} - \hsic_{l} \leq \delta_{l}.
    \label{eq:cond1}
\end{equation}
This implies that based on Fig.~\ref{app:fig:all_layers}, at any given layer, we could reach arbitrarily close to $\hsic^*$. Given this, we list the 2 steps to build the \RS.

%\textbf{Step 1: }
%We first assumes that at each layer, we select the appropriate $\sigma$ values such that it guarantees  \eq{eq:cond1} is always true.



\textbf{Step 1: } Define $\{\mathcal{E}_{n}\}_{n =  1}^{\infty}$ as a sequence of numbers $\hsic^{*} - \frac{\hsic^{*} - \hsic_0}{n}$ on the real line. We have the following properties for this sequence:
\begin{equation}
  \lim_{n\rightarrow\infty} \mathcal{E}_{n} = \hsic^{*}
 , \quad \mathcal{E}_{1} = \mathcal{H}_{0}.   
\end{equation}


Using these two properties, for any $\hsic_{l-1} \in [\hsic_{0},\hsic^{*}]$ there exist an unique $n$, where  \begin{equation}
    \mathcal{E}_{n} \leq \hsic_{l-1} < \mathcal{E}_{n+1}.
    \label{eq:bounding_box}
\end{equation}

\textbf{Step 2: }  
%At step $l$, let $m$ be the number that satisfies 
%\begin{equation}
%\mathcal{E}_{m} \leq \hsic_{l-1} <  \mathcal{E}_{m+1},
%\end{equation}
%Therefore, we know that 
%\begin{equation}
%\mathcal{E}_{m} <  \mathcal{E}_{m+1}.
%\end{equation}
%Also let us define $\delta_l$ as
%\begin{equation}
%    \delta_{l} = \hsic^{*} - \mathcal{E}_{m+1}.
%    \label{eq:define_delta}
%\end{equation}
%Under this construction, the following inequality is always true.
%\begin{equation}
%    \delta_{l} \leq \hsic^{*} - \mathcal{E}_m.
%\end{equation}
%This inequality becomes clear given Fig.~\ref{app:fig:differential} below.
%        \begin{figure}[h]
%        \center
%            \includegraphics[width=10cm]{img/diff.png}
%            \caption{}
%            \label{app:fig:differential}
%        \end{figure} 
%    Moreover, with this construction, sequence $\{\delta_{l}\}$ is strictly decreasing sequence. i.e. $\delta_{l} > \delta_{l+1}$ and $\lim_{l \rightarrow \infty} \delta_{l} = 0$. 
    For any given $l$, we choose $\delta_{l}$ to satisfies \eq{eq:cond1} by the following procedure, First find an $n$ that satisfies
    \begin{equation}
        \mathcal{E}_{n} \leq \hsic_{l-1} <  \mathcal{E}_{n+1}, 
        \label{ineq:differential}
    \end{equation}
    and second define $\delta_l$ to be 
    \begin{equation}
        \delta_{l} = \hsic^{*} - \mathcal{E}_{n+1}.
        \label{eq:delta_define}
    \end{equation}
    
%    Following this construction, the following statements must be true
%   
%    \begin{align}
%        %\delta_{l-1} 
%        %& \ge \hsic^* - \hsic_{l-1}
%        %& \text{Or it would violate Step 1.} \\
%        \delta_{l-1} 
%        & \ge \hsic^* - \mathcal{E}_n
%        & \text{Given definition \eq{eq:delta_define}.}\\
%        \hsic^* - \mathcal{E}_n & \ge \hsic^* - \hsic_{l-1}
%        & \text{Given definition \eq{eq:bounding_box}.}
%    \end{align}
    
%    this implies that at $\hsic_{l-1}$, we have 
%    \begin{equation}
%        \delta_{l-1} \ge 
%        \hsic^* - \mathcal{E}_n \ge
%        \hsic^* - \hsic_{l-1}.
%        \label{eq:last_delta}
%    \end{equation}
    

%    From \eq{ineq:differential}, its obvious that 
%    \begin{equation}
%        \mathcal{E}_{n} <  \mathcal{E}_{n+1}.
%    \end{equation}   
%    Therefore, we have the relationship
%    \begin{align}
%        \mathcal{E}_{n} & <  \mathcal{E}_{n+1} \\
%        -\mathcal{E}_{n} & >  -\mathcal{E}_{n+1} \\
%        \hsic^* - \mathcal{E}_{n} 
%        & >  
%        \hsic^* - \mathcal{E}_{n+1} \\
%        \delta_{l-1} \ge
%        \hsic^* - \mathcal{E}_{n} 
%        & >  
%        \hsic^* - \mathcal{E}_{n+1} 
%        & \text{Applying \eq{eq:last_delta}.}
%        \\       
%        \delta_{l-1} & >  \delta_{l} & 
%        \text{Follow definition \eq{eq:delta_define}.}
%        \label{eq:mono_decrease_delta}
%    \end{align}      
%    From \eq{eq:mono_decrease_delta}, we see that $\{ \delta_n \}$ is a monotonically decreasing sequence.
    
    
%    \blue{
%    Based on the definition of $\delta_{l-1}$, where 
%    $\delta_{l-1} = \hsic^{*} - \mathcal{E}_{n}$, the following inequality must be true where}
To satisfy \eq{eq:cond1}, the following must be true.  \begin{equation}
    \hsic^{*} - \hsic_{l-1} \leq \delta_{l-1}.
    \label{eq:delta_greater_than_l1}
\end{equation}
and further we found $n$ such that
\begin{equation}
    \mathcal{E}_{n} \leq \hsic_{l-1} <  \mathcal{E}_{n+1} \implies \hsic^{*} - \mathcal{E}_{n} \geq \hsic^{*} - \hsic_{l-1} > \hsic^{*} - \mathcal{E}_{n+1}.
    \label{eq:all_ineqals}
\end{equation}
Thus combining \eq{eq:delta_define}, \eq{eq:delta_greater_than_l1}, and \eq{eq:all_ineqals} we have
\begin{equation}
    \delta_{l-1} > \delta_{l}.
\end{equation}
Therefore, $\{ \delta_l \}$ is a decreasing sequence.

 

\textbf{Step 3: } 
Note that $\{\mathcal{E}_{n}\}$ is a converging sequence where 
\begin{equation}
    \lim_{n \rightarrow \infty}
    \hsic^{*} - \frac{\hsic^{*} - \hsic_0}{n} = \hsic^*.
\end{equation}
Therefore, $\{\Delta_n\} = \hsic^* - \{\mathcal{E}_n\}$ is also a converging sequence where 
\begin{equation}
    \lim_{n \rightarrow \infty}
    \hsic^* - \hsic^{*} + \frac{\hsic^{*} - \hsic_0}{n} = 0
\end{equation}
and $\{\delta_{l}\}$ is a subsequence of $\{\Delta_{l}\}$. Since any subsequence of a converging sequence also converges to the same limit, we know that
\begin{equation}
    %\lim_{n \rightarrow \infty}
    %\mathcal{E}_n = \hsic^* 
    %\implies
    \lim_{l \rightarrow \infty} \delta_l = 0.
\end{equation}
   

        
% As $l \rightarrow \infty$, we have the inequality
% \begin{align}
%     \lim_{l \rightarrow \infty}
%     \delta_{l} 
%     & \leq
%     \hsic^{*} - 
%     \lim_{l \rightarrow \infty}
%     \mathcal{E}_{l}, \\
%     & \leq
%     \hsic^{*} - \lim_{l \rightarrow  \infty}(\hsic^{*} - \frac{\hsic^{*} - \hsic_0}{l}), \\
%     & \leq 0.
% \end{align}

Following this construction, if we always choose $\hsic_l$ such that 
\begin{equation}
    \hsic^{*} - \hsic_{l} \leq \delta_{l}.
    \label{eq:key_inequality}
\end{equation}
As $l \rightarrow \infty$, the inequality becomes
\begin{align}
    \hsic^{*} - 
    \lim_{l \rightarrow \infty} 
    \hsic_{l} 
    &  \leq 
    \lim_{l \rightarrow \infty} 
    \delta_{l}, \\
    &  \leq 
    0.
\end{align}
Since we know that 
\begin{equation}
    \hsic^{*} - \hsic_l \geq 0\, \forall l. 
\end{equation}
The condition of 
\begin{equation}
    0 \leq
    \hsic^{*} - \lim_{l \rightarrow \infty} \hsic_l \leq 0
\end{equation}
is true only if 
\begin{equation}
    \hsic^{*} - \lim_{l \rightarrow \infty} \hsic_l = 0.
\end{equation}
This allows us to conclude 
\begin{equation}
    \hsic^{*} = \lim_{l \rightarrow \infty} \hsic_l.
\end{equation}



% where $\delta_{l} = \min(\frac{\hsic^* - \hsic_0}{l+1},\hsic^{*} - \hsic_{l-1}+\epsilon)$, where $0<\epsilon <$ such that 
% \begin{equation}
%     \forall l>0: \hsic^{*} - \hsic_{l} \leq \delta_{l}
% \end{equation}
% then as $l \rightarrow \infty$, we have
% \begin{equation}
%     \lim_{l\rightarrow  \infty}\delta_{l} = \min(\frac{\hsic^* - \hsic_0}{l+1},\hsic^{*} - \hsic_{l-1}) = \min(0,\hsic^{*} -  \lim_{l \rightarrow \infty}  \hsic_l)
% \end{equation}

% $\hsic^{*} -  \lim_{l \rightarrow \infty} >0$,

%hence $\lim_{l\rightarrow \infty}\delta_{l} = 0$, which we can conclude that \begin{equation}
%    \hsic^{*} - \lim_{l \rightarrow \infty}  \hsic_l \leq 0 
%\end{equation}, on the other hand we have $\hsic^{*} - \hsic_l \geq 0\, \forall l$ which conclude the first condition of the proof:
%\begin{equation}
%   \lim_{l \rightarrow \infty}  \hsic_l = \hsic^*
%\end{equation}

\textbf{Proof of the Monotonic Improvement. } 

Given \eq{eq:bounding_box} and \eq{eq:delta_define}, 
at each step we have the following: 
\begin{align}
    \hsic_{l-1} & < \mathcal{E}_{n+1} \\
    & \leq 
    \hsic^{*} - \delta_{l}. 
\end{align}
Rearranging this inequality, we have
\begin{equation}
    \delta_{l} < \hsic^{*} - \hsic_{l-1}.
    \label{eq:keyIneq}
\end{equation}
By combining the inequalities from \eq{eq:keyIneq} and  \eq{eq:key_inequality}, we have the following relationships.
\begin{align}
    \hsic^{*} - \hsic_{l} \leq \delta_{l} & < \hsic^{*} - \hsic_{l-1} \\
    \hsic^{*} - \hsic_{l} & < \hsic^{*} - \hsic_{l-1} \\
    - \hsic_{l} & < - \hsic_{l-1} \\
    \hsic_{l} & > \hsic_{l-1}, \\
\end{align}
which concludes the proof of theorem.


\end{adjustwidth}
\end{proof}

%\begin{lemma}
%    There exists a $\sigma_{l-1}$ and $\sigma_l$ such that convergence is monotonic where
%    \begin{equation}
%    \hsic_{l} > \hsic_{l-1} \quad \forall l.
%    \end{equation}
%\end{lemma}
%\begin{proof}
% Given the proof from \citelemma{app:lemma:approach_optimal_H}, each layer we have
%\begin{equation}
%    \hsic^* - \hsic_l \le \frac{\hsic^* - \hsic_0}{l}.     
%\end{equation} 
%Since $\frac{\hsic^* - \hsic_0}{l}$ decreases as $l$ increase, then at each layer, we have the condition
%\begin{equation}
%    \hsic_{l+1} > \hsic_l.
%\end{equation}
%
%    
%    
%\end{proof}







\begin{lemma}
\label{app:lemma:W_not_optimal} Given $\frac{1}{\sqrt{\zeta}}$ as a normalizing constant for  $W_s = \frac{1}{\sqrt{\zeta}} \sum_{\alpha} r_{\alpha}$ such that $W^TW=I$, then $W_s$ is not guaranteed to be the optimal solution for the HSIC objective.
\end{lemma}

\begin{proof}
    We start with the Lagrangian
    \begin{equation}
        \mathcal{L} = 
        - \sum_{i,j} \Gij \ISMexp - \Tr(\Lambda(W^TW - I)).
    \end{equation}
    If we now take the derivative with respect to the Lagrange, we get
    \begin{equation}
        \nabla \mathcal{L} = 
        \frac{1}{\sigma^2}
        \sum_{i,j} \Gij \ISMexp
        (r_i - r_j)(r_i - r_j)^TW 
        - 2W\Lambda.
    \end{equation}
    By setting the gradient to 0, we have
     \begin{align}
        \left[
        \frac{1}{2\sigma^2}
        \sum_{i,j} \Gij \ISMexp
        (r_i - r_j)(r_i - r_j)^T 
        \right]
        W 
        =&  W\Lambda. \\
        \mathcal{Q}_l W =& W \Lambda.
        \label{app:eq:ism_conclusion}
    \end{align}   
    From \eq{app:eq:ism_conclusion}, we see that $W$ is only the optimal solution when $W$ is the eigenvector of $Q_l$. Therefore, by setting $W$ to 
    $W_s = \frac{1}{\sqrt{\zeta}} \sum_{\alpha} r_{\alpha}$, it is not guaranteed to yield an optimal.
    
   
%    From this relationship, we see that $W$ is only an optimal solution 
%   
%    Now, we put $W = \sum_{\alpha} r_{\alpha}$ into the gradient of the Lagrangian and set the gradient to 0.
%    \begin{equation}
%    \begin{split}
%        \nabla \mathcal{L}
%        ((\frac{1}{\sqrt{\zeta}} 
%        \sum_{\alpha} r_\alpha)) = 
%        \frac{1}{\sigma^2}\sum_{i,j} \Gij e^{-\frac{(r_i - r_j)^T (\sum_{\alpha} r_\alpha) (\sum_{\alpha} r_\alpha)^T(r_i - r_j)}{2 \zeta \sigma^2}}
%        (r_i - r_j)(r_i - r_j)^T(\sum_{\alpha} r_\alpha)\\
%        & - 2 (\sum_{\alpha} r_\alpha) \Lambda.
%    \end{split}
%    \end{equation}
%     \begin{equation}
%    \begin{split}
%        \frac{1}{2\sigma^2}\sum_{i,j} \Gij e^{-\frac{(r_i - r_j)^T (\sum_{\alpha} r_\alpha) (\sum_{\alpha} r_\alpha)^T(r_i - r_j)}{2 \zeta \sigma^2}}
%        (r_i - r_j)(r_i - r_j)^T(\sum_{\alpha} r_\alpha)
%        = (\sum_{\alpha} r_\alpha) \Lambda.
%    \end{split}
%    \end{equation}   
\end{proof}




\end{appendices}

==> append3/ad_matrix_derivation.tex <==
\begin{appendices} 
\section{Derivation for $\sum_{i,j} \Psi_{i,j} (x_i - x_j)(x_i - x_j)^T = 2X^T(D_\Psi - \Psi)X$}
\label{app:matrix_derivation}
Since $\Psi$ is a symmetric matrix, and $A_{i, j} = ( x_i - x_j) ( x_i -
x_j)^T $, we can
rewrite the expression into
\[ \begin{array}{lll}
     \sum_{i, j} \Psi_{i, j} A_{i, j}  & = &  \sum_{i, j} \Psi_{i, j} ( x_i -
     x_j) ( x_i - x_j)^T\\
     & = & \sum_{i, j} \Psi_{i, j} ( x_i x_i^T - x_j x_i^T - x_i x_j^T +
     x_j x_j^T)\\
     & = & 2 \sum_{i, j} \Psi_{i, j} ( x_i x_i^T - x_j x_i^T)\\
     & = & \left[ 2 \sum_{i, j} \Psi_{i, j} ( x_i x_i^T) \right] - \left[ 2
     \sum_{i, j} \Psi_{i, j} ( x_i x_j^T) \right] .
   \end{array} \]
If we expand the 1st term, we get
\begin{align}
    2\sum_{i}^n \sum_{j}^n 
    \Psi_{i, j} ( x_i x_i^T)
    & = 
    2 \sum_i
   \Psi_{i, 1} ( x_i x_i^T) +
   \ldots + \Psi_{i, n} ( x_i x_i^T) \\
   &= 
   2 \sum_{i}^n 
   [\Psi_{1, 1} + \Psi_{1, 2} + ...]
   x_i x_i^T \\
   &= 
   2\sum_{i}^n 
   d_i 
   x_i x_i^T \\  
   &=
   2 X^TD_\Psi X
\end{align}
Given $\Psi_i$ as the $i$th row, next we look at the 2nd term
\begin{align}
    2 \sum_i \sum_j \Psi_{i, j}  x_i x_j^T
    &=
    2 \sum_i \Psi_{i, 1}  x_i x_1^T
    + \Psi_{i, 2}  x_i x_2^T
    + \Psi_{i, 3}  x_i x_3^T + ...\\
    &=
    2 \sum_i   x_i (\Psi_{i, 1} x_1^T)
    + x_i (\Psi_{i, 2} x_2^T)
    + x_i (\Psi_{i, 3} x_3^T) + ...\\
    &=
    2 \sum_i   x_i 
    \left[
    (\Psi_{i, 1} x_1^T)
    + (\Psi_{i, 2} x_2^T)
    + (\Psi_{i, 3} x_3^T) + ...
    \right]\\
    &=
    2 \sum_i   x_i 
    \left[
    X^T \Psi_i^T
    \right]^T\\   
    &=
    2 \sum_i   x_i 
    \left[
    \Psi_i X
    \right]\\      
    &=
    2 \left[   
    x_1 \Psi_1 X + 
    x_2 \Psi_2 X + 
    x_3 \Psi_3 X + ...
    \right]\\         
    &=
    2 \left[   
    x_1 \Psi_1  + 
    x_2 \Psi_2  + 
    x_3 \Psi_3  + ...
    \right]X \\            
    &=
    2X^T \Psi  X \\               
\end{align}
Putting both terms together, we get
\begin{align}
    \sum_{i,j} \Psi_{i,j} A_{i,j} &=  2 X^TD_\Psi X -  2X^T \Psi  X a\\
    &=  2 X^T[ D_\Psi - \Psi] X \\
\end{align}

\end{appendices} 

==> append3/af_sigma_values.tex <==
\clearpage
\newpage

\begin{appendices}
\section{Sigma Values used for Random and Adversarial Simulation}
\label{app:sigma_values}

The simulation of Thm.~\ref{thm:hsequence} as shown in Fig.~\ref{fig:thm_proof} spread the improvement across multiple layers. The $\sigma_l$ and $\hsic_l$ values are recorded here. We note that $\sigma_l$ are reasonably large and not approaching 0 and the improvement of $\hsic_l$ is monotonic. 

\begin{figure}[h]
\center
    \includegraphics[width=9cm]{img/Random_sigma.png}
    \caption{}
\end{figure} 

\begin{figure}[h]
\center
    \includegraphics[width=9cm]{img/adv.png}
    \caption{}
\end{figure} 


%\newpage

Given a sufficiently small $\sigma_0$ and $\sigma_1$, Thm.~\ref{thm:hsequence} claims that it can come arbitrarily close to the global optimal using a minimum of 2 layers. We here simulate 2 layers using a relatively small $\sigma$ values ($\sigma_0 = 10^{-5}$) on the Random (left) and Adversarial (right) data and display the results of the 2 layers below. Notice that given 2 layer, it generated a clearly separable clusters that are pushed far apart.

    \begin{figure}[!h]
    \begin{minipage}[H]{6.0cm}
        \includegraphics[width=6cm]{img/random_2_layer.png}
        \caption{Random Dataset with 2\\layers and $\sigma=10^{-5}$}
    \end{minipage}%
    \begin{minipage}[H]{6.0cm}
        \includegraphics[width=6cm]{img/adversarial_2_layer.png}
        \caption{Adversarial Dataset with 2 \\layers and $\sigma=10^{-5}$}
    \end{minipage}
    \end{figure}          

\end{appendices}

==> appendices/2nd_necessary.tex <==
\begin{appendices}
\section{2nd Order Necessary Conditions}\label{app:2nd_order}
\begin{lemma} 
  [Bertsekas, Proposition 3.1.1~{\cite{bertsekas1997nonlinear}}] (Lagrange Multiplier Theorem - Necessary Conditions)
    Consider the optimization problem:
  $ \min_{W : h (W) = 0} f (W), $
where $f : \mathbb{R}^{d \times q} \to \mathbb{R}$ and $h :
  \mathcal{R}^{d \times q} \to \mathbb{R}^{q \times q}$ are twice continuously
  differentiable. Let   $\mathcal{L}$ be the Lagrangian and $h(W)$ its equality constraint. Then, a local minimum must satisfy the following  conditions:
  \begin{subequations}
    \begin{align} 
    &\nabla_W \mathcal{L} (W^{\ast}, \Lambda^{\ast}) = 0, \label{eq:1st_W}\\
    &\nabla_{\Lambda} \mathcal{L} (W^{\ast}, \Lambda^{\ast}) = 0, \label{eq:1st_lambda}\\
    \begin{split}
     \tmop{Tr}( Z^T &\nabla_{W W}^2 \mathcal{L}(W^{\ast}, \Lambda^{\ast}) Z) \geq 0 \\ 
     &\tmop{for}   \tmop{all} Z \neq 0 , \tmop{with}  \nabla h (W^{\ast})^T Z = 0.   \label{eq:2nd_W_in_append} 
    \end{split}
    \end{align}   
  \end{subequations}
\end{lemma}
\end{appendices}


==> appendices/A_lemma_1.tex <==
\begin{appendices}
\section{Lemma \ref{lemma:lemma1}}
\label{app:lemma_1_proof}
\subsection{Assumptions and Notations of the Proof}
Since the positive and negative properties of the $\Gamma$ matrix are used throughout several proofs in the paper, we prove its properties as a lemma here. Following the convention of the paper, we are given a dataset $X \in \mathbb{R}^{N \times d}$ of $C$ classes where $N$ denotes the number of samples and $d$ the dimensions of the data. Given $C$ classes, we let $n_c$ be the number of samples in the $c$th class. Let its classification labels use one-hot encoding and denoted as $Y \in \mathbb{R}^{N \times C}$. Also let $H$ be the centering matrix defined as $H = I - \frac{1}{N} \mathbf{1}_{N \times N}$ where $\mathbf{1}_{N \times N}  \in \mathbb{R}^{N \times N}$ represents a matrix of all 1s. Since $H$ is a centering matrix, it has the property $H = H^T$. 
Lastly, let $\Gamma \in \mathbb{R}^{N \times N}$ matrix be defined as $\Gamma = HYY^TH$. 


\subsection{Lemmas of the Proof}
\begin{lemma}\label{lemma:lemma1}
If the size of any single class is less than the size of the union of any other two classes, then every ($x_i, x_j$) pair of samples of the same class has a corresponding positive $\Gamma_{i,j}$ and every ($x_i, x_j$) pair of samples of different classes has a corresponding negative $\Gamma_{i,j}$.
\end{lemma}
\begin{proof}
Given $C$ classes, the total number of samples $N$ is the summation of the number of samples, $n_c$, for each class where
    \begin{equation}
    N = \sum_{c=1} n_c.
    \end{equation}
It can be easily verified that the linear kernel matrix $K = Y Y^T$ has $(i,j)$th element as 1 and 0 if the $(x_i,x_j)$ pair belong to the same and different classes respectively. It can also be easily verified that $K=K^T$. We denote the constant $\eta$ here as 
    \begin{equation}
    \eta = \mathbf{1}_N^T K \mathbf{1}_N
    \end{equation}
where $\mathbf{1}_N$ is a vector of 1s of length $N$. In other words, $\eta$ represents the cardinality of all $(x_i,x_j)$ pairs that belong to the same classes and can also be computed as 
    \begin{equation}
    \eta = \sum_{c=1} n_c^2.
    \end{equation}
We next define the degree vector as 
    \begin{equation}
    d = [d_1, d_2, ... d_N]^T = K \mathbf{1}_N
    \end{equation}
and the stacked degree matrix $D \in \mathbb{R}^{N \times N}$ as
    \begin{equation}
    D = [d, d, ...].
    \end{equation}
To clarify, the columns of $D$ consists of repeated vectors of $d$. Given these relationship, we first apply the centering matrix to $K$ and obtain
    \begin{equation}
    HK = (I - \frac{1}{N} \mathbf{1}_{N \times N})K =
    K - \frac{1}{N} D^T.
    \end{equation}
Next, we apply the centering matrix on the right hand side and obtain  
    \begin{align*}
        \Gamma = HKH &= ((HKH)^T)^T \\
        &= (H (HK)^T)^T \\
        &= (H (K - \frac{1}{N} D^T)^T)^T \\
        &= ((I - \frac{1}{N} \mathbf{1}_{N \times N}) (K^T - \frac{1}{N} D))^T \\
        &= K - \frac{1}{N} D^T - \frac{1}{N} D + 
        \frac{\eta}{N^2} \mathbf{1}_{N \times N}.
    \end{align*}
Therefore, at each element of $\Gamma$ we get
    \begin{equation}
    \Gamma_{i,j} = K_{i,j} - \frac{1}{N}(d_i + d_j) + \frac{\eta}{N^2}.
    \end{equation}
First, we assume that the $(x_i,x_j)$ pair belong to the same class of size $n_{\kappa}$, and therefore $K_{i,j}=1$, we obtain
    \begin{align*}
    \Gamma_{i,j} &= 1 - \frac{2 n_{\kappa}}{N} + \frac{\eta}{N^2}\\
    &= \frac{N^2}{N^2} - \frac{2 n_{\kappa} N}{N^2} + \frac{\eta}{N^2}.
    \end{align*}
Since we want to show that this value is always positive, the division by $N^2$ can be ignored. Hence, we obtain
    \begin{align*}
    \frac{N^2}{N^2} - \frac{2 n_{\kappa} N}{N^2} + \frac{\eta}{N^2} &> 0 \\
    N^2 - 2 n_{\kappa} N + \eta &> 0\\
    \left[\sum_{c=1} n_c\right]\left[\sum_{c=1} n_c\right] - 2 n_{\kappa} \sum_{c=1} n_c + \sum_{c=1} n_c^2 &> 0
    \end{align*}
Since $\sum_{c=1} n_c^2$ is always positive, it is always greater than 0. For now we ignore this term and focus on proving the following inequality.
    \begin{align*}
    \left[\sum_{c=1} n_c\right]\left[\sum_{c=1} n_c\right] >& 2 n_{\kappa} \left[ \sum_{c=1} n_c \right] \\
    \left[\sum_{c=1} n_c\right] >& 2 n_{\kappa}  \\
    n_1 + n_2 + ... + n_k + ... + n_C > &2n_k\\
    n_1 + n_2 + ... + 0 + ... + n_C >& n_k
    \end{align*}
Since $n_k$ by assumption cannot be greater than the summation of any 2 classes, the above inequality is always true.

Next, we show that if $(x_i,x_j)$ are not in the same class, the $\Gamma_{i,j}$ value is always negative. In this case, $K_{i,j} = 0$ and therefore, we get
    \begin{align*}
    \Gamma_{i,j} &= 0 - \frac{1}{N}(d_i + d_j) + \frac{\eta}{N^2} \\
    &= \frac{\eta}{N^2} - \frac{N}{N^2}(d_i + d_j) .
    \end{align*}
Again, we can ignore the denominator. We let samples $x_i$ and $x_j$ come from two distinct class group of sizes $n_\alpha$ and $n_\beta$. To obtain a negative value for $\Gamma_{i,j}$ we need to satisfy the inequality 
    \begin{align*}
    \eta - N(d_i + d_j) &< 0\\
    \sum_{c=1} n_c^2 - (n_\alpha + n_\beta)(\sum_{c=1} n_c) &< 0 \\
    (n_\alpha^2 + n_\beta^2)
    - (n_\alpha^2 + n_\beta^2)
    - 2(n_\alpha n_\beta)
    - \sum_{c=1} n_c(n_c - n_\alpha - n_\beta) &< 0 \\
    - 2(n_\alpha n_\beta)
    - \sum_{c=1} n_c(n_c - n_\alpha - n_\beta) &< 0
    \end{align*}
Since $-2(n_\alpha n_\beta)$ is always negative, we can ignore this term. In fact, since $n_c$ is always positive, we can also remove it from the 2nd term and simply need to show that for all $c$
    \begin{align*}
        n_c - n_\alpha - n_\beta &< 0, \\
        n_c &< n_\alpha + n_\beta. 
    \end{align*}

Since the size of any class is always smaller than the size of the union any two classes, the inequality must be true.
Hence, its corresponding $\Gamma_{i,j}$ will also always be negative.
\end{proof}

It is important to note that our proof is simply a theoretical exercise to match the formulation with HSIC. In practice, since the labels are known, $\Gamma_{i,j}$ can always be set to 1 and -1 based on the label. This is equivalent to changing the definition of the one-hot encoded labels. Therefore, the assumption that any class cannot be larger than the combination of any other two classes can be easily circumvented if the data is highly unbalanced. In general, this proof recommends to set $\Gamma_{i,j}$ directly to positive and negative 1 instead of relying on the centering matrix.  
\end{appendices}


==> appendices/a_HSIC_objective.tex <==
\begin{appendices}
\section{Proof for Theorem \ref{thm:CCN_becomes_HSIC}}
\label{app:proof_for_CCN_becomes_HSIC}

Let $R_{l-1} \in \mathbb{R}^{n \times m}$ be the input of a layer, $R_{l} \in \mathbb{R}^{n \times m}$ the output of a layer, $W_l \in \mathbb{R}^{m \times q}$ its layer weights and $\Psi$ the activation function. We also let $H$ be the centering matrix defined as $H = I - \frac{1}{n} \mathbf{1}_{n\times n}$.
A layer of MLP is equivalent to a single cyclic transition of our model starting from RKHS as showing in Fig.~\ref{fig:flow}. 
    \begin{figure}[!h]
    \centering
        \includegraphics[width=4cm,height=1.5cm]{{img/Diagram1.png}}
        \caption{Flow of information}
        \label{fig:flow}
    \end{figure}  

The dependence between $R_l = \Psi(R_{l-1} W_l)$ and its label $Y$ can be maximized by maximizing norm squared of their Cross Covariance Matrix. The Cross Covariance Matrix empirically can be computed with
    \begin{equation}
        Cov = \frac{1}{n-1}\Psi(R_{l-1}W_l)^TH H Y.
    \end{equation}
We further condense the Cross Covariance Matrix into a single value by finding its norm squared. Coincidentally, this matches the definition of HSIC in RKHS where
    \begin{equation}
        \hsic(R_{l-1}W_l) = 
        ||Cov||^2 = \frac{1}{(n-1)^2} \Tr(
        Y^T H H \Psi(R_{l-1}W_l)
        \Psi(R_{l-1}W_l)^TH H Y).
    \end{equation}
Note that since $H = HH$ and $H = H^T$, we can further condense the expression into
    \begin{equation}
        \hsic(R_{l-1}W_l) = 
        ||Cov||^2 = \frac{1}{(n-1)^2} \Tr(
        H\Psi(R_{l-1}W_l)
        \Psi(R_{l-1}W_l)^T HYY^T).
    \end{equation}
Since $YY^T$ is simply the kernel matrix for $Y$, we denote it as $K_Y$. Similarly, we also obtain the kernel matrix $K_{R_{l-1}W_l} = \Psi(R_{l-1}W_l) \Psi(R_{l-1}W_l)^T$, thereby yielding the standard HSIC objective
    \begin{equation}
        \hsic(R_{l-1}W_l) = 
        ||Cov||^2 = \frac{1}{(n-1)^2} \Tr(
        HK_{R_{l-1}W_l} H K_Y).
    \end{equation}
At this point, our goal is to discover the optimal network weight $W_l$ constrained on $W^TW=I$ at the $l$th layer that maximizes this dependency between $\Psi(R_{l-1}W_l)$ and $Y$, therefore, we arrive to our objective Eq.~(\ref{eq:hsic_obj_pure}) where
    \begin{equation}
        \underset{W_l}{\max} \quad \Tr( HK_Y H K_{R_{l-1} W_l} )
        \hspace{0.3cm} \text{s.t} \hspace{0.3cm} W_l^TW_l = I.
    \end{equation}
\end{appendices}

==> appendices/a_thm_1_2.tex <==
\begin{appendices}
\section{Proof for Proposition \ref{thm:central_theorem}}
\label{app:central_theorem}
\textbf{Theorem} \ref{thm:central_theorem} :
\textit{ If each cyclic transition is greedily optimized to generate a monotonic sequence in a bounded space, then Properties~\ref{prop:convergent_property} and \ref{prop:convergent_limit_property} are satisfied.}

\begin{proof}
To begin our proof, we first evoke the Monotone Convergence Theorem \cite{bibby1974axiomatisations} which states that a monotone sequence is guaranteed to have a limit if and only if the sequence is bounded. 
Since this condition is assumed to be true in Theorem \ref{thm:central_theorem}, then it follows that the sequence generated by the cyclic transitions must also converge to a limit. Hence, Property~\ref{prop:convergent_property} is satisfied.


As for Property 2, the limit of the sequence must satisfy the 2nd order condition. By assuming that the MLP is solved greedily, this implies that the output of the previous layer is used as input for the next layer. Therefore, each cycle is its own optimization problem. Assuming that each cyclic transition is solved to satisfy the 2nd order condition, then every element of the \textit{risk sequence} must also satisfy the 2nd order condition. Therefore guaranteeing the limit of the sequence to satisfy the 2nd order condition and Property 2.
\end{proof}
\end{appendices}














==> appendices/b_hsic_is_affinity.tex <==

\begin{appendices}
\section{Proof for Theorem \ref{thm:ccn_satisfies_dependence_property}}
\label{app:ccn_satisfies_dependence_property}
\textbf{Theorem} \ref{thm:ccn_satisfies_dependence_property}:  
\textit{HSIC is an affinity objective}.  

\begin{proof}
Given $\mathcal{S}$ and $\mathcal{S}^c$ as sets of all pairs of samples of $(x_i,x_j)$ from a dataset $X$ with labels $Y$ that belongs to the same and different classes respectively, let $\Gamma_{i,j}$ be a set of scalar values, and let $\kappa$ be a similarity measure between any pairs of $(x_i, x_j)$. 

To prove Theorem~\ref{thm:ccn_satisfies_dependence_property}, we first leverage the result from \citet{gretton2005measuring} and rewrite the CCN objective as  
\begin{equation}
    \underset{W}{\max} \quad \Tr( K_{XW} H K_Y H)
    \hspace{1cm} \text{s.t} \hspace{1cm} W^TW = I.
     \label{eq:in_appendix_hsic_trace_obj}
\end{equation}
    If we let $\Gamma = HK_YH$ and convert the trace into a sum, then Eq.~(\ref{eq:in_appendix_hsic_trace_obj}) becomes
    \begin{equation}
        \underset{W}{\max} \quad \sum_{i,j} \Gamma_{i,j} K_{(XW)_{i,j}}
        \hspace{1cm} \text{s.t} \hspace{1cm} W^TW = I.
         \label{eq:in_appendix_hsic_sum}
    \end{equation}
    By the definition of kernel matrices, $K_{(XW)_{i,j}}$ is the inner product of $\Psi(W^Tx_i)$ and $\Psi(W^Tx_j)$, or $\langle \Psi(W^Tx_i), \Psi(W^Tx_j) \rangle$. By applying Lemma~\ref{lemma:lemma1} in Appendix~\ref{app:lemma_1_proof}, 
    Eq.~(\ref{eq:in_appendix_hsic_sum}) can be split into positive and negative $\Gamma_{i,j}$s where 
     \begin{equation}
        \underset{W}{\max} \quad \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} 
        \langle \Psi(W^Tx_i), \Psi(W^Tx_j) \rangle - 
        \sum_{i,j \in \mathcal{S}^c}
        \Gamma_{i,j} 
        \langle \Psi(W^Tx_i), \Psi(W^Tx_j) \rangle
        \hspace{0.2cm} \text{s.t} \hspace{0.2cm} W^TW = I.
    \end{equation}   
    Since the inner product between unit vectors is a similarity measure of the angular distance, by setting $\kappa(. , .)$ as the inner product and letting $f = \Psi \circ W$ the theorem is proven.
\end{proof}
\end{appendices}

==> appendices/b_thm2_redo.tex <==
\begin{appendices}
\section{Proof for Theorem \ref{thm:the_right_activation_function}}
\label{app:the_right_activation_function}
Given:
    \begin{equation}
        \min_{W_l} \quad -\hsic(R_{l-1}W_l, Y) \quad
        \st W_l^TW_l = I.
        \label{eq:app:hsic}
    \end{equation}
    
\textbf{Theorem \ref{thm:the_right_activation_function}: }
    \textit{Given a \textbf{risk sequence} of globally optimized empirical risks $(\mathcal{E}_1^*, ..., \mathcal{E}_L^*)$ that is individually generated via the Greedy method with Eq.~(\ref{eq:app:hsic}) as proposed by Algorithm 1. If a RBF kernel is used, the \textbf{risk sequence} monotonically decreases and converges.}
    


\subsection{Assumptions and Notations of the Proof}

\begin{addmargin}[1em]{2em}% 1em left, 2em right
    Here, we let $R_{l-1}$ be the input to the $l$th layer where $r_i$ represents the $i$th sample of $R_{l-1}$.
    Given $W_l$ as the weight of the $l$th layer and let the non-linear activation function at the $l$th layer is denoted as $\phi_l$. Given $\mathcal{S}$ and $\mathcal{S}^c$ as sets of all pairs of samples of $(r_i,r_j)$ from a dataset $R_{l-1}$ that belongs to the same and different classes respectively. Corresponding to the data matrix $R_{l-1}$ is the label matrix $Y \in \mathbb{R}^{n \times c}$ where $c$ denotes the number of classes. Each label $y_i \in \mathbb{R}^c$ is in the one-hot encoding format. 
    
    We also here note the definition of an injective mapping, i.e., $\phi$ is injective if
    \begin{equation}
        x_{i} \neq x_{j} \rightarrow \phi(x_{i}) \neq \phi(x_{j}).
    \end{equation} 
    
 Although there are many ways to generate converging sequences, here, we leverage the 
Monotone Convergence Theorem \cite{bibby1974axiomatisations} where a monotone sequence is guaranteed to have a limit if and only if the sequence is bounded. Therefore, if each transition generates an $\mathcal{E}_l$ lower than $\mathcal{E}_{l-1}$ in a bounded space, the \textit{risk sequence} is guaranteed to converge, i.e., the monotonic decrease of the \textit{risk sequence} directly implies a convergence.

If we let $\Gamma = HK_YH$, then Eq.~(\ref{eq:app:hsic}) can be reformulated into
\begin{equation}
    \max_{W_l} \sum_{i,j} \Gamma_{i,j} K_{R_{l-1}W_{l_{i,j}}} \quad
    \st W_l^TW_l = I.
    \label{eq:app:hsic_sum}
\end{equation}
Since $\Gamma_{i,j}$ came directly from the label, it is a bounded value, i.e, the elements of th $\Gamma$ matrix is bounded. In addition, since the kernel matrix is the inner product of the elements in RKHS, and each function is bounded in $L_2$, the kernel matrix itself is also bounded. Together, the empirical risk $\mathcal{E} = \sum_{i,j} \Gamma_{i,j} K_{R_{l-1}W_{l_{i,j}}}$ must also exist in a bounded space. Since the space for $\mathcal{E}$ is bounded, the key to prove Thm.~\ref{thm:the_right_activation_function} is to demonstrate the monotonicity of \textit{risk sequence} by confirming the inequality 
\begin{equation}
    \mathcal{E}^*_l \ge \mathcal{E}^*_{l+1}.
    \label{eq:app:inequal}
\end{equation}
Since the empirical risks at local minimums can vary wildly, for theoretical analysis purpose, we assume that the sequence is generated only at the global minimum at each stage. In addition, we assume that an algorithm capable of obtaining the global is given. Specifically, we assume to be given an algorithm capable of solving Eq.~(\ref{eq:app:hsic}) while satisfying the First and Second Order Necessary Conditions as defined by \citet{bertsekas1997nonlinear}. Given these assumption, the contribution of the prove is to show that in an ideal case, applying the feature map of RBF kernels as the non-linearity of a network layer leads to a sequence that satisfies Inequality~(\ref{eq:app:inequal}).
\end{addmargin}

\begin{proof}
We first note that $f_{l^\circ} = f_l \circ f_{l-1} \circ ... \circ f_1$, therefore the globally optimal argument of Eq.~(\ref{eq:app:hsic_sum}) can be rewritten and solved as
\begin{equation}
    W_l^* = \argmax_{W_l} \quad
    \sum_{i,j} \Gamma_{i,j} 
    \langle
        f_{l^\circ}(x_i), f_{l^\circ}(x_j)
    \rangle
    \quad
    \st W_l^TW_l = I.
    \label{eq:app:hsic_sum}
\end{equation}
If we let the set $\mathcal{Q}_{l}$ be the space of potential $W$ matrices for Eq.~(\ref{eq:app:hsic_sum}), then $W^*_l$ is the optimal $W$ at layer $l$ within the set $\mathcal{Q}_l$. Next, if we let $\mathcal{Q}_{l+1}$ be the space of potential $W$ matrices at the $l+1$ layer. If we can show that $W^*_l$ is also inside the set of $\mathcal{Q}_{l+1}$, then the best $W$ matrix in $\mathcal{Q}_{l+1}$ must be at least as good as $W^*_l$, and therefore, $\mathcal{E}^*_l \ge \mathcal{E}^*_{l+1}$ is also true.

We next note that Eq.~(\ref{eq:app:hsic_sum}) using a RBF kernel can also be written as
\begin{equation}
    W_l^* = \argmax_{W_l} \quad
    \sum_{i,j} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}}
    \quad
    \st W_l^TW_l = I.
    \label{eq:app:hsic_rbf_sum}
\end{equation}
Since $\Gamma_{i,j}$ is positive for all $(r_i,r_j) \in \mathcal{S}$ and negative for $(r_i,r_j) \in \mathcal{S}^c$, Eq.~(\ref{eq:app:hsic_rbf_sum}) can be further broken into 
\begin{equation}
    W_l^* = \argmax_{W_l} \quad
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}}
    }_\text{1st term}
    -
    \underbrace{
    \sum_{i,j \in \mathcal{S}^c} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}} 
    }_\text{2nd term}
    \quad
    \st W_l^TW_l = I.
    \label{eq:app:hsic_rbf_sum_split}
\end{equation}
Since the $\Gamma_{i,j}$ of Eq.~(\ref{eq:app:hsic_rbf_sum_split}) are all positive for the 1st term and negative for the 2nd term. It immediately tells us what the global optimal solution should be. Namely, we wish for the first exponential terms to all be 1s, and the 2nd expoential term to all be 0s. This solution is possible if there exists a $W_l^*$ such that 
\begin{equation}
    \underbrace{
    W_l^T(r_i-r_j) = 0}_{\text{Condition 1}} 
    \quad 
    \forall \quad (r_i,r_j) \in \mathcal{S}
\end{equation}
and
\begin{equation}
    \underbrace{
    W_l^T(r_i-r_j) > 0}_{\text{Condition 2}} 
    \quad 
    \forall \quad (r_i,r_j) \in \mathcal{S}^c
\end{equation}
    We emphasize that $W_l^T(r_i - r_j) > 0$ is a sufficient condition because $\sigma > 0$ can be set arbitrarily small for the 2nd exponential term to approach 0. Specifically, we note that if $W^*_l$ exists, then when $\sigma$ is set arbitrarily small the 1st term becomes
\begin{equation}
    \underbrace{ 
    \lim_{\sigma \to 0} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}}
    }_\text{1st term} = 1 \quad
    \forall i,j \in \mathcal{S},
\end{equation}
and the 2nd term becomes
\begin{equation}
    \underbrace{ 
    \lim_{\sigma \to 0} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}}
    }_\text{1st term} = 0 \quad
    \forall i,j \in \mathcal{S}^c.
\end{equation}
Therefore, as $\sigma \to 0$, $W_l^T(r_i - r_j) > 0$ and $W_l^T(r_i - r_j) >> 0$ for all $(r_i,r_j) \in \mathcal{S}^c$ produces the same empirical risk $\mathcal{E}_l$. Our theorem focuses on the usage of the RBF kernels because as $\sigma \to 0$, it simplifies each element of our \textit{risk sequence} into two possibilities when a layered is optimized: 
\begin{enumerate}
  \item Condition 1 and 2 are satisfied (global optimal solution).
  \item Condition 1 failed and condition 2 is satisfied (not global optimal solution). 
\end{enumerate}
We claim that if the $(l-1)$th layer is in the first possible situation, it will always stay in the 1st situation given the next additional layer. However if the $(l-1)$th layer is in the 2nd situation, 

having a tuning $\sigma$ 


allows us

is an injective mapping \cite{sriperumbudur2008injective}.


possible for $f_{l+1}$ to be an identity map, i.e., 
\begin{equation}
    f_{l+1} \circ f_l(x) = f_l(x).
    \label{eq:app:identity_map}
\end{equation}
This possibility implies that the option of not changing Eq.~(\ref{eq:app:hsic_sum}) is a potential solution when $f_{l+1}$ is added. And if not changing the equation is a option, $W^*_l$ must be within the set of $\mathcal{Q}_{l+1}$. To finalize the prove, we provide the mapping where a RBF kernel with an $W_{l+1}$ can induce a $f_{l+1}$ that is an identity map.


, i.e., if we let the feature map of a characteristic kernel be $\phi$, then there exists a $\phi^{-1}$ such that $\phi^{-1} [ \phi(R_{l-1}) ] = R_{l-1}$. Additionally, we know that $W \in \mathbb{R}^{d \times q}$ where $d$ is the dimension of its input and $q$ can range from 1 to $\infty$, $W^{-1}$ also exists in the potential solution space. Since the composition of an injective $W$ and $\phi$ forms $f_{l+1}$, an injective $f_{l+1}$ exists within the set of potential solutions. Therefore, at the $l+1$th layer, it can 
\end{proof}
\end{appendices}















%\begin{addmargin}[1em]{2em}% 1em left, 2em right
%    We are given the following 3 properties:
%    $\newline$
%    \textbf{Property \ref{prop:convergent_property} : } 
%    \textit{ The \textbf{risk sequence} must converge to a limit.}
%    $\newline$
%    \textbf{Property \ref{prop:convergent_limit_property} : } 
%    \textit{The network weight $W_L$ given $W_1,..., W_{L-1}$ must satisfy the First and Second Order Necessary Conditions as defined by \citet{bertsekas1997nonlinear} for the limit empirical risk $\mathcal{E}_L$. }
%    $\newline$
%    \textbf{Property \ref{prop:separability_prop} : } 
%    \textit{ The empirical risk must satisfy the \textit{affinity property} defined as} $\newline$
%    \textbf{Definition \ref{def:affinity_def} : }
%    \textit{ Given $\mathcal{S}$ and $\mathcal{S}^c$ as sets of all pairs of samples of $(x_i,x_j)$ from a dataset $X$ that belongs to the same and different classes respectively, let all $\mu_{i,j}$ values be non-negative scalars, and let $\kappa$ be a similarity measure between any pairs of $(x_i, x_j)$. An empirical risk satisfies the \textit{affinity property} if there exists a $\kappa$ such that its optimal solution $f^*$ is also the optimal solution for the $\textbf{affinity objective}$, which we define here as}
%        \begin{align*}
%        \underset{f}{\max} \hspace{0.05cm} 
%        \sum_{i,j \in \mathcal{S}} \mu_{i,j} \mathcal{\kappa}(f(x_i), f(x_j)) - \sum_{i,j \in \mathcal{S}^c} 
%        \mu_{i,j}
%        \mathcal{\kappa}(f(x_i), f(x_j)).
%         \label{eq:separability_property_definition}
%        \end{align*}
%        \label{def:affinity_def}
%    
%
%
%
%
%
%
%
%
%
%
%    Given $\mathcal{S}$ and $\mathcal{S}^c$ as sets of all pairs of samples of $(x_i,x_j)$ from a dataset $X \in \mathbb{R}^{n \times d}$ that belongs to the same and different classes respectively. Corresponding to the data matrix $X$ is the label matrix $Y \in \mathbb{R}^{n \times c}$ where $c$ denotes the number of classes. Each label $y_i \in \mathbb{R}^c$ is in the one-hot encoding format. Let $\Gamma_{i,j}$ be a set of scalars, and let $\kappa$ be a similarity measure between any pairs of $(x_i, x_j)$. 
%    
%    By leveraging the Monotone Convergence Theorem, we know that a monotonic sequence in a bounded space converges to a fixed point. Since the solution space is bounded via the constraint of $W^TW=I$, the objective is to prove the monotonic improvements. This can be accomplished by proving the existence of a solution $W_l$ for the following inequality 
%    \begin{equation}
%        \underset{f_l}{\max} \quad ||\text{Cov}(f_{l^\circ}(X), Y)||_F \geq
%        ||\text{Cov}(f^*_{(l-1)^\circ}(X), Y)||_F.
%        \label{eq:key_inequality}
%    \end{equation}
%    Here, we denote $f^*_{(l-1)^\circ}$ as the optimal mapping discovered from the previous layer. The goal of the proof is to show the existence of $f_l$ such that $f_{l^\circ}$ will produce an equal or higher dependence at the current layer.
%    
%    Note that by using the Gaussian feature map as the activation function, the theoretical dimension of the mapping output is infinity with a norm of 1. Given an input sample $x_i$, we define $r_i$ such that $r_i = f^*_{(l-1)^\circ}(x_i)$. Following this notation, we let $R_{l-1} = [r_1, r_2, ..., r_n]^T$, therefore, $R_{l-1} = f^*_{(l-1)^\circ}(X)$ where $||r_i|| = 1$ for all $i$. In addition, by using a Gaussian kernel, the inner product between any two samples is bounded between 0 and 1 where $0 \le r_i^Tr_j \le 1$. We also leverage Dini's Theorem \cite{bartle1992introduction} in our proof, which states:
%    
%    \textbf{Dini's Theorem. }
%    If a monotone sequence of continuous functions converges pointwise on a compact space and if the limit function is also continuous, then the convergence is uniform.
%
%    The proof for Theorem \ref{thm:the_right_activation_function} is divided into 2 Lemmas, i.e., lemmas \ref{lemma:gaussian_equal_} and 
%    \ref{lemma:exist_weights}. In the next subsection, we provide a brief summary of how each lemma combine to prove the theorem.
%\end{addmargin}

==> appendices/b_thm_3.tex <==
\begin{appendices}
\section{Proof for Theorem \ref{thm:the_right_activation_function}}
\label{app:the_right_activation_function}

\textbf{Theorem \ref{thm:the_right_activation_function}: }
    For Gaussian kernels,  there exist a set of weights ${W_1, ..., W_L}$ such that the CCN objective generates a uniformly converging \textit{risk sequence}

\subsection{Assumptions and Notations of the Proof}
\begin{addmargin}[1em]{2em}% 1em left, 2em right
    Given $\mathcal{S}$ and $\mathcal{S}^c$ as sets of all pairs of samples of $(x_i,x_j)$ from a dataset $X \in \mathbb{R}^{n \times d}$ that belongs to the same and different classes respectively. Corresponding to the data matrix $X$ is the label matrix $Y \in \mathbb{R}^{n \times c}$ where $c$ denotes the number of classes. Each label $y_i \in \mathbb{R}^c$ is in the one-hot encoding format. Let $\Gamma_{i,j}$ be a set of scalars, and let $\kappa$ be a similarity measure between any pairs of $(x_i, x_j)$. 
    
    By leveraging the Monotone Convergence Theorem, we know that a monotonic sequence in a bounded space converges to a fixed point. Since the solution space is bounded via the constraint of $W^TW=I$, the objective is to prove the monotonic improvements. This can be accomplished by proving the existence of a solution $W_l$ for the following inequality 
    \begin{equation}
        \underset{f_l}{\max} \quad ||\text{Cov}(f_{l^\circ}(X), Y)||_F \geq
        ||\text{Cov}(f^*_{(l-1)^\circ}(X), Y)||_F.
        \label{eq:key_inequality}
    \end{equation}
    Here, we denote $f^*_{(l-1)^\circ}$ as the optimal mapping discovered from the previous layer. The goal of the proof is to show the existence of $f_l$ such that $f_{l^\circ}$ will produce an equal or higher dependence at the current layer.
    
    Note that by using the Gaussian feature map as the activation function, the theoretical dimension of the mapping output is infinity with a norm of 1. Given an input sample $x_i$, we define $r_i$ such that $r_i = f^*_{(l-1)^\circ}(x_i)$. Following this notation, we let $R_{l-1} = [r_1, r_2, ..., r_n]^T$, therefore, $R_{l-1} = f^*_{(l-1)^\circ}(X)$ where $||r_i|| = 1$ for all $i$. In addition, by using a Gaussian kernel, the inner product between any two samples is bounded between 0 and 1 where $0 \le r_i^Tr_j \le 1$. We also leverage Dini's Theorem \cite{bartle1992introduction} in our proof, which states:
    
    \textbf{Dini's Theorem. }
    If a monotone sequence of continuous functions converges pointwise on a compact space and if the limit function is also continuous, then the convergence is uniform.

    The proof for Theorem \ref{thm:the_right_activation_function} is divided into 2 Lemmas, i.e., lemmas \ref{lemma:gaussian_equal_} and 
    \ref{lemma:exist_weights}. In the next subsection, we provide a brief summary of how each lemma combine to prove the theorem.
\end{addmargin}

\subsection{Summary of the Proof}

\begin{addmargin}[1em]{2em}% 1em left, 2em right
\textbf{In Lemma~\ref{lemma:gaussian_equal_},} we demonstrate that when a Gaussian kernel is used with HSIC, the argmax of the HSIC objective is equivalent to the argmax of an \textit{affinity objective} using a negative Euclidean distance as a similarity measure. We refer to this objective as the \textit{Euclidean Affinity} defined as
\begin{equation}
        \underset{W}{\argmax} \quad   
        \Tr(W^TA_=W)
         - 
        \Tr(W^T A_{\ne}W) 
        \hspace{0.2cm} \text{s.t} \hspace{0.2cm} W^TW = I.
       \label{eq:euclid_object} 
\end{equation}
$A_=$ is defined as 
\begin{equation}
    A_= = \frac{1}{\sigma^2} \sum_{i,j \in \mathcal{S}} (r_i - r_j)(r_i - r_j)^T,
\end{equation}
and $A_{\ne}$ is defined as 
\begin{equation}
    A_{\ne} = \frac{1}{\sigma^2}\sum_{i,j \in \mathcal{\tilde{S}}} (r_i - r_j)(r_i - r_j)^T.
\end{equation}

Therefore, instead of solving the HSIC objective directly, we can optimize the \textit{Euclidean Affinity} as a surrogate objective since the argmax for both objectives are equivalent.

\textbf{In Lemma~\ref{lemma:exist_weights},} we first define $V$ as the set of eigenvectors of $A_{\ne}$ that have positive eigenvalues. Given $V$, we show that if the null space of $A_=$ is sufficiently large to intersect with the span of $V$, then a globally optimal solution $W^*$ exists. Since the null space of $A_=$ for a Gaussian kernel is infinitely large, unless the span of $A_=$ completely overlaps the span of $V$ (not possible), an intersection always exists, i.e., a global optimal $W^*$ exists. Given the existence of $W^*$, there must also exist a set of $W$s, $\{W_1, ..., W^*\}$, sampled from interpolation points between a point within the neighborhood of $W^*$ and $W^*$ that monotonically improves the objective. Lastly, since the Gaussian kernel is a Universal kernel, all of its functions in RKHS are continuous, therefore, the monotonic convergence is also uniform.
\end{addmargin}


\subsection{Lemmas of the Proof}

\begin{lemma}\label{lemma:gaussian_equal_}
Assuming that the feature map of a Gaussian kernel is used as the activation function, then the LHS of the Inequality~(\ref{eq:key_inequality}) we denote here as 
\begin{equation}
    \underset{W}{\argmax} \quad ||\text{Cov}(\Psi(R_{l-1}W), Y)||_F 
    \quad \text{s.t : } \quad W^TW = I
    \label{eq:cov_objective2}
\end{equation}
is equivalent to Eq.~(\ref{eq:euclid_object}).
\end{lemma}

\begin{proof}
Following the proof by \citet{gretton2005measuring}, the norm of the cross-covariance can be reformulated into the empirical HSIC objective where the inequality becomes
\begin{equation}
    ||\text{Cov}(\Psi(R_{l-1}W), Y)||_F
    =
    HSIC(R_{l-1} W, Y).
\end{equation}
Therefore, optimizing the CCN objective is equivalent to solving
\begin{equation}
    \underset{W}{\argmax} \quad 
    \Tr(K_{R_l W} H K_Y H) 
    \quad \textit{s.t : } \quad W^TW = I.
\end{equation}
If we let $\Gamma_{i,j}$ be the $(i,j)th$ element of the matrix $\Gamma = HK_YH$ and write out the Gaussian kernel, the objective becomes

\begin{equation}
    \underset{W}{\argmax} \quad \sum_{i,j} \Gamma_{i,j}e ^{- \frac{||W^Tr_i - W^Tr_j||^2}{2 \sigma^2}} \quad 
     s.t \quad W^TW = I.
     \label{eq:hsic_obj_with_gaussian2}
\end{equation}

Following Lemma~\ref{lemma:lemma1}, $\Gamma_{i,j}$ is positive if $(r_i,r_j)$ pair belongs to the same class, and it is negative when the pair are in different classes. We can split the summation into the positive and negative $\Gamma_{i,j}$ pairs.

\begin{equation}
    \underset{W}{\argmax} \quad \sum_{i,j \in S} \Gamma_{i,j}e ^{- \frac{||W^Tr_i - W^Tr_j||^2}{2 \sigma^2}} - \sum_{i,j \in S^c} \Gamma_{i,j}e ^{- \frac{||W^Tr_i - W^Tr_j||^2}{2 \sigma^2}}\quad 
     s.t \quad W^TW = I.
     \label{eq:hsic_obj_with_gaussian3}
\end{equation}
From Eq.~(\ref{eq:hsic_obj_with_gaussian3}), we see that given an appropriate $\sigma$ value the global optimal solution is achieved when the exponential terms are either 0 or 1 such that
\begin{equation}
    \underset{W}{\max} \quad \sum_{i,j \in S} \Gamma_{i,j}e ^{- \frac{||W^Tr_i - W^Tr_j||^2}{2 \sigma^2}} + \sum_{i,j \in S^c} -\Gamma_{i,j}e ^{- \frac{||W^Tr_i - W^Tr_j||^2}{2 \sigma^2}} = 
    \sum_{i,j \in S} \Gamma_{i,j}[1] - \sum_{i,j \in S^c} \Gamma_{i,j}[0]. 
     \label{eq:hsic_obj_with_gaussian4}
\end{equation}
Therefore, if there exists a $W^*$ that satisfies the following two conditions, $W^*$ must also be the global optimal. 
\begin{align}
    \label{eq:p23}
    \forall i,j \in S \quad & 
    \lim_{\sigma \rightarrow 0}
    e ^{- \frac{||W^Tr_i - W^Tr_j||^2}{2 \sigma^2}} = 1\\
    \label{eq:p24}
    \forall i,j \in S^c \quad & 
    \lim_{\sigma \rightarrow 0}
    e^{- \frac{||W^Tr_i - W^Tr_j||^2}{2 \sigma^2}} = 0.
\end{align}
Next, we consider the global optimal of the objective
\begin{equation}
    \underset{W}{\argmin} \quad
    \frac{1}{\sigma^2}
    \sum_{i,j \in \mathcal{S}} ||W^Tr_i - W^Tr_j||^2_{2} - 
    \frac{1}{\sigma^2}
    \sum_{i,j \in \mathcal{S}^c} ||W^Tr_i - W^Tr_j||^2_{2} 
    \quad \text{s.t : } \quad W^TW = I.
    \label{eq:dep_prop_obj}
\end{equation}
Similarly, we can state that if there exists a $W^*$ that satisfies the following two conditions, $W^*$ must also be the global optimal of Eq.~(\ref{eq:dep_prop_obj}).
\begin{align}
    \label{eq:pp2}
    \forall i,j \in S \quad & \lim_{\sigma \rightarrow 0}
        \frac{||W^Tr_i - W^Tr_j||^2}{2 \sigma^2} = 0\\
    \label{eq:pp3}
    \forall i,j \in S^c \quad & \lim_{\sigma \rightarrow 0} 
        \frac{||W^Tr_i - W^Tr_j||^2}{2 \sigma^2} = \infty.
\end{align}
Notice that the $W^*$ that satisfies conditions Eq.~(\ref{eq:pp2}) and (\ref{eq:pp3}) is the same $W^*$ that satisfies Eq.~(\ref{eq:p23}) and (\ref{eq:p24}). Therefore, if the global optimal of $W^*$ for Eq.~(\ref{eq:dep_prop_obj}) satisfies Eq.~(\ref{eq:pp2}) and (\ref{eq:pp3}), then the same $W^*$ would also be the global optimal for Eq.~(\ref{eq:hsic_obj_with_gaussian3}). 

Our goal is to use Eq.~(\ref{eq:hsic_obj_with_gaussian3}) as a surrogate to understand the conditions that guarantees the existence of $W^*$, thereby satisfying Eq.~(\ref{eq:pp2}) and (\ref{eq:pp3}). After, multiplying the square terms out, Eq.~(\ref{eq:dep_prop_obj}) becomes







%Since the optimal solution for Eq.~(\ref{eq:hsic_obj_with_gaussian4}) is true for any positive and negative $\Gamma_{i,j}$ of any magnitude 
%
%Since the Gaussian kernel is bounded between 0 and 1, Eq.~(\ref{eq:hsic_obj_with_gaussian2}) is maximized when the Gaussian kernel is equal to 1 when $\Gamma$ is positive and 0 when $\Gamma$ is negative. We emphasize here that the actual magnitude of $\Gamma_{i,j}$ is irrelevant. As long as $\Gamma_{i,j}$ is positive, the optimal solution is always when the exponential term is equal to 1. Conversely, for negative $\Gamma_{i,j}$ values, the maximal solution will negate the negative term by setting the exponential term to 0.
%
%From this observation, we know that if there exists a $W^*$ such that this 0 and 1 divergence is possible for the exponential term, then we can focus on optimizing the just exponent of the exponential. Therefore, $W^*$ must also maximize 

%The jump from Eq.~(\ref{eq:hsic_obj_with_gaussian2}) to Eq.~(\ref{eq:dep_prop_obj}) is a big leap. This is because they are actually different objectives with completely different solution landscapes. In fact, in practice, optimizing each equation with SGD will likely yield completely different solutions. This is due to the limitation of the optimization algorithm and the fact $W$ may not be flexible enough drive the 1st summation to 0 while driving the 2nd summation to $-\infty$. Yet, if we temporarily forget these limitations and simply assume the existence of a $W^*$ capable of driving the two terms into 0 and $-\infty$, then it becomes possible that the arguments of the global optimum are equivalent.

%The advantage of this approach is the simplicity of this alternative formulation. By studying this formulation, it will yield significant insights into the conditions which guarantee the existence of $W^*$. We also invite the reader to take a second to interpret the equation above; we are searching for a $W^*$ such that samples of the same class are compressed together while samples from different classes are pushed apart. 

\begin{equation}
    \underset{W}{\argmin} \quad
    \frac{1}{\sigma^2}
    \sum_{i,j \in \mathcal{S}} 
    (r_i - r_j)^T W W^T (r_i - r_j) - 
    \frac{1}{\sigma^2}
    \sum_{i,j \in \mathcal{S}^c} 
    (r_i - r_j)^T W W^T (r_i - r_j)
    \quad \text{s.t : } \quad W^TW = I.
    \label{eq:dep_prop_obj_2}
\end{equation}
Since $(r_i - r_j)^T W W^T (r_i - r_j)$ is a scalar value, we can place a Trace around the term and rotate them to obtain
\begin{equation}
    \underset{W}{\argmin} \quad
    \frac{1}{\sigma^2}
    \sum_{i,j \in \mathcal{S}} 
    \Tr[W^T (r_i - r_j)(r_i - r_j)^T W ] - 
    \frac{1}{\sigma^2}
    \sum_{i,j \in \mathcal{S}^c} 
    \Tr[W^T (r_i - r_j)(r_i - r_j)^T W]
    \quad \text{s.t : } \quad W^TW = I.
    \label{eq:dep_prop_obj_3}
\end{equation}
At this point, we can simply move the $\frac{1}{\sigma^2}$ value and the summation operation into the Trace to obtain
\begin{equation}
    \underset{W}{\argmin} \quad
    \Tr(W^T A_= W ) - 
    \Tr(W^T A_{\ne} W)
    \quad \text{s.t : } \quad W^TW = I.
    \label{eq:dep_prop_obj_4}
\end{equation}
%To push the Gaussian kernel to 1, we must minimize $||W^Tr_i - W^Tr_j||^2$ for $(i,j) \in \mathcal{S}$ towards 0 and maximize the same expression for pairs in $\bar{\mathcal{S}}$. Since $0 \le r_i^Tr_j \le 1$ and $W^TW=I$, $||W^Tr_i - W^Tr_j||$ is maximized at $\sqrt{2}$. Here, we observe that the same solution $W$ that minimizes Eq.~(\ref{eq:dep_prop_obj}) must also maximize Eq.~(\ref{eq:cov_objective2})
\end{proof}


\begin{lemma}\label{lemma:exist_weights}
    There exist a set of weights ${W_1, ..., W_L}$ such that the CCN objective generates a uniformly converging \textit{risk sequence}
\end{lemma}
\begin{proof}
Looking at the 1st term of Eq.~(\ref{eq:dep_prop_obj_3}) more carefully and focus on the $W^T (r_i - r_j)$ portion where $r_i$ and $r_j$ are assume to belong to the same class. In the most ideal case, we wish find a subspace projection $W$ that pulls all sample pairs together, i.e., we want $0 = W^T (r_i - r_j)$ for all $(r_i,r_j)$ pairs. This is possible only in the case where $W$ is in the null space of $A_=$.

Simultaneously, we want a $W$ that pushes $(r_i - r_j)$ distance infinitely large for the 2nd term. While infinity may not be possible, we know that the samples are maximally separated if $W$ is in the span of the eigenvectors of $A_{\ne}$ that has an associated positive eigenvalue. We refer to this set of eigenvectors as $V$. 

At this point, we can mentally draw the 2 spaces as 2 circles in a Venn diagram. One circle is the null space of $A_=$ while the other circle is the span of $V$. Therefore, the intersection of these 2 spaces would achieve both objectives simultaneously. Since the 1st term is pushed to 0, as long as the 2nd term is $\ne$ 0, we can set $\sigma$ to be very small to push the 2nd term toward infinity. Therefore, the key to the existence of $W^*$ is the existence of this intersection. Alternatively, we can state that if the null space of $A_=$ is sufficiently large such that it covers the span of $V$, then $W^*$ exists. 

Here, we leverage the feature map of a Gaussian kernel in that it has $A_= \in \mathbb{R}^{\infty \times \infty}$. Therefore, given that $A_=$ has a finite rank, its null space must have infinite dimensions. The only possibility for the null space of $A_=$ not to intersect with the span of $V$, is if $A_= = A_{\ne}$. Since $A_=$ and $A_{\ne}$ are by definition different, the null space of $A_=$ from a Gaussian kernel will always be sufficiently large to intersect the span of $V$, i.e., the usage of a Gaussian kernel guarantees the existence of $W^*$ for both Eq.~(\ref{eq:dep_prop_obj_4}) and (\ref{eq:hsic_obj_with_gaussian2}).

Given the existence of $W^*$ in the solution space of $\mathcal{W}$, we define its neighborhood of radius $r$ as 
\begin{equation}
    B_r(W^*) = \{W \in \mathcal{W}: d(W^*,W) < r\}.
\end{equation}
Given $B_r(W^*)$, there must also exist a $r$ and a set of $W$s, $\{W_1, ..., W^*\}$, sampled from interpolation points between a point within $B_r(W^*)$ and $W^*$ that monotonically improves the objective. In addition, since the Gaussian kernel is a Universal kernel, all of its functions in RKHS are continuous, therefore, the monotonic convergence is also uniform.
\end{proof}

We caution that proving the existence of a solution doesn't imply that the solution can be obtained easily or within a reasonable time. We have found experimentally that ISM is a fast algorithm that maintains this inequality with a uniform convergence.


\newpage 

\textbf{Aria's attempt:}

Define $\mathcal{E}_{l} = \{W^{*} = W_{1} ,\dots, W_{l}| W^{*} =      \underset{W}{\argmin} \quad
    \Tr(W^T A_= W ) - 
    \Tr(W^T A_{\ne} W)
    \quad \text{s.t : } \quad W^TW = I     \}$ to be the set of all weights that achieves optimal solution till depth $l$.
    
\textbf{Claim: The set $\mathcal{E}_{l} \subseteq (\mathcal{E}_{l+1})_{l}$ }.

If the claim is proven, the optimal solution at depth $l$ is consist of solutions at depth $l-1$, thus the optimal solution of depth $l$ is lower or equal than the optimal solution at depth $l-1$, meaning:

\begin{equation}
     ({\min} \quad
    \Tr(W^T A_= W ) - 
    \Tr(W^T A_{\ne} W)
    )_{l} \leq   ({\min} \quad
    \Tr(W^T A_= W ) - 
    \Tr(W^T A_{\ne} W)
    )_{l-1}
\end{equation}

Applying Lemma 2, we can conclude the following:
\begin{equation}
    \underset{f_l}{\max} \quad ||\text{Cov}(f_{l^\circ}(X), Y)||_F \geq
        ||\text{Cov}(f^*_{(l-1)^\circ}(X), Y)||_F.
\end{equation}

Hence the optimal $W$ for each depth induces a monotonically decreasing risk sequence. Furthermore the risk sequence is bounded from bellow by zero, thus the risk sequences is converging to its infimum. 



\textbf{Proof of the claim}:

$\mathcal{E}_{l} \subseteq (\mathcal{E}_{l+1})_{l}$:

For proving the claim we prove the following:

$$W^{*} \in \mathcal{E}_{l} \rightarrow W^{*} \in \mathcal{E}_{l+1}$$


Assume $W^{*} \in \mathcal{E}_{l} $. Matrix $A_{=}, A_{\neq}$ is positive semi definite, hence, $\Tr(W^T A_= W ),\Tr(W^T A_{\neq}W)$ is always a positive number, thus if the optimal solution $W^{*}$ exists in depth $l$ should satisfies that $\Tr(W^T A_= W ) = 0$ and $\Tr(W^T A_{\neq} W ) \neq 0$.

\textbf{Studying the behavior of $\Tr(W^T A_= W ) = 0$}:

Again because $A_{=}$ is positive semi definite, $\Tr(W^T A_= W ) $ is only zero, if $ W^T A_= W   = \Vec{0}$, 

\begin{equation}
   W^T A_= W  = W^{T} \frac{1}{\sigma^2} \sum_{i,j \in \mathcal{S}} (r_i - r_j)(r_i - r_j)^T W =  \frac{1}{\sigma^2} \sum_{i,j \in \mathcal{S}} W^T (r_i - r_j)(r_i - r_j)^T W
\end{equation}
because every elements inside the summation $(r_i - r_j)(r_i - r_j)^T$ is positive semi definite matrix, hence, $W^T (r_i - r_j)(r_i - r_j)^T W = \Vec{0} , i,j \in \mathcal{S}$. Matrix $W$ can be seen through its columns $W = [W_{1},\dots,W_{q}]$, thus $W^T (r_i - r_j)(r_i - r_j)^T W = \Vec{0}$ becomes:

\begin{equation}
\begin{split}
    &W_{1}^T (r_i - r_j)(r_i - r_j)^T W_{1} = 0 = ||(r_i - r_j)^T W_{1}||_{2} = 0 \rightarrow (r_i - r_j)^T W_{1} = 0 \rightarrow r_i^{T} W_{1} = r_j^T W_{1}  
    \\
    .\\
    .\\
    .\\
   & W_{q}^T (r_i - r_j)(r_i - r_j)^T W_{q} = 0  = ||(r_i - r_j)^T W_{q}||_{2} = 0 \rightarrow (r_i - r_j)^T W_{q} = 0 \rightarrow r_i^{T} W_{q} = r_j^T W_{q}
    \end{split}
\end{equation}
Which means the in IDs space $r_{i}$ and $r_{j}$ get mapped to a same point through $W$ linear transformation for $i,j \in \mathcal{S}$.  

Assuming Gaussian feature map $\phi$, for $x_{i} = x_{j}$, after the nonlinear mapping, they mapped to the same point is RKHS space, meaning $\phi(x_{i}) = \phi(x_{j})$, and hence for the next depth $l+1$ adding any linear $W$ will still keep $i,j$ points on top of each other. Hence the We concluded that, if $W^{*} $ till layer $l$ satisfies $\Tr(W^T A_= W ) = 0$, adding any $W$ at layer $l+1$ will still keep this part of the objective the same.



\textbf{Studying the behavior of $\Tr(W^T A_{\neq} W ) >> 0$}:



With the same argument, we can use the fact that $A_{\neq}$ is semi positive definite, hence, $\Tr(W^T A_{\neq} W ) \neq 0$ is equivalent to $W^T A_{\neq} W  \neq \Vec{0}$, which means To be continued ...


 we know that $\phi$ is injective and hence based on definition of injectivity, we have:
 
 $$ x_{i} \neq x_{j} \rightarrow \phi(x_{i}) \neq \phi(x_{j}) $$
 
 which means if at layer $l$, the optimal $W^{*}$ does not map $i,j$ samples, after applying $\phi$, they are not going to map to each other, so at layer $l+1$ the samples not in the same class have distance, hence there exist a projection down keep this distances positive, \textbf{if point are distinct, is there a projection that keep their distance positive, I need to think to prove it but it makes sence, because if there, we don't really need it becuase of the following}, There exist a $W$ at step $l+1$, which still keeps them apart and that is W that all is zero and the second column is all one, due to the gaussian feature map, second the features map in second dimension in RKHS is invertable meaning, if $x_{i} \neq x_{j}$ then that elements is not equal as well, hence projection through that dimension keeps their distance. Hence choosing this $W$ for $l+1$, have all the criterias for optimal solution in $\mathcal{E}_{l+1}$.
 
 Hence every solution in $\mathcal{E}_{l}$ is inside the solution of $\mathcal{E}_{l+1}$.
 
 
 
 End of proof.


\textbf{Proving there exist a certain projection in Gaussian feature map that is injetive:}


Pick $W$ to be projection of the first two dimension of Gaussian kernel.
\textbf{Claim: $\phi \circ W$ is injective}

\textbf{proof}

\begin{equation}
\begin{split}
    X_{1}\exp{X_{1}^{2}} = X_{2}\exp{X_{2}^{2}}
    \\
    \exp{X_{1}^{2}} = \exp{X_{2}^{2}}
    \\
    \rightarrow X_{1} = X_{2}
    \end{split}
\end{equation}


\newpage

\textbf{Proof of global monotonically non-decreasing}:







\textbf{Claim}: \textit{There exists $W_{l}$, where $\mathcal{E}_{l-1}$ = $\mathcal{E}_{l}$}.


If the claim is proven, the optimal solution at depth $l$ is consist of solutions at depth $l-1$, thus the optimal solution of depth $l$ is lower or equal than the optimal solution at depth $l-1$, meaning:

\begin{equation}
     ({\min} \quad
    \Tr(W^T A_= W ) - 
    \Tr(W^T A_{\ne} W)
    )_{l} \leq   ({\min} \quad
    \Tr(W^T A_= W ) - 
    \Tr(W^T A_{\ne} W)
    )_{l-1}
\end{equation}

Applying Lemma 2, we can conclude the following:
\begin{equation}
    \underset{f_l}{\max} \quad ||\text{Cov}(f_{l^\circ}(X), Y)||_F \geq
        ||\text{Cov}(f^*_{(l-1)^\circ}(X), Y)||_F.
\end{equation}

Hence the optimal $W$ for each depth induces a monotonically decreasing risk sequence. Furthermore the risk sequence is bounded from bellow by zero, thus the risk sequences is converging to its infimum. 



\textbf{Proof of the claim for the global case}:

For proving the claim we prove the following:

$$\exists W^{*} ,\,  \mathcal{E}_{l}(W_{1},\dots,W_{l-1},W^{*}) = \mathcal{E}_{l-1}(W_{1},\dots,W_{l-1})$$














Assume $W^{*} \in \mathcal{E}_{l} $. Matrix $A_{=}, A_{\neq}$ is positive semi definite, hence, $\Tr(W^T A_= W ),\Tr(W^T A_{\neq}W)$ is always a positive number, thus if the optimal solution $W^{*}$ exists in depth $l$ should satisfies that $\Tr(W^T A_= W ) = 0$ and $\Tr(W^T A_{\neq} W ) = \infty$.

\textbf{Studying the behavior of $\Tr(W^T A_= W ) = 0$}:
Again because $A_{=}$ is positive semi definite, $\Tr(W^T A_= W ) $ is only zero, if $ W^T A_= W   = \Vec{0}$, 

\begin{equation}
   W^T A_= W  = W^{T} \frac{1}{\sigma^2} \sum_{i,j \in \mathcal{S}} (r_i - r_j)(r_i - r_j)^T W =  \frac{1}{\sigma^2} \sum_{i,j \in \mathcal{S}} W^T (r_i - r_j)(r_i - r_j)^T W
\end{equation}
because every elements inside the summation $(r_i - r_j)(r_i - r_j)^T$ is positive semi definite matrix, hence, $W^T (r_i - r_j)(r_i - r_j)^T W = \Vec{0} , i,j \in \mathcal{S}$. Matrix $W$ can be seen through its columns $W = [W_{1},\dots,W_{q}]$, thus $W^T (r_i - r_j)(r_i - r_j)^T W = \Vec{0}$ becomes:

\begin{equation}
\begin{split}
    &W_{1}^T (r_i - r_j)(r_i - r_j)^T W_{1} = 0 \rightarrow W_{1}^T (r_i - r_j)(r_i - r_j)^T W_{1} W_{1}^{T} = 0 \rightarrow W_{1}^{T} A_{=}_{ij} = 0 \rightarrow A_{=}_{ij}^{T}W_{1} = A_{=}_{ij} W_{1} =0.
    \\
    .\\
    .\\
    .\\
   & W_{q}^T (r_i - r_j)(r_i - r_j)^T W_{q} = 0  = ||(r_i - r_j)^T W_{q}||_{2} = 0 \rightarrow (r_i - r_j)^T W_{q} = 0 \rightarrow r_i^{T} W_{q} = r_j^T W_{q}
    \end{split}
\end{equation}
Which means the in IDs space $r_{i}$ and $r_{j}$ get mapped to a same point through $W$ linear transformation for $i,j \in \mathcal{S}$.  

Assuming Gaussian feature map $\phi$, for $x_{i} = x_{j}$, after the nonlinear mapping, they mapped to the same point is RKHS space, meaning $\phi(x_{i}) = \phi(x_{j})$, and hence for the next depth $l+1$ adding any linear $W$ will still keep $i,j$ points on top of each other. Hence the We concluded that, if $W^{*} $ till layer $l$ satisfies $\Tr(W^T A_= W ) = 0$, adding any $W$ at layer $l+1$ will still keep this part of the objective the same.



\textbf{Studying the behavior of $\Tr(W^T A_{\neq} W ) >> 0$}:



With the same argument, we can use the fact that $A_{\neq}$ is semi positive definite, hence, $\Tr(W^T A_{\neq} W ) \neq 0$ is equivalent to $W^T A_{\neq} W  \neq \Vec{0}$, We can continue the same arguments and prove the following:

\begin{equation}
    W_{q}^T (r_i - r_j)(r_i - r_j)^T W_{q} >> 0 \rightarrow A_{\neq}_{ij} W_{q} >> 0 
\end{equation}

which corresponds to the largest eigenvalue.



 we know that $\phi$ is injective and hence based on definition of injectivity, we have:
 
 $$ x_{i} \neq x_{j} \rightarrow \phi(x_{i}) \neq \phi(x_{j}) $$
 
 which means if at layer $l$, the optimal $W^{*}$ does not map $i,j$ samples, after applying $\phi$, they are not going to map to each other, so at layer $l+1$ the samples not in the same class have distance, hence there exist a projection down keep this distances positive, There exist a $W$ at step $l$, which still keeps them apart and that is $W^{*} = [I_{q} 0]$, due to the gaussian feature map, as long as $q > 1$ we have a injective map, if $x_{i} \neq x_{j}$ then $\phi(x_{i}) \neq \phi(x_{j}) $, hence projection through that dimension keeps them distinct meaning in RKHS space composition of function till layer $l$ and after layer $l$ are geometrically equivalent, hence based on the corollary and theorem when $\simga \rightarrow \infty$, we have  $\mathcal{E}_{l} = \mathcal{E}_{l-1}$
 

 End of proof.


\textbf{Proving there exist a certain projection in Gaussian feature map that is injetive:}


Pick $W$ to be projection of the first two dimension of Gaussian kernel.
\textbf{Claim: $\phi \circ W$ is injective}

\textbf{proof}:

For $q>1$, we have the first two elements, hence:

\begin{equation}
\begin{split}
    X_{1}\exp{X_{1}^{2}} = X_{2}\exp{X_{2}^{2}}
    \\
    \exp{X_{1}^{2}} = \exp{X_{2}^{2}}
    \\
    \rightarrow X_{1} = X_{2}
    \end{split}
\end{equation}





\textbf{claim: The same proof works for local solution}

Picking $W_{l} = [I_{q},0]$, would makes $\phi \circ W_{l}$ injective. Hence if two points $x_{i}^{l-1}  \neq x_{j}^{l-1} $ then $\phi \circ W_{l}(x_{i}^{l-1} ) = x_{i}^{l}  \neq \phi \circ W_{l}(x_{j}^{l-1} ) = x_{j}^{l} $. Therefore the points samples that $x_{i}^{l-1}  = x_{j}^{l-1} $, we would have $\phi \circ W_{l}(x_{i}^{l-1} ) = \phi \circ W_{l}(x_{j}^{l-1} )$, and the point that are different would still be different. Hence 
\begin{align}
    \label{eq:p234}\forall x_{i}^{l-1} \neq x_{j}^{l-1}  \rightarrow r_{i} \neq r_{j} \rightarrow   ||W^Tr_i - W^Tr_j|| > 0  & 
    \rightarrow \lim_{\sigma \rightarrow 0}
    e ^{- \frac{||W^Tr_i - W^Tr_j||^2}{2 \sigma^2}} = 1\\
    \label{eq:p245}
    \forall x_{i}^{l-1}  = x_{j}^{l-1}  \rightarrow r_{i} = r_{j} \rightarrow   ||W^Tr_i - W^Tr_j|| = 0  & \rightarrow  
    \lim_{\sigma \rightarrow 0}
    e^{- \frac{||W^Tr_i - W^Tr_j||^2}{2 \sigma^2}} = 0.
\end{align}







%  \newpage



\newpage


\begin{definition}
Function $f,g : \mathbb{R}^{m} \rightarrow \mathbb{R}^{m}$ are geometrically equivalent iff:

\begin{equation}
    \forall x,y \in \mathbb{R}^{m}, d(f(x),f(y)) > 0 \Leftrightarrow  d(g(x),g(y))>0
\end{equation}

We show this, $f \approx_\textit{GE} g$
\end{definition}

\begin{theorem}
For function $W : \mathbb{R}^{m} \rightarrow \mathbb{R}^{m}$, if $W$ is injective: 

\begin{equation}
    W\circ f \approx_\textit{GE} f \approx_\textit{GE} f \circ W
\end{equation}


\end{theorem}
\begin{proof}
     \begin{equation}
   0 \sum_{i,j} \Gamma_{i,j}e ^{- \frac{||W^Tr_i - W^Tr_j||^2}{2 \sigma^2}} \quad 
     s.t \quad W^TW = I.
     \label{eq:proof help}
\end{equation}
\end{proof}

\begin{theorem} 
If $f \approx_\textit{GE} g$, $\forall \epsilon > 0$, $\exists \sigma_{0}$ which for $\forall \sigma \leq \sigma_{0}$ then:
\begin{equation}
|   || cov(f(x),Y)   ||_{F} - || cov(g(x),Y)   ||_{G} | \leq \epsilon
\end{equation}

\end{theorem}


\begin{corollary}
For injecive $W_{l}$,  $\exists \sigma_{0}$ which for $\forall \sigma \leq \sigma_{0}$ then:

$$ \epsilon_{l} \geq \epsilon_{l-1} $$
    
\end{corollary}




\begin{theorem}
Assume if: $|S^{c}| \geq 3$, then, $\forall i,j \in S$ 
$$Null(A_{ij}) \cap Span(A_{\neq}) \neq {0}$$
\end{theorem}

\begin{proof}

\textbf{Claim: $rank(A_{\neq}) > 1$}:

We prove this through contradiction. Assume  $rank(A_{\neq}) \leq 1$, so its either zero, or one. 

\begin{itemize}
    \item Case $rank(A_{\neq}) = 0$. We know that $A_{\neq} \geq 0$ hence, if the rank is zero, then $\forall  W \in \mathbb{R}^{m}$: 
    
    
    \begin{equation}
        \begin{split}
        A_{\neq}W = \sum_{i} \phi_{i}\phi_{i}^{T}W \rightarrow 
        \\
        W^{T}A_{\neq}W = \sum_{i} W^{T}\phi_{i}\phi_{i}^{T}W \rightarrow W^{T}\phi_{i}\phi_{i}^{T}W = 0 \forall i
        \\  \rightarrow W = \phi_{i} \phi_{i}^{T}\phi_{i}\phi_{i}^{T}\phi_{i} = |\phi_{i}|^{2}= 0 \rightarrow
        \phi_{i} = 0 \forall i
        \end{split}
    \end{equation}

which is a contradiction because that means:

$$\forall i,j \in S^{c}, r_i = r_j$$, which means everything are just one point.
    
 \item Case $rank(A_{\neq}) = 1$. 
 
 
 \begin{lemma}
     For $A = \sum_{i}^{n}  \phi_{i}\phi_{i}^{T}$, we have: 
     
     $$\textit{span}(A) = \textit{span}(\{\phi_{1},\dots,\phi_{n}\}) $$
     
\begin{proof}
     For any $W \in \mathbb{R}^{m}$ we have the following: 
     \begin{equation}
         A_{\neq} W= \sum_{i} \phi_{i}\phi_{i}^{T} W = \sum_{i} c_i \phi_{i}  
     \end{equation}
     where $c_{i} = \phi_{i}^{T} W$
\end{proof}     
     
 \end{lemma}
    
    Claim: Now Assuming $|S^{c}| \geq 3$, we have contradiction.
    
    assume the case $|S^{c}| = 3 $Choose three separate points from $S^{c}$, $r_{1},r_{2},r_{3}$ on the positive quarter of unit ball, without loss of generality assume choose $r_{1}$ to be the one with largest angle and $r_{3}$ with smallest. From previous lemma we know that span of $A_{\neq}$ is equal to $span \{(r_1 - r_2), (r_2 -r_3), (r_1-r_3)  \}$. having the condition that the rank is equal to one means that any vector $\{(r_1 - r_2), (r_2 -r_3), (r_1-r_3) \}$ can be represented as $\{(r_1 - r_3) \}$. In particular we have the following:
    
    \begin{equation}
    \begin{split}
        r_{1} - r_{2} =  \lambda_{1} (r_1 -r_3)
        \\
         r_{2} - r_{3} =  \lambda_{2} (r_1 -r_3)
    \end{split}
    \end{equation}
    
    Hence $r_{j} = r_{3}(1-\lambda_2) + \lambda_2 r_{1}$, because of the assumption that $r_{2}$ is between $r_{1}$ and $r_{3}$, hence we can assume $0<\lambda_2<1$. It is strict inequalities because the points are separate. Now we have the followings:
    
    \begin{equation}
    \begin{split}
        r_{2}^{T} r_{2} = ( r_{3}(1-\lambda_2) + \lambda_2 r_{1})^{T}( r_{3}(1-\lambda_2) + \lambda_2 r_{1}) 
        \\
         = 1 + 2\lambda_{2}^{2} - 2\lambda_2 + 2\lambda_2(1-\lambda_2) r_3^{T}r_{1} 
         \\ 
         < 1 + 2\lambda_{2}^{2} - 2\lambda_2 + 2\lambda_2(1-\lambda_2) = 1
    \end{split}
    \end{equation}

    which we used the fact that $ r_3^{T}r_{1}  < 1$ using the fact $r_{1} \neq r_3$. And $0<\lambda_2<1$. which is a contradiction due to the fact that the norm of $r_2$ is equal to one.
    
    

\end{itemize}


Hence this proves the claim that $rank(A_{\neq}) > 1$.


\begin{lemma}
    If $rank(A_{\neq}) > 1$ then, $\forall i,j \in S$:
    $$Null(A_{ij}) \cap Span(A_{\neq}) \neq \{0\}$$
\end{lemma}
    
    \begin{proof}
For $A_{ij} = (r_i-r_j)(r_i-r_j)^T$, hence it has a rank one, call the vector $r_i-r_j = \phi$. we have two cases 
\begin{itemize}
    \item $\phi\in span(A_{\neq})$: but the $span(A_{\neq})$ has more than element, hence other elements should be $null(A_{ij})$, hence $Null(A_{ij}) \cap Span(A_{\neq}) \neq \{0\}$. 
    \item $\phi\in null(A_{\neq})$, but the elements of $span(A_{\neq})$ should be in $null(A_{ij})$, hence $Null(A_{ij}) \cap Span(A_{\neq}) \neq \{0\}$. 
\end{itemize}       

So in either case the intersection is not empty.

    \end{proof}
    
    
This proves that for any elements $i,j \in S$, the intersection $Null(A_{ij}) \cap Span(A_{\neq}) \neq \{0\}$ has a non trivial element inside of it. 

\end{proof}








\begin{theorem}
For $|S^{c}| \geq 3$ then,$\exists W$, $\exists \sigma_{0}$ where $\forall \sigma \leq \sigma_{0}$ we have: 
    $$ \epsilon_{l} > \epsilon_{l-1} $$
\end{theorem}

\begin{proof}
     So
\end{proof}



\begin{corollary}
The global optimal solution can be reach in finite time solving greedy steps.
\end{corollary}


\end{appendices}



\newpage




\textbf{Aria's:}




\begin{theorem} For all $\sigma \leq \sigma_{0}$, $\exists W_{l}$
 
 \begin{equation}
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}}
    }_\text{1st term}
    -
    \underbrace{
    \sum_{i,j \in \mathcal{S}^c} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}} 
    }_\text{2nd term}
    \quad \geq \sum_{i,j \in \mathcal{S}\cup \mathcal{S}^{c}} \Gamma_{i,j} 
    r_{i}^{T}r_{j}
\end{equation}


\end{theorem}



\begin{proof}


Note that if any term from the last layer are mapped together, meaning $r_{i} = r_{j}$, then the LHS and RHS would be equal, so without loss of generality we can assume all the samples here are no equal, meaning $r_{i} \neq r_{j}$. For this proof assume we have two classes denoted as $\mathcal{S}^{1}, \mathcal{S}^{2}$.

\begin{lemma} For any $1>\mathcal{E} > 0$  ,$\exists \sigma_{0}$ that:

$$\forall i,j \quad r_{i}^Tr_{j} \leq \mathcal{E}$$

\end{lemma}

\begin{proof}

For previous kernel property, we know that:

$$<r_{i},r_{j}> = e^\frac{-|.|^2}{2\sigma ^2}$$
where $|.|$ is the distance before projecting to the RKHS space. We have finitely many of samples, hence there exists a maximum distance $|.|$ of them. Hence by choosing $\sigma_{0} = \sqrt{\frac{-|.|}{2\ln{\mathcal{E}}}}$, we conclude the proof of the lemma.

\end{proof}


Hence based on the lemma the upper bound of RHS is: 

\begin{equation}
    \sum_{i,j \in \mathcal{S}\cup \mathcal{S}^{c}} \Gamma_{i,j}
    r_{i}^{T}r_{j} \leq \mathcal{E} \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} -  \sum_{i,j \in \cup \mathcal{S}^{c}} \Gamma_{i,j} \leq \mathcal{E} \sum_{i,j \in \mathcal{S}} \Gamma_{i,j}
\end{equation}


Hence we need to prove the following: 


 \begin{equation}
    \underbrace{ 
    \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}}
    }_\text{1st term}
    -
    \underbrace{
    \sum_{i,j \in \mathcal{S}^c} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}} 
    }_\text{2nd term}
    \quad \geq \mathcal{E} \sum_{i,j \in \mathcal{S}} \Gamma_{i,j}
\end{equation}


\textbf{First term}:

By decreasing the $\sigma_{0}$, the $<r_{i},r_{j}>$ approaches to zero, meaning they become almost orthogonal.

hence there exist a finite orthogonal axis $\{e_{1},\dots, e_{n}\}$, where $n$ is the number of samples. and we have the following property:

\begin{lemma}
\begin{equation}
    \forall i,j <e_{i},r_{i}> \geq 1-\mathcal{E} , <e_{i},r_{j}> \leq \mathcal{E}.
\end{equation}
\end{lemma}

\begin{equation}
    \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}}
   = \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}}
   + \sum_{i,j \in \mathcal{S}^2} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}}
\end{equation}

pick $W =  \sum_{i\in \mathcal{S}^1}e_{i}$. Hence we have:


\begin{equation}
    \lim_{\mathcal{E} \longrightarrow 0}   \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}} = \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2}{2\sigma^2}}
\end{equation}

and for $\mathcal{S}^2$:

\begin{equation}
    \lim_{\mathcal{E} \longrightarrow 0}   \sum_{i,j \in \mathcal{S}^2} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}} = \sum_{i,j \in \mathcal{S}^2} \Gamma_{i,j} 
    e^{-\frac{0}{2\sigma^2}} = \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
\end{equation}

For $\mathcal{S}^c$

\begin{equation}
    \lim_{\mathcal{E} \longrightarrow 0}   \sum_{i,j \in \mathcal{S}^c} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}} = \sum_{i,j \in \mathcal{S}^c} \Gamma_{i,j} 
    e^{-\frac{1}{2\sigma^2}}
\end{equation}


\begin{lemma} We have the following:
\begin{equation}
    \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2}{2\sigma^2}} + \sum_{i,j \in \mathcal{S}^1}  \Gamma_{i,j} - \sum_{i,j \in \mathcal{S}^c} \Gamma_{i,j} 
    e^{-\frac{1}{2\sigma^2}} \geq \mathcal{E} \sum_{i,j \in \mathcal{S}} \Gamma_{i,j}
\end{equation}

\end{lemma}
\begin{proof}

Taking things to one side would gives us the following: 

\begin{equation}
         \sum_{i,j \in \mathcal{S}^1}  \Gamma_{i,j} \geq \mathcal{E} \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} -  \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2}{2\sigma^2}} + \sum_{i,j \in \mathcal{S}^1}  + \sum_{i,j \in \mathcal{S}^c} \Gamma_{i,j} 
    e^{-\frac{1}{2\sigma^2}}
\end{equation}

The LHS is a positive number, and the RHS can be controlled to be arbitrary close to zero by making $\sigma$ of this layer and $\mathcal{E}$ small.  
\end{proof}




\begin{lemma}
    \begin{equation}
    \begin{split}
        \lim_{\mathcal{E} \longrightarrow 0}  ( \sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}} +   &\sum_{i,j \in \mathcal{S}^c} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}} +   \sum_{i,j \in \mathcal{S}^c} \Gamma_{i,j} 
    e^{-\frac{(r_i-r_j)^TW_l W_l^T(r_i-r_j)}{2\sigma^2}} ) =
    \\
    &\sum_{i,j \in \mathcal{S}^1} \Gamma_{i,j} 
    e^{-\frac{2}{2\sigma^2}} + \sum_{i,j \in \mathcal{S}^2}  \Gamma_{i,j} - \sum_{i,j \in \mathcal{S}^c} \Gamma_{i,j} 
    e^{-\frac{1}{2\sigma^2}}
    \end{split}
    \end{equation}
    
    because every part of the RHS is continuous function of $\mathcal{E}$, hence we can get arbitrary close to the LHS.
    
\end{lemma}




Lets call the LHS of lemma 4 as $f_1$, ad RHS of it as $l_1$, and the RHS of lemma 3 as $l_2$.

We want to prove that $f_1 \geq l_2$. From lemma 3 we prove that we can make $f_1 - l_2> \delta >0$, in fact we make it as large as $ \sum_{i,j \in \mathcal{S}^2}  \Gamma_{i,j}$. From lemma 4 we know that we can make $|f_1-l_1|< \delta/3 $. hence we have $l_1 - l_2 > 2*\delta/3 > 0$. Hence the proof is compelte. 





\end{proof}


\newpage

==> appendices/d_app_4.tex <==
%\begin{appendices}
%\section{Proof for Property \ref{prop:kernel_in_RKHS} and \ref{prop:kernel_in_IDS}}
%\label{app:kernel_define_metric_in_IDS}
%\begin{proof}
%From Appendix~\ref{app:ccn_satisfies_dependence_property}, we concluded that HSIC can be rewritten into the equation that satisfies the \textit{separability property} where we optimize   
%     \begin{equation}
%        \underset{W}{\max} \quad \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} 
%        \langle \Psi(W^Tx_i), \Psi(W^Tx_j) \rangle - 
%        \sum_{i,j \in \bar{\mathcal{S}}}
%        \Gamma_{i,j} 
%        \langle \Psi(W^Tx_i), \Psi(W^Tx_j) \rangle
%        \hspace{0.2cm} \text{s.t} \hspace{0.2cm} W^TW = I.
%        \label{eq:inner_controls_the_metric}
%    \end{equation}   
%From Eq.~(\ref{eq:inner_controls_the_metric}), we see that the inner product is always used as the metric in RKHS. However, if the kernel is written as a function, it is also equivalent to 
%     \begin{equation}
%        \underset{W}{\max} \quad \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} 
%        \kappa(W^Tx_i, W^Tx_j)  - 
%        \sum_{i,j \in \bar{\mathcal{S}}}
%        \Gamma_{i,j} 
%        \kappa(W^Tx_i, W^Tx_j)
%        \hspace{0.2cm} \text{s.t} \hspace{0.2cm} W^TW = I.
%        \label{eq:inner_controls_the_IDS}
%    \end{equation}   
%Since Eq.~(\ref{eq:inner_controls_the_IDS}) reflects the result in IDS, the kernel function directly controls how the distance between samples are measured. Given this control, it defines the metric which satisfies the \textit{separability property}.
%\end{proof}
%\end{appendices}

==> appendices/e_HSIC_as_CE.tex <==
\begin{appendices}
\section{Proof for Corollary \ref{corollary:mse} and \ref{corollary:ce}}
\label{app:corollary:ce}

\textbf{Corollary} \ref{corollary:mse}: 
    \textit{Given $\hsic_l \rightarrow \hsic^*$, the network output in IDS solves MSE via a translation of labels.}
   
\begin{proof} \hspace{1pt}
\begin{adjustwidth}{0.5cm}{0.0cm}
    As $\hsic_l \rightarrow \hsic^*$, Thm.~\ref{thm:geometric_interpret} shows that sample of the same class are mapped into the same point. Assuming that $\fm$ has mapped the sample into $c$ points $\alpha = [\alpha_1, ..., \alpha_c]$ that's different from the truth label
    $\xi = [\xi_1, ..., \xi_c]$. Then the $\mse$ objective is minimized by translating the $\fm$ output by 
    \begin{equation}
        \xi - \alpha.
    \end{equation}
\end{adjustwidth}
\end{proof}

\textbf{Corollary} \ref{corollary:ce}: 
    \textit{Given $\hsic_l \rightarrow \hsic^*$, the network output in RKHS solves $\ce$ via a change of bases.}
    
\textbf{Assumptions, and Notations. }
\begin{enumerate}
    \item  
        $n $ is the number of samples.
    \item
        $\nclass$ is the number of classes.
    \item
        $y_i \in \mathbb{R}^{\nclass}$ is the ground truth label for the $i^{th}$ sample. It is one-hot encoded where only the $j^{th}$ element is 1 if $x_i$ belongs to the $j^{th}$ class, all other elements would be 0.
    \item
        We denote $\fm$ as the network, and $\hat{y}_i \in \mathbb{R}^{\nclass}$ as the network output where $\hat{y}_i = \fm(x_i)$. We also assume that $\hat{y}_i$ is constrained on a probability simplex where $1 = \hat{y}_i^T \mathbf{1}_n$.
    %\item
    %    We denote $\fm_{\hsic}$ as a network using $\hsic$ as the objective, and $\hat{z}_i \in \mathbb{R}^{\nclass}$ as the network output where $\hat{z}_i = \fm_{\hsic}(x_i)$. 
    %\item
    %    We denote the $j^{th}$ element of $z_i$, $y_i$, and $\hat{y}_i$ as $z_i$, $y_{i,j}$ and $\hat{y}_{i,j}$ respectively.
    \item
        We denote the $j^{th}$ element of $y_i$, and $\hat{y}_i$ as $y_{i,j}$ and $\hat{y}_{i,j}$ respectively.
    \item
        We define
    \begin{addmargin}[1em]{2em}% 1em left, 2em right
    \textbf{Orthogonality Condition: }
        A set of samples $\{\hat{y}_1, ..., \hat{y}_n\}$ satisfies the orthogonality condition if
        \begin{equation} 
        \begin{cases}
        \langle \hat{y_{i}}, \hat{y_{j}}\rangle =1 & \forall\quad i,j \textrm{ same class} \\
        \langle \hat{y_{i}}, \hat{y_{j}}\rangle=0 & \forall\quad i,j \textrm{ not in the same class}
        \end{cases}.
        \end{equation}
    \end{addmargin}
    \item
        We define the Cross-Entropy objective as 
        \begin{equation}
        \underset{\fm}{\argmin} -\sum_{i=1}^{n} \sum_{j=1}^{\nclass} y_{i,j} \log(\fm(x_{i})_{i,j}).
        \end{equation}
    \end{enumerate}
\begin{proof}\hspace{1pt}
\begin{adjustwidth}{0.5cm}{0.0cm}
From Thm.~\ref{thm:geometric_interpret}, we know that the network $\fm$ output, $\{ \hat{y}_1, \hat{y}_2, ..., \hat{y}_n \}$,  satisfy the orthogonality condition at $\hsic^*$. Then there exists a set of  orthogonal bases represented by $\Xi = [\xi_1, \xi_2, ..., \xi_c]$ that maps $\{ \hat{y}_1, \hat{y}_2, ..., \hat{y}_n \}$ to simulate the output of a softmax layer. Let $\xi_{i} = \hat{y}_{j} , j\in \cS^{i}$, i.e., for the $i_{th}$ class we arbitrary choose one of the samples from this class and assigns $\xi_i$ of that class to be equal to the sample's output. Realize in our problem we have $<\hat{y}_{i},\hat{y}_{i}> = 1$, so if $<\hat{y}_{i},\hat{y}_{j}> = 1$, then subtracting these two would lead to $<\hat{y}_{i},\hat{y}_{i}-\hat{y}_{j}> = 0$, which is the same as $\hat{y}_{i}=\hat{y}_{j}$.
So this representation is well-defined and its independent of choices of the sample from each group if they satisfy orthogonality condition.
Now we define transformed labels, $Y$ as:
\begin{equation}
    Y = \hat{Y} \Xi.
\end{equation}
Note that $Y = [y_1, y_2, ..., y_n]^T$ which each $y_{i}$ is a one hot vector representing the class membership of $i$ sample in $c$ classes.
Since given $\Xi$ as the change of basis, we can match $\hat{Y}$ to $Y$ exactly, $\ce$ is minimized.
\end{adjustwidth}
\end{proof}
\end{appendices}




==> appendices/e_app_5.tex <==
\begin{appendices}
\section{KNet's Relationship to Information Bottleneck}
\label{app:theorem_information_bottleneck}

Representing a layer from the HSIC perspective is descriptive of its objective mechanically. Namely, it can be visualized that it is finding the weights $W_l$ to map into the IDS such that when it is mapped back to RKHS, the new representation possesses a maximal dependence on the labels. While this understanding explains the network process mechanically, there also exists a strong relationship to information theory. 

Here, let $P(X)$ and $P(Y)$ be the probability distribution for samples for $X$ and $Y$. From statistics, besides the correlation index, dependence can also be measured by the distance between $P(X)P(Y)$ to $P(X,Y)$, where a distance of 0 implies a complete independence between $X$ and $Y$. In information theory, this dependence is measured by the Mutual Information (MI) where the distance between $P(X)P(Y)$ to $P(X,Y)$ is measured by KL divergence. Therefore, when the mutual information between $X$ and $Y$ is maximized, the statistical dependence between $P(X)$ and $P(Y)$ is also maximized. 

HSIC is related to MI in that it also measures the distances between $P(X)P(Y)$ and $P(X,Y)$. However, instead of using KL divergence, HSIC uses a metric called Maximal Mean discrepancy (MMD). Therefore, when we maximize the HSIC of a layer output to its labels, we are simultaneously discovering a mapping where the distribution of its images is highly dependent on the labels. 

By establishing the relationship between HSIC and MI, an MLP using Eq.~(\ref{eq:hsic_obj_pure}) can be interpreted as an information bottleneck (IB) defined by \citet{tishby2000information}, i.e., the network compresses the data while filtering out information unrelated to the labels. Here, we provide a short proof of this relationship.

\begin{proof}
\citet{tishby2000information} defined relevant information in signal $x \in X$ as being the information that this signal provides about another signal $y \in Y$. The information bottleneck concept compresses $x$ into $\hat{x}$ such that $\hat{x}$'s information about $y$ is maximally retained. They measure this minimally sufficient amount of information through the information bottleneck formulation where they maximize

\begin{equation}
    \underset{\hat{X}}{\max} \quad MI(\hat{X}, Y) - \beta MI(\hat{X}, X). 
     \label{eq:information_bottleneck}
\end{equation}

Since HSIC also measure the distance between distributions, by changing KL divergence to MMD, each layer can be defined by the same information bottleneck rewritten into 

\begin{equation}
    \underset{W}{\max} \quad HSIC(R_{l-1}W, Y) - \beta HSIC(R_{l-1}W, R_{l-1}),
     \label{eq:HSIC_information_bottleneck}
\end{equation}

or

\begin{equation}
    \underset{W}{\max} 
    \hspace{0.2cm}
    \Tr(K_{R_{l-1}W} HK_YH) - \beta \Tr(K_{R_{l-1}W} H K_{R_{i}}H).
\end{equation}

Applying the property of trace to sum two terms, it then becomes 

\begin{equation}
    \underset{W}{\max} 
    \hspace{0.2cm}
    \Tr(K_{R_{l-1}W} H(K_Y-\beta K_{R_{i}})H).
\end{equation}

We next take the Cholesky decomposition and get $\hat{Y} \hat{Y}^T = H(K_Y-\beta K_{R_{i}})H$, the formulation again reduces down to the proposed HSIC formulation of 

\begin{equation}
    \underset{W}{\max} 
    \hspace{0.2cm}
    HSIC(R_{l-1}W, \hat{Y}),
\end{equation}

where the definition of a label $\hat{Y}$ now includes the input information. This suggests that by adjusting the label definition of the HSIC formulation, MLP acts as a information bottleneck if the distances between distributions are measured by MMD.


\end{proof}
\end{appendices}




==> appendices/f_HSIC_as_MSE.tex <==
\begin{appendices}
\section{Proof for Theorem \ref{thm:HSIC_as_MSE}}
\label{app:theorem_3_proof}
\textbf{Theorem} \ref{thm:HSIC_as_MSE}
\textit{The argmin of the MSE objective is satisfied by the argmax of the HSIC objective if the final $\Psi$ is discarded to produce an output in IDS.} 

\subsection{Assumptions and Notations of the Proof}
Given $\mathcal{S}$ and $\mathcal{S}^c$ as sets of all pairs of samples of $(x_i,x_j)$ from a dataset $X$ that belongs to the same and different classes respectively. We let $c$ be the number of classes and let $\Gamma_{i,j}$ be a set of  scalars derived from the labels following Lemma~\ref{lemma:lemma1}.

We prove this theorem by breaking the proof into three lemmas. 
Previously in Appendix~\ref{app:theorem_2_proof}, we have denoted $\hat{y}_i$ as the output of a layer after the activation function. We have specifically emphasized that $\hat{y}_i$ resides within RKHS. Here we denote the output of a layer for $x_i$ as $\hat{z}_i$  where the output is the point after the linear transformation $W$ \textit{prior} to the activation function, i.e., $W^T x_i = \hat{z}_i$. Therefore, although we are looking at the same formulation, we now focus on what is happening within IDS as HSIC is being optimized. Following this notation, we denote $z_i$ as the ground truth label for the sample $x_i$. 

\subsection{Summary the Proof}
To summarize the proof, we first prove in Lemma~\ref{lemma:mse_min_condition} that the MSE is minimized if and only if 

\[
\ \begin{cases}
 (\hat{z_{i}} - \hat{z_{j}})^2 = 0 & \textrm{if}\quad i,j \textrm{ same class} \\
 (\hat{z_{i}} - \hat{z_{j}})^2 \ne 0  & \textrm{if}\quad i,j \textrm{ not in the same class}
\end{cases}.
\]

In Lemma~\ref{lemma:HSIC_mse_opt_condition}, we show that that the HSIC objective using a Gaussian kernel is optimized if and only if  

\[
\ \begin{cases}
 (\hat{z_{i}} - \hat{z_{j}})^2 = 0 & \textrm{if}\quad i,j \textrm{ same class} \\
 (\hat{z_{i}} - \hat{z_{j}})^2 = 2& \textrm{if}\quad i,j \textrm{ not in the same class}
\end{cases}.
\]

Finally, in Lemma~\ref{lemma:HSIC_satisfies_MSE}, we draw from Lemma~\ref{lemma:mse_min_condition} and \ref{lemma:HSIC_mse_opt_condition} to show since the solutions space using the HSIC objective is a subset within the solution space using MSE, a solution that solves the HSIC objective must also satisfy MSE.



\subsection{Lemmas of the Proof}
\begin{lemma}\label{lemma:mse_min_condition}
The MSE is minimized if and only if 

\[
\ \begin{cases}
 (\hat{z_{i}} - \hat{z_{j}})^2 = 0 & \textrm{if}\quad i,j \textrm{ same class} \\
 (\hat{z_{i}} - \hat{z_{j}})^2 \ne 0  & \textrm{if}\quad i,j \textrm{ not in the same class}
\end{cases}.
\]
\end{lemma}

\begin{proof}
First, we assume that the MSE objective is already optimized, this implies that the output must satisfy $\hat{z}_i = z_i$ for any sample. Since $z_i = z_j$ for all samples of the same class, the condition $\hat{z}_i = \hat{z}_j$ must also be satisfied. As for the 2nd condition of $(\hat{z_{i}} - \hat{z_{j}})^2 \ne 0$ when $i,j$ are not in the same class, this is immediately satisfied by the definition of classification by MSE. 

Conversely, we next assume that $(\hat{z_{i}} - \hat{z_{j}})^2 = 0$ if sample pair $(x_i, x_j)$ are in the same class, and $(\hat{z_{i}} - \hat{z_{j}})^2 \neq 0$ if they are in different classes. This implies that all samples are mapped onto $c$ distinct points. Since MSE is a supervised problem, the labels can then be easily matched to one of the $c$ distinct points such that for each sample $\hat{z}_i$ we get $z_i = \hat{z}_i$. From here, it can be easily seen that the MSE objective is minimized to 0.

\begin{equation}
    0 = \sum_{i,j \in \mathcal{S}} (z_i - \hat{z}_i)^2 
\end{equation}
\end{proof}


\begin{lemma}\label{lemma:HSIC_mse_opt_condition}
The HSIC objective is optimized if and only if 

\[
\ \begin{cases}
 (\hat{z_{i}} - \hat{z_{j}})^2 = 0 & \textrm{if}\quad i,j \textrm{ same class} \\
 (\hat{z_{i}} - \hat{z_{j}})^2 = 2 & \textrm{if}\quad i,j \textrm{ not in the same class}
\end{cases}.
\]
\end{lemma}

\begin{proof}
First we assume that the HSIC objective using a Gaussian kernel is already optimized. This yields the optimal parameters for the MLP where

\begin{equation}
    \theta^* = 
    \underset{\theta}{\argmax} \quad \sum_{i,j} \Gamma_{i,j}e ^{-\gamma||g_\theta(x_i) - g_\theta(x_j)||^2}. 
     \label{eq_app:hsic_obj_with_gaussian_4}
\end{equation}

Applying Lemma~\ref{lemma:lemma1}, when $\Gamma_{i,j} > 0$  
the objective is maximized when $g_\theta$ forces $||g_\theta(x_i) - g_\theta(x_j)||^2$ towards 0. Conversely, when $\Gamma_{i,j} < 0$, $g_\theta$ will push $||g_\theta(x_i) - g_\theta(x_j)||$ towards the diameter of the solutions space. Here, by using the Gaussian kernel, we know that the maximum distance between two unit vectors is $\sqrt{2}$. By appropriately setting $\gamma$, we can ensure that 
\begin{equation}
    e^{-2\gamma } \approx 0.
\end{equation}

Converse, if we assume that $(\hat{z_{i}} - \hat{z_{j}})^2 = 0$ for all $(x_i,x_j)$ sample pairs in the same class and $(\hat{z_{i}} - \hat{z_{j}})^2 = \sqrt{2}$ for samples from different classes, if we plug these conditions into Eq.~(\ref{eq_app:hsic_obj_with_gaussian_4}) then
\begin{equation}
    \sum_{i,j \in \mathcal{S}} \Gamma_{i,j} = 
    \underset{\theta}{\max} \quad \sum_{i,j} \Gamma_{i,j}e ^{-\gamma(g_\theta(x_i) - g_\theta(x_j))^2}. 
     \label{eq_app:hsic_obj_with_gaussian_6}
\end{equation}
 
 Since $\sum_{i,j \in \mathcal{S}} \Gamma_{i,j}$ is the absolute upper bound for Eq.~(\ref{eq_app:hsic_obj_with_gaussian_6}), this solution must also be the optimal. 
 
\end{proof}

\begin{lemma}\label{lemma:HSIC_satisfies_MSE}
The the optimal condition of the MSE objective is satisfied if the HSIC objective is optimized.
\end{lemma}

\begin{proof}
When solving MSE, the labels can be anywhere. As long as different labels are distinguishable from each other, the distance between samples of different classes is not part of the objective. 

For HSIC since the distance between samples is part of the objective, the labels must be exactly $\sqrt{2}$ apart at an optimal solution. Therefore, the HSIC solution is a specific case of the MSE solution space.

We let the argmin solution space of MSE be $\mathcal{M}$ and the argmax solution space of HSIC be $\mathcal{H}$, then $\mathcal{H} \subset \mathcal{M}$. Therefore, a solution within $\mathcal{H}$ must also be a solution within $\mathcal{M}$. Which lead us to conclude that the argmax of the HSIC objective must also satisfy the MSE objective. 
\end{proof}
\end{appendices}



==> appendices/g_properties.tex <==
\begin{appendices}
\section{Proof for Property \ref{prop:pulling_samples_together}}
\label{app:optimizing_IDS}

\begin{proof}
Given $\Gamma = HYY^TH$ and assuming that we use the traditional Gaussian kernel for $\Psi$, then at each layer, the objective becomes 
\begin{equation}
    \underset{W}{\max} \quad \sum_{i,j} \Gamma_{i,j}e ^{-\gamma(W^Tx_i - W^Tx_j)^2} \hspace{0.2cm}
     \text{s.t} \hspace{0.2cm} W^TW = I.
     \label{eq:hsic_obj_with_gaussian_2}
\end{equation}
By applying Lemma~\ref{lemma:lemma1}, the HSIC objective is maximized when $(W^Tx_i - W^Tx_j)=0$ for all $(x_i,x_j)$ samples of the same class, and $(W^Tx_i - W^Tx_j)$ is maximized for pairs in different classes. Notice that these results come after applying the input by $W$, therefore, these observations are happening in the IDS.
\end{proof}
\end{appendices}

\begin{appendices}
\section{Proof for Property \ref{prop:align_samples_together}}
\label{app:optimizing_RKHS}
\begin{proof}
We first note that Eq.~(\ref{eq:hsic_obj_with_gaussian_2}) can also be written as 
\begin{equation}
    \underset{W}{\max} \quad \sum_{i,j} \Gamma_{i,j} \langle 
    \psi(W^Tx_i), \psi(W^T x_j) \rangle, 
     \hspace{0.2cm} \text{s.t} \hspace{0.2cm} W^TW = I.
     \label{eq:hsic_obj}
\end{equation}
Assuming the conditions defined in Lemma~\ref{lemma:lemma1}, HSIC is optimized when the angular distance is pushed towards 0 and $\pi/2$.  Therefore, the Gaussian kernel pushes samples to become perfectly aligned or orthogonal on a unit hypersphere in RKHS. 
\end{proof}
\end{appendices}


%\begin{appendices}
%\section{Example of Using the Polynomial Kernel}
%\label{app:using_polynomial_kernel}
%\begin{proof}
%Using the polynomial kernel, the HSIC objective can be rewritten as 
%\begin{equation}
%    \underset{W}{\max} \quad \sum_{i,j} \Gamma_{i,j} (x_i^TW W^Ty_j + 1)^2. 
%     \label{eq:hsic_obj_with_poly}
%\end{equation}
%Following the same logic from the Gaussian kernel, we see that when two samples are in the same class, the optimal $W_l$ for the polynomial kernel pushes samples to be angularly aligned. However, when the samples are in different classes, $W_l$ will push the samples to points in opposite directions. Therefore, the polynomial kernel uses angular distance as the metric in IDS. This points to an interesting observation. Namely, that the kernel function defines the metric of similarity in IDS. However, once the samples are projected into RKHS, the inner product is always used as the metric. 
%\end{proof}
%\end{appendices}

==> appendices/h_app_8.tex <==
%\begin{appendices}
%\section{Details on SPCA and Kernelized SPCA}
%\label{app:SPCA_SKPCA}
%Supervised PCA is also based on an HSIC formulation where we perform dimension reduction within RKHS with
%\begin{equation}
%    \underset{W}{\max} \quad \Tr( \Psi W W^T \Psi^T H K_Y H)
%    \hspace{1cm} \text{s.t} \hspace{1cm} W^TW = I, 
%     \label{eq:hsic_trace_with_SPCA}
%\end{equation}
%where $\Psi$ is the image of the data mapped into RKHS. With this formulation, we seek to find the low dimension subspace that is maximally dependent on the labels Y. By applying the rotation property of the Trace operator, this equation can be reformulated into
%\begin{equation}
%    \underset{W}{\max} \quad \Tr( W^T \Psi^T H K_Y H \Psi W)
%    \hspace{1cm} \text{s.t} \hspace{1cm} W^TW = I. 
%\end{equation}
%Since $\Psi$ may potentially have infinite dimensions dependent on the kernel choice, the original Supervised PCA used a linear kernel where $\Psi = X$. Therefore, given the application of Random Fourier Feature to approximate potentially infinite dimensions, $\Psi$ becomes a finite dimension matrix; thereby enabling the feasibility of its computation. To solve this problem, the solution is simply the most dominant eigenvectors of the matrix $\Psi^THK_YH\Psi$.
%\end{appendices}

==> appendices/i_app_9.tex <==
\begin{appendices}
\section{ISM Algorithm}
\label{app:ISM Algorithm}

To define $\Phi$, we must first define $\Psi$ and $\mathcal{L}_\Psi$. If we let $\odot$ be the Hadamard product between matrices, then $\Psi = \Gamma \odot K_{XW}$. Given $\Psi$, we define $D_\Psi$ and $\mathcal{L}_{\Psi}$ respectively as the degree matrix and the Laplacian of $\Psi$ where $D_\Psi=\text{Diag}(\Psi 1_n)$ and $\mathcal{L}_\Psi = D_\Psi - \Psi$. Having the key notations defined, the $\Phi$ matrix associated with the Gaussian kernel is defined as
    \begin{equation}
        \Phi=-X^T\mathcal{L}_{\Psi} X.
        \label{eq:def_phi}
    \end{equation}
Since $\Phi$ associated with the Gaussian kernel is itself a function of $W$, an approximation of $\Phi$ via the 2nd order Taylor expansion produces an $\Phi_0$ independent of $W$ defined as
    \begin{equation}
        \Phi_0=-X^T \mathcal{L}_{\Gamma} X.
    \end{equation}
Since the Laplacian matrix based on $\Gamma$ no longer require $W$, an initial $W_0$ can be used 
for Eq.~(\ref{eq:def_phi}) to obtain $W_1$. By follow this pattern, ISM iteratively use $W_i$ to find $W_{i+1}$ until convergence. While this work focuses on the Gaussian kernel, we include the $\Phi/\Phi_0$ equation for other kernels in Tables~\ref{table:init_phis} and \ref{table:phis}. The ISM algorithm is also included in Algorithm~\ref{alg:ism}.

For convergence, we can converge when the Frobenius Norm $||W_i - W_{i-1}||_F$ falls below a predefined threshold $\delta$. However, based on the ISM algorithm, they found that in practice, the comparison of the most dominant eigenvalues is faster.

\begin{table}[h]   
\begin{minipage}{2.4in}
    \footnotesize
      \begin{tabular}{c|l}
        Kernel & Approximation of $\Phi$s\\
        \midrule
            Linear
            	& $\Phi_0=X^T\Gamma X$ \\
            Squared
            	& $\Phi_0=X^T \mathcal{L}_{\Gamma} X$ \\  
            Polynomial
            	& $\Phi_0=X^T \Gamma X$\\
            Gaussian
            	& $\Phi_0=-X^T \mathcal{L}_{\Gamma} X$\\
            Multiquadratic
            	& $\Phi_0=X^T\mathcal{L}_{\Gamma} X$\\
            \bottomrule       
      \end{tabular}
      \caption{Equations for the approximate \\$\Phi$s for the common kernels.}
      \label{table:init_phis}
\end{minipage}
\begin{minipage}{2in}
    \footnotesize
      \begin{tabular}{c|l}
        Kernel & $\Phi$ Equations\\
        \midrule
            Linear
            	& $\Phi=X^T\Gamma X$ \\
            Squared
            	& $\Phi=X^T \mathcal{L}_{\Gamma}X$ \\  
            Polynomial
            	& $\Phi=X^T\Psi X$ 
             	\hspace{0.2cm}
            	,
            	\hspace{0.2cm}           	
            	$\Psi = \Gamma \odot K_{XW,p-1}$ \\ 
            Gaussian
            	& $\Phi=-X^T\mathcal{L}_{\Psi} X$ 
            	,
            	$\Psi = \Gamma \odot K_{XW}$\\
            Multiquadratic
            	& $\Phi=X^T\mathcal{L}_{\Psi} X$ 
            	,
            	$\Psi = \Gamma \odot K_{XW}^{(-1)}$\\ 
        \bottomrule       
      \end{tabular}
      \caption{Equations for $\Phi$s for the common kernels.}
      \label{table:phis}
\end{minipage}
\end{table}

%\begin{table}[h]   
%    \centering
%      \begin{tabular}{c|l}
%        Kernel & Approximation of $\Phi$s\\
%        \midrule
%            Linear
%            	& $\Phi_0=X^T\Gamma X$ \\
%            Squared
%            	& $\Phi_0=X^T \mathcal{L}_{\Gamma} X$ \\  
%            Polynomial
%            	& $\Phi_0=X^T \Gamma X$\\
%            Gaussian
%            	& $\Phi_0=-X^T \mathcal{L}_{\Gamma} X$\\
%            Multiquadratic
%            	& $\Phi_0=X^T\mathcal{L}_{\Gamma} X$\\
%            \bottomrule       
%      \end{tabular}
%      \caption{Equations for approximate $\Phi$s for the common kernels.}
%      \label{table:init_phis}
%\end{table}
%
%\begin{table}[h]
%    \centering
%    \begin{tabular}{c|l}
%      Kernel & $\Phi$ Equations\\
%      \midrule
%          Linear
%          	& $\Phi=X^T\Gamma X$ \\
%          Squared
%          	& $\Phi=X^T \mathcal{L}_{\Gamma}X$ \\  
%          Polynomial
%          	& $\Phi=X^T\Psi X$ 
%           	\hspace{0.2cm}
%          	,
%          	\hspace{0.2cm}           	
%          	$\Psi = \Gamma \odot K_{XW,p-1}$ \\ 
%          Gaussian
%          	& $\Phi=-X^T\mathcal{L}_{\Psi} X$ 
%          	,
%          	$\Psi = \Gamma \odot K_{XW}$\\
%          Multiquadratic
%          	& $\Phi=X^T\mathcal{L}_{\Psi} X$ 
%          	,
%          	$\Psi = \Gamma \odot K_{XW}^{(-1)}$\\ 
%      \bottomrule       
%    \end{tabular}
%    \caption{Equations for $\Phi$s for the common kernels.}
%    \label{table:phis}
%\end{table}


    \begin{algorithm}[H]
    \footnotesize
     \textbf{Input :} Data $X$, kernel, Subspace Dimension $q$\\ \textbf{Output :} Projected subspace $W$ \\
     \textbf{Initialization :} Initialize $\Phi_0$ using Table~\ref{table:init_phis}.\\ Set $W_0$ to $V_{\text{max}}$ of $\Phi_0$.\\
     \While{$||\Lambda_i - \Lambda_{i-1}||_2/||\Lambda_i||_2 < \delta$ }{
        Compute $\Phi$ using Table~\ref{table:phis}\\
        Set $W_k$ to $V_{\text{max}}$ of $\Phi$
     }
     \caption{ISM Algorithm}
     \label{alg:ism}
    \end{algorithm}    

\end{appendices}

==> appendices/j_app_a_dataset.tex <==
\newpage
\begin{appendices}
\section{Dataset Details}
\label{app:data_detail}

No samples were excludes from any of the dataset. 

\textbf{Wine. } 
    This dataset has 13 features, 178 samples, and 3 classes. The features are continuous and heavily unbalanced in magnitude. The dataset can be downloaded at \url{https://archive.ics.uci.edu/ml/datasets/wine.}
    

 \textbf{Divorce. } 
    This dataset has 54 features, 170 samples, and 2 classes. The features are discrete and balanced in magnitude.  The dataset can be downloaded at \url{https://archive.ics.uci.edu/ml/datasets/Divorce+Predictors+data+set.}
    
 \textbf{Car. } 
     This dataset has 6 features, 1728 samples and 2 classes. The features are discrete and balanced in magnitude.  The dataset can be downloaded at \url{https://archive.ics.uci.edu/ml/datasets/Car+Evaluation.}       
 
\textbf{Cancer. } 
    This dataset has 9 features, 683 samples, and 2 classes. The features are discrete and unbalanced in magnitude. The dataset can be downloaded at \url{https://archive.ics.uci.edu/ml/datasets/Breast+Cancer+Wisconsin+(Diagnostic)}.
    
 \textbf{Face. } 
    This dataset consists of images of 20 people in various poses. The 624 images are vectorized into 960 features.  
    The dataset can be downloaded at 
    \url{https://archive.ics.uci.edu/ml/datasets/CMU+Face+Images}.

\textbf{Random. } 
    This dataset has 2 features, 80 samples and 2 classes. It is generate with a gaussian distribution where half of the samples are randomly labeled as 1 or 0.
    
\textbf{Adversarial. } 
    This dataset has 2 features, 80 samples and 2 classes. It is generate with the following code:
    \begin{lstlisting}    
    #!/usr/bin/env python
    
    n = 40
    X1 = np.random.rand(n,2)
    X2 = X1 + 0.01*np.random.randn(n,2)
    
    X = np.vstack((X1,X2))
    Y = np.vstack(( np.zeros((n,1)), np.ones((n,1)) ))
    \end{lstlisting}    
 
\end{appendices}

==> appendices/k_metrics.tex <==

%\begin{appendices}
%\section{Equations for Evaluation Metrics}
%\label{app:metric_calculation}
%For all metrics assume that $X \in \mathbb{R}^{n \times d}$ and $Y \in \mathbb{R}^{n \times c}$ as the data and the label respectively. 
%
%\textbf{Normalized HSIC. } 
%    The normalized HSIC can be calculated with 
%    \begin{equation}
%        \mathbb{H} = \frac{HSIC(X,Y)}{\sqrt{HSIC(X,X) HSIC(Y,Y)}}.
%    \end{equation}    
%
%\textbf{Silhouette Score. } 
%    We used the Silhouette score library from Sklearn with the function \url{https://scikit-learn.org/stable/modules/generated/sklearn.metrics.silhouette_score.html}.
%    The Silhouette Coefficient is calculated using the mean intra-cluster distance (a) and the mean nearest-cluster distance (b) for each sample. The Silhouette Coefficient for a sample is (b - a) / max(a, b). To clarify, b is the distance between a sample and the nearest cluster that the sample is not a part of. 
%    
%\textbf{Average Cosine Similarity Ratio (CS). } 
%    Given $\mathcal{S}$ and $\mathcal{S}^c$ as sets of all pairs of samples of $(x_i,x_j)$ from a dataset $X$ that belongs to the same and different classes respectively. The average cosine similarity ratio is defined as 
%    \begin{equation}
%    CS = \frac
%    {\sum_{i,j \in \mathcal{S}^c} \langle f(x_i), f(x_j) \rangle}
%    {\sum_{i,j \in \mathcal{S}} \langle f(x_i), f(x_j) \rangle}.
%    \end{equation}
%    Since the inner product between samples not in the same class should be 0, this ratio should approach 0 as the ratio improves.
%\end{appendices}


\begin{appendices}
%\section{\texorpdfstring{$W_l$} Dimensions for each 10 Fold of each Dataset}
\section{$W_l$ Dimensions for each 10 Fold of each Dataset}
\label{app:W_dimensions}
We report the input and output dimensions of each $W_l$ for every layer of each dataset in the form of $(\alpha, \beta)$; the corresponding dimension becomes $W_l \in \mathbb{R}^{\alpha \times \beta}$. Since each dataset consists of 10-folds, the network structure for each fold is reported. We note that the input of the 1st layer is the dimension of the original data. However, after the first layer, the width of the RFF becomes the output of each layer; here we use 300. 

The $\beta$ value is chosen during the ISM algorithm. By keeping only the most dominant eigenvector of the $\Phi$ matrix, the output dimension of each layer corresponds with the rank of $\Phi$. It can be seen from each dataset that the first layer significantly expands the rank. The expansion is generally followed by a compression of fewer and fewer eigenvalues. These results conform with the observations made by \citet{montavon2011kernel} and \citet{ansuini2019intrinsic}.

\begin{tabular}{ll}
\centering
\tiny
\setlength{\tabcolsep}{7.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{cccccc|}
	\hline
Data & Layer 1 & Layer 2 & Layer 3 & Layer 4 \\ 
	\hline
adversarial 1 & (2, 2) & (300, 61) & (300, 35) \\ 
adversarial 2 & (2, 2) & (300, 61) & (300, 35) \\ 
adversarial 3 & (2, 2) & (300, 61) & (300, 8) & (300, 4) \\ 
adversarial 4 & (2, 2) & (300, 61) & (300, 29) \\ 
adversarial 5 & (2, 2) & (300, 61) & (300, 29) \\ 
adversarial 6 & (2, 2) & (300, 61) & (300, 7) & (300, 4) \\ 
adversarial 7 & (2, 2) & (300, 61) & (300, 34) \\ 
adversarial 8 & (2, 2) & (300, 12) & (300, 61) & (300, 30) \\ 
adversarial 9 & (2, 2) & (300, 61) & (300, 33) \\ 
adversarial 10 & (2, 2) & (300, 61) & (300, 33) \\ 
	\hline
\end{tabular}
&
\centering
\tiny
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{ccccc|}
	\hline
Data & Layer 1 & Layer 2 & Layer 3 \\ 
	\hline
Random 1 & (3, 3) & (300, 47) & (300, 25) \\ 
Random 2 & (3, 3) & (300, 46) & (300, 25) \\ 
Random 3 & (3, 3) & (300, 46) & (300, 25) \\ 
Random 4 & (3, 3) & (300, 47) & (300, 4) \\ 
Random 5 & (3, 3) & (300, 47) & (300, 25) \\ 
Random 6 & (3, 3) & (300, 45) & (300, 23) \\ 
Random 7 & (3, 3) & (300, 45) & (300, 25) \\ 
Random 8 & (3, 3) & (300, 45) & (300, 21) \\ 
Random 9 & (3, 3) & (300, 45) & (300, 26) \\ 
Random 10 & (3, 3) & (300, 47) & (300, 25) \\ 
	\hline
\end{tabular}
\end{tabular}




\begin{tabular}{ll}
\tiny
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{cccccccc|}
	\hline
Data & Layer 1 & Layer 2 & Layer 3 & Layer 4 & Layer 5 & Layer 6 \\ 
	\hline
spiral 1 & (2, 2) & (300, 15) & (300, 6) & (300, 7) & (300, 6) \\ 
spiral 2 & (2, 2) & (300, 13) & (300, 6) & (300, 7) & (300, 6) & (300, 6) \\ 
spiral 3 & (2, 2) & (300, 12) & (300, 6) & (300, 7) & (300, 6) & (300, 6) \\ 
spiral 4 & (2, 2) & (300, 13) & (300, 6) & (300, 7) & (300, 6) & (300, 6) \\ 
spiral 5 & (2, 2) & (300, 13) & (300, 6) & (300, 7) & (300, 6) \\ 
spiral 6 & (2, 2) & (300, 14) & (300, 6) & (300, 7) & (300, 6) \\ 
spiral 7 & (2, 2) & (300, 14) & (300, 6) & (300, 7) & (300, 6) \\ 
spiral 8 & (2, 2) & (300, 14) & (300, 6) & (300, 7) & (300, 6) & (300, 6) \\ 
spiral 9 & (2, 2) & (300, 13) & (300, 6) & (300, 7) & (300, 6) \\ 
spiral 10 & (2, 2) & (300, 14) & (300, 6) & (300, 7) & (300, 6) \\ 
	\hline
\end{tabular}
&
\tiny
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{cccccccc}
	\hline
Data & Layer 1 & Layer 2 & Layer 3 & Layer 4 & Layer 5 & Layer 6 \\ 
	\hline
wine 1 & (13, 11) & (300, 76) & (300, 6) & (300, 7) & (300, 6) & (300, 6) \\ 
wine 2 & (13, 11) & (300, 76) & (300, 6) & (300, 6) & (300, 6) & (300, 6) \\ 
wine 3 & (13, 11) & (300, 75) & (300, 6) & (300, 7) & (300, 6) & (300, 6) \\ 
wine 4 & (13, 11) & (300, 76) & (300, 6) & (300, 6) & (300, 6) & (300, 6) \\ 
wine 5 & (13, 11) & (300, 74) & (300, 6) & (300, 7) & (300, 6) & (300, 6) \\ 
wine 6 & (13, 11) & (300, 74) & (300, 6) & (300, 6) & (300, 6) & (300, 6) \\ 
wine 7 & (13, 11) & (300, 74) & (300, 6) & (300, 6) & (300, 6) & (300, 6) \\ 
wine 8 & (13, 11) & (300, 75) & (300, 6) & (300, 7) & (300, 6) & (300, 6) \\ 
wine 9 & (13, 11) & (300, 75) & (300, 6) & (300, 8) & (300, 6) & (300, 6) \\ 
wine 10 & (13, 11) & (300, 76) & (300, 6) & (300, 7) & (300, 6) & (300, 6) \\ 
	\hline
\end{tabular}
\end{tabular}

\begin{tabular}{ll}
\tiny
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{cccccccc|}
	\hline
Data & Layer 1 & Layer 2 & Layer 3 & Layer 4 & Layer 5 & Layer 6 \\ 
	\hline
car 1 & (6, 6) & (300, 96) & (300, 6) & (300, 8) & (300, 6) \\ 
car 2 & (6, 6) & (300, 96) & (300, 6) & (300, 8) & (300, 6) \\ 
car 3 & (6, 6) & (300, 91) & (300, 6) & (300, 8) & (300, 6) \\ 
car 4 & (6, 6) & (300, 88) & (300, 6) & (300, 8) & (300, 6) & (300, 6) \\ 
car 5 & (6, 6) & (300, 94) & (300, 6) & (300, 8) & (300, 6) \\ 
car 6 & (6, 6) & (300, 93) & (300, 6) & (300, 7) \\ 
car 7 & (6, 6) & (300, 92) & (300, 6) & (300, 8) & (300, 6) \\ 
car 8 & (6, 6) & (300, 95) & (300, 6) & (300, 7) & (300, 6) \\ 
car 9 & (6, 6) & (300, 96) & (300, 6) & (300, 9) & (300, 6) \\ 
car 10 & (6, 6) & (300, 99) & (300, 6) & (300, 8) & (300, 6) \\ 
	\hline
\end{tabular}
&
\tiny
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{ccccccc|}
	\hline
Data & Layer 1 & Layer 2 & Layer 3 & Layer 4 & Layer 5 \\ 
	\hline
divorce 1 & (54, 35) & (300, 44) & (300, 5) & (300, 5) \\ 
divorce 2 & (54, 35) & (300, 45) & (300, 4) & (300, 4) \\ 
divorce 3 & (54, 36) & (300, 49) & (300, 6) & (300, 6) \\ 
divorce 4 & (54, 36) & (300, 47) & (300, 7) & (300, 6) \\ 
divorce 5 & (54, 35) & (300, 45) & (300, 6) & (300, 6) \\ 
divorce 6 & (54, 36) & (300, 47) & (300, 6) & (300, 6) \\ 
divorce 7 & (54, 35) & (300, 45) & (300, 6) & (300, 6) & (300, 4) \\ 
divorce 8 & (54, 36) & (300, 47) & (300, 6) & (300, 7) & (300, 4) \\ 
divorce 9 & (54, 36) & (300, 47) & (300, 5) & (300, 5) \\ 
divorce 10 & (54, 36) & (300, 47) & (300, 6) & (300, 6) \\ 
	\hline
\end{tabular}
\end{tabular}


\begin{table}[h]
\tiny
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{cccccccccccc|}
	\hline
Data & Layer 1 & Layer 2 & Layer 3 & Layer 4 & Layer 5 & Layer 6 & Layer 7 & Layer 8 & Layer 9 & Layer 10 \\ 
	\hline
cancer 1 & (9, 8) & (300, 90) & (300, 5) & (300, 6) & (300, 6) & (300, 5) & (300, 4) & (300, 5) & (300, 6) & (300, 6) \\ 
cancer 2 & (9, 8) & (300, 90) & (300, 6) & (300, 7) & (300, 8) & (300, 11) & (300, 8) & (300, 4) \\ 
cancer 3 & (9, 8) & (300, 88) & (300, 5) & (300, 6) & (300, 7) & (300, 7) & (300, 6) & (300, 4) \\ 
cancer 4 & (9, 8) & (300, 93) & (300, 6) & (300, 7) & (300, 9) & (300, 11) & (300, 8) \\ 
cancer 5 & (9, 8) & (300, 93) & (300, 9) & (300, 10) & (300, 10) & (300, 11) & (300, 9) & (300, 7) \\ 
cancer 6 & (9, 8) & (300, 92) & (300, 7) & (300, 8) & (300, 8) & (300, 7) & (300, 7) \\ 
cancer 7 & (9, 8) & (300, 90) & (300, 4) & (300, 4) & (300, 5) & (300, 6) & (300, 6) & (300, 6) & (300, 6) \\ 
cancer 8 & (9, 8) & (300, 88) & (300, 5) & (300, 6) & (300, 7) & (300, 8) & (300, 7) & (300, 6) \\ 
cancer 9 & (9, 8) & (300, 88) & (300, 5) & (300, 7) & (300, 7) & (300, 7) & (300, 7) \\ 
cancer 10 & (9, 8) & (300, 97) & (300, 9) & (300, 11) & (300, 12) & (300, 13) & (300, 6) \\ 
	\hline
\end{tabular}
\end{table}

\begin{table}[h]
\tiny
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{cccccc|}
	\hline
Data & Layer 1 & Layer 2 & Layer 3 & Layer 4 \\ 
	\hline
face 1 & (960, 233) & (300, 74) & (300, 73) & (300, 46) \\ 
face 2 & (960, 231) & (300, 75) & (300, 73) & (300, 43) \\ 
face 3 & (960, 231) & (300, 76) & (300, 73) & (300, 44) \\ 
face 4 & (960, 232) & (300, 76) & (300, 74) & (300, 44) \\ 
face 5 & (960, 231) & (300, 77) & (300, 73) & (300, 43) \\ 
face 6 & (960, 232) & (300, 74) & (300, 72) & (300, 47) \\ 
face 7 & (960, 232) & (300, 76) & (300, 73) & (300, 45) \\ 
face 8 & (960, 230) & (300, 74) & (300, 74) & (300, 44) \\ 
face 9 & (960, 233) & (300, 76) & (300, 76) & (300, 45) \\ 
face 10 & (960, 231) & (300, 76) & (300, 70) & (300, 43) \\ 
	\hline
\end{tabular}
\end{table}

\end{appendices}

\clearpage
\newpage


%\begin{appendices}
%\section{Dimension Expand of the First Few Layers }
%\label{app:dim_expansion}
%    A kernel function is traditionally used to map data from a low dimensional representation to a high dimensional feature space. The purpose of this mapping is to project the data to a new set of bases to extract relationships within the data that is not obvious in the original bases. Therefore, given an appropriate new set of bases, it is possible and likely that additional dimensions will be discovered in the new bases from the raw data. This observation is commonly seen with kernel methods when the data contain nonlinear relationships. Following this logic, while the results from \citet{ansuini2019intrinsic} may suggest that the "Hunchback" phenomenon is always occuring, our model indicates an expansion \textit{only if} the new bases are capable of capturing additional information. In fact, for simple data patterns where the original bases are sufficient, the dimension can even shrink. This is precisely observed in Appendix~\ref{app:metric_graphs} where the Divorce and Face datasets only experienced compression. 
%    
%    By maximizing the HSIC objective, our model discovers a new set of bases via $W_l$. Therefore, if there exists a set of bases in a higher dimension that captures a better dependency a higher HSIC value is also obtained. This will often be the case for Gaussian kernels due to its flexibility.  However, if all available information is already captured by the new bases, the HSIC objective only increases by compression as shown by our theorems. The "hunchback" pattern as observed by \citet{ansuini2019intrinsic} is simply a process of kernel discovery to discover representations that maximize HSIC and the \textit{separability objective}.
%   
%\end{appendices}



==> appendices/l_kernel_graphs.tex <==
\clearpage
%\newpage

\begin{appendices}
\section{Graphs of Kernel Sequences}
\label{app:kernel_sequence_graph}

A representation of the \KS are displayed in the figures below for each dataset. The samples of the kernel matrix are previously organized to form a block structure by placing samples of the same class adjacent to each other. Since the Gaussian kernel is restricted to values between 0 and 1, we let white and dark blue be 0 and 1 respectively where the gradients reflect values in between. Our theorems predict that the \KS will evolve from an uninformative kernel into a highly discriminating kernel of perfect block structures. 

\begin{figure}[h]
\center
    \includegraphics[width=9cm]{img/wine_kernel.png}
    \caption{The kernel sequence for the wine dataset.}
\end{figure} 

\begin{figure}[h]
\center
    \includegraphics[width=9cm]{img/cancer_kernel.png}
    \caption{The kernel sequence for the cancer dataset.}
\end{figure} 

\begin{figure}[h]
\center
    \includegraphics[width=9cm]{img/adv_kernel.png}
    \caption{The kernel sequence for the Adversarial dataset.}
\end{figure} 

\begin{figure}[h]
\center
    \includegraphics[width=9cm]{img/car_kernel.png}
    \caption{The kernel sequence for the car dataset.}
\end{figure} 

\begin{figure}[h]
\center
    \includegraphics[width=11cm]{img/face_kernel.png}
    \caption{The kernel sequence for the face dataset.}
\end{figure} 

\begin{figure}[h]
\center
    \includegraphics[width=9cm]{img/divorce_kernel.png}
    \caption{The kernel sequence for the divorce dataset.}
\end{figure} 

\begin{figure}[h]
\center
    \includegraphics[width=11cm]{img/spiral_kernel.png}
    \caption{The kernel sequence for the spiral dataset.}
\end{figure} 



\begin{figure}[h]
\center
    \includegraphics[width=11cm]{img/random_kernel.png}
    \caption{The kernel sequence for the Random dataset.}
\end{figure} 
\end{appendices}

==> appendices/m_metric_graphs.tex <==


\clearpage
\newpage

\begin{appendices}
\section{Evaluation Metrics Graphs}
\label{app:metric_graphs}

\begin{figure}[h]
\center
    \includegraphics[width=10cm]{img/r1.png}
    \caption{}
\end{figure} 

\begin{figure}[h]
\center
    \includegraphics[width=10cm]{img/r2.png}
    \caption{Figures of key metrics for all datasets as samples progress through the network. It is important to notice the uniformly and monotonically increasing \RS for each plot
    since this guarantees a converging kernel/risk sequence. As the $\mathcal{T}$ approach 0, samples of the same/difference classes in IDS are being pulled into a single point or pushed maximally apart respectively. As $C$ approach 0, samples of the same/difference classes in RKHS are being pulled into 0 or $\frac{\pi}{2}$ cosine similarity respectively.}
\end{figure} 

\end{appendices}


==> appendices/n_optimal_sigma.tex <==
\newpage
\begin{appendices}
\section{Optimal Gaussian $\sigma$ for Maximum Kernel Separation}
\label{app:opt_sigma}
Although the Gaussian kernel is the most common kernel choice for kernel methods, its $\sigma$ value is a hyperparameter that must be tuned for each dataset. This work proposes to set the $\sigma$ value based on the maximum kernel separation. The source code is made publicly available on \url{https://github.com/anonamous}.
%\url{https://github.com/endsley/opt_gaussian_-}.


Let $X \in \mathbb{R}^{n \times d}$ be a dataset of $n$ samples with $d$ features and let $Y \in \mathbb{R}^{n \times \nclass}$ be the corresponding one-hot encoded labels where $\nclass$ denotes the number of classes. Given $\kappa_X(\cdot, \cdot)$ and $\kappa_Y(\cdot,\cdot)$ as two kernel functions that applies respectively to $X$ and $Y$ to construct kernel matrices $K_X \in \mathbb{R}^{n \times n}$ and $K_Y \in \mathbb{R}^{n \times n}$. Given a set $\mathcal{S}$, we denote $|\mathcal{S}|$ as the number of elements within the set. Also let $\mathcal{S}$ and $\mathcal{S}^c$ be sets of all pairs of samples of $(x_i,x_j)$ from a dataset $X$ that belongs to the same and different classes respectively, then the average kernel value for all $(x_i,x_j)$ pairs with the same class is
\begin{equation}
    d_{\mathcal{S}} = \frac{1}{|\mathcal{S}|}\sum_{i,j \in \mathcal{S}} e^{-\frac{||x_i - x_j||^2}{2\sigma^2}}
\end{equation}
and the average kernel value for all $(x_i,x_j)$ pairs between different classes is
\begin{equation}
    d_{\mathcal{S}^c} = 
    \frac{1}{|\mathcal{S}^c|}\sum_{i,j \in \mathcal{S}^c} e^{-\frac{||x_i - x_j||^2}{2\sigma^2}}. 
\end{equation}
We propose to find the $\sigma$ that maximizes the difference between $d_{\mathcal{S}}$ and $d_{\mathcal{S}^c}$ or 
\begin{equation}
    \underset{\sigma}{\max} \quad 
    \frac{1}{|\mathcal{S}|}\sum_{i,j \in \mathcal{S}} e^{-\frac{||x_i - x_j||^2}{2\sigma^2}} - 
    \frac{1}{|\mathcal{S}^c|}\sum_{i,j \in \mathcal{S}^c} e^{-\frac{||x_i - x_j||^2}{2\sigma^2}}.
    \label{eq:main_objective}
\end{equation}
It turns out that is expression can be computed efficiently. Let $g = \frac{1}{|\mathcal{S}|}$ and $\bar{g} = \frac{1}{|\mathcal{S}^c|}$, and let $\textbf{1}_{n \times n} \in \mathbb{R}^{n \times n}$ be a matrix of 1s, then we can define $Q$ as
\begin{equation}
    Q = -g K_Y + \bar{g} (\textbf{1}_{n \times n} - K_Y).
\end{equation}
Or $Q$ can be written more compactly as
\begin{equation}
    Q = \bar{g} \textbf{1}_{n \times n} - (g + \bar{g})K_Y. 
\end{equation}
Given $Q$, Eq.~(\ref{eq:main_objective}) becomes
\begin{equation}
    \underset{\sigma}{\min} \quad 
    \Tr(K_X Q).
    \label{eq:obj_compact}
\end{equation}
This objective can be efficiently solved with BFGS. 

Below in Fig.~\ref{fig:max_kernel_separation}, we plot out the average within cluster kernel and the between cluster kernel values as we vary $\sigma$. From the plot, we can see that the maximum separation is discovered via BFGS. 
    \begin{figure}[h]
        \centering
        \includegraphics[width=10cm,height=7cm]{img/opt_kernel_separation.png}
        \caption{Maximum Kernel separation.}
        \label{fig:max_kernel_separation}
    \end{figure} 
    
    
\textbf{Relation to HSIC. }    
From Eq.~(\ref{eq:obj_compact}), we can see that the $\sigma$ that causes maximum kernel separation is directly related to HSIC. Given that the HSIC objective is normally written as
\begin{equation}
    \underset{\sigma}{\min} \quad 
    \Tr(K_X H K_Y H),
\end{equation}
by setting $Q=HK_YH$, we can see how the two formulations are related. While the maximum kernel separation places the weight of each sample pair equally, HSIC weights the pair differently.
We also notice that the $Q_{i,j}$ element is positive/negative for $(x_i,x_j)$ pairs that are with/between classes respectively. Therefore, the argument for the global optimum should be relatively close for both objectives. Below in Figure~\ref{fig:max_HSIC}, we show a figure of HSIC values as we vary $\sigma$. Notice how the optimal $\sigma$ is almost equivalent to the solution from maximum kernel separation. For the purpose of \kc, we use $\sigma$ that maximizes the HSIC value.
    \begin{figure}[h]
        \centering
        \includegraphics[width=10cm,height=7cm]{img/opt_HSIC.png}
        \caption{Maximal HSIC.}
        \label{fig:max_HSIC}
    \end{figure} 
\end{appendices}

==> tex/b_intro.tex <==
\section{Introduction}


%Since the seminal work by \citet{rumelhart1988learning}, Multilayer Perceptrons (MLPs) have been actively researched from both theroetical and biological perspectives. Due to MLP's brain-inspired architecture, many have searched for a more direct connection between MLPs and our brains \cite{zador2019critique,walker2020Deep}. This attempt has triggered a controversy \cite{whittington2019theories} around the neural plausibility of backpropagation (BP), i.e., while some contend that brains cannot simulate BP \cite{crick1989recent,grossberg1987competitive}, others have recently proposed counterclaims with a new generation of models \cite{hinton2007backpropagation,Lilli2020Backpropagation,liao2016important,bengio2017stdp,guerguiev2017towards,sacramento2018dendritic,whittington2017approximation}. 
%This work was originally  inspired by this debate, yet our research led us down a different path. Instead of finding more answers to the biological plausibility of BP, this work discovered an alternative strategy to solve MLP for \textit{classification} where the weights are trained locally without the usage of BP and Gradient Descent (GD).

Since the seminal work by \citet{rumelhart1988learning}, Multilayer Perceptrons (MLPs) have become a popular tool for classification. Yet, the theoretical understanding of its inner workings remains an active area of research. As a result, the training process necessitates a careful choice of network width, depth, initialization weights, and activation functions; the number of hyper-parameters can even exceed the number of samples. The careful engineering of the network settings and weights are required because the community is still building its theoretical foundation. 


Much work has been dedicated to understanding MLPs.  Some have investigated MLP's expressiveness  \cite{cybenko1989approximation,hornik1991approximation,lu2017expressive,montufar2014number,poole2016exponential}, others have concentrated on the appropriate initialization of the weights \cite{glorot2010understanding,he2015delving,schoenholz2016deep}. Recent discoveries on the characteristic and geometry of the network weights \cite{li2018measuring,fort2019large,poggio2020complexity} indicate that the optimal weights of a network reside on a subspace. In fact, the magnitude of the weights does not matter, instead, the key lies in the direction of the weights. We connect the dots from these clues to the Reproducing Kernel Hilbert Space (RKHS) \cite{gretton2012kernel,minh2006mercer} and develop a new kernel-based network that redefines classification as a dependence maximization problem.

%problem from a different angle.

Our motivation to link kernels to neural networks is not without evidence. \citet{montavon2011kernel} used Kernel PCA with a Gaussian kernel (\rbfk) to learn the weights of an MLP, demonstrating how stacks of kernels and MLPs can exhibit similar predictive capability. Recently, \citet{belkin2018understand} have compared MLP and kernel's ability to yield good generalization results despite overfitting. Their experiments suggest 
that this key property of MLPs is also manifested in kernel methods; which led them to conclude that to truly understand MLPs, we need to better understand the kernel discovery process. MLPs have also been modeled as a Gaussian process (GP) \cite{neal2012bayesian,matthews2018gaussian,lee2017deep}. This kernel interpretation has inspired a significant amount of research \cite{hayou2019impact,lee2019wide,yang2019scaling,duvenaud2014avoiding}. Extending from the GP perspective, the Neural Tangent Kernel (NTK) has been proposed to describe the dynamics of the network during training \cite{jacot2018neural,arora2019exact}, further elucidating the relationship between MLPs and kernels. 


We depart from previous kernel work by representing MLP layers as a converging sequence of kernel feature maps parameterized by the layer weights. We solve each layer greedily by identifying the optimal feature map that maximizes the Hilbert Schmidt Independence Criterion (HSIC) between the layer output and the label. While a related work by \citet{ma2019hsic} also used layer-wise learning via HSIC, their objective simulates Information Bottleneck and they employed a traditional network structure solved by Stochastic Gradient Descend (SGD). In contrast, our network deviate from standard concepts of activation functions by using the feature map of a \rbfk{} in its place, leveraging the kernel trick during optimizing. The layer-wise sequential training implies that all learning is local, and neither backpropagation (BP) nor even SGD is needed. 

As the key theoretical result, the function class represented by the network is proved to be sufficiently rich to learn any dataset labeling using a finite number of layers, in the sense of reaching minimum mean-squared error or cross-entropy: assuming no overlapping of two data points with different labels. Lastly, we exploit the recent work on the geometric landscape of the network solution by constraining the solution to a linear subspace. This allows us to replace SGD with an existing spectral method, Iterative Spectral Method (ISM) \cite{wu2018iterative, wu2019deep}. By greedily solving each layer spectrally, exploding/vanishing gradients are avoided and natural choices of network width and depth emerges. 







==> tex/x_broader_impact.tex <==
\section{Broader Impact}

In our attempt to explain the nature of Neural Networks, we discovered an alternative perspective to solve them, a kernel interpretation where all of its internal mechanisms are well understood. Although more research is required to make our method practical to larger datasets, we are confident that these obstacles will be solved in the near future. Additionally, a convolutional extension of our work is definitely feasible. Therefore, a logical direction of our research suggests that it will lead to significantly faster classifiers, paving the way for better medical applications, better self-driving cars, and better weather prediction. 

While we cannot predict how others might use our work, however, we can make predictions based on the direction of our research. We hope that given this technology, medical researchers can train better models to predict cancer and other diseases. Environmental scientists might be able to better measure pollution, air quality, and water quality. We want better micro-lending algorithms that allow economically depressed regions of the world to thrive. We hope our research might even lead to better algorithms that discover vaccines to mitigate the impact of a pandemic.  

As researchers, in our quest for the truth, we hope to remake the world a better place. Yet, by sharing our discoveries with the world, we lose control over its impact. Good intention alone cannot prevent the military or any terrorist organizations from leveraging the technology to create killer robots. Nor can it prevent totalitarian states from using it to suppress its own citizens. The same convolutional adaptation we hope to use to improve cancer prediction can be used by countries to identify citizens who criticize the government, locking them away without due process. Even in the best case where technology is developed without any malice, we see the potential of millions of jobs being automated. Worse yet, it is always those who are least able to adapt to new jobs, the most vulnerable, that are being replaced by our inventions.

None of these problems are easy to solve. Yet, as we see the mounting problems of the world, many of them caused by the advancement of our research, how much responsibility should we bear as individual researchers? Is the addition of the broader impact section sufficient?  Or should we consider a version of the Hippocratic oath for our profession? For the betterment of the world, we must begin the dialog to answer these questions.  As researchers and as citizens of the world, let us take on more responsibility to mitigate the worst impact of our work on society. 



%How can any particular solution work unless we also vote the right person into office. Therefore, we question if perhaps more of us should take greater leadership in the decision making process by entering into the uncomfortable world of politics, not as advisors, but as leaders of our society. Perhaps some people in our community would do a much greater service for the world running a country instead of a lab.

%we must join the group that makes decisions for our society. In the research community,, too few of us run for office. Consequently, we are the ones giving advice and not the ones making the decisions. So much of our time and energy is spent writing grants for our next projects, explaining to the decision-makers how our work can be used to change society. Imagine the time and energy that could be directed to actual research if the decision-makers had a background in science and research.  Therefore, it is a reasonable question to ask: can we in the research community better serve society if some of us become the decision-makers?



%As academics, it is clear why so few of us enter the political world, we became researchers to research and many of us lack the political ambition for politics. In this quest to find the truth through our research, the university environment is simply too comfortable. Unlike the political bickering we see on television, we live in our own bubble where truth always wins. Yet, outside of this bubble, fake news is winning. In academia, our decisions are not made to be popular by the masses, instead, we are often forced into a position to be the bearers of an inconvenient truth. 

%Yet, as we see the mounting problems of the world, many of them caused by the advancement of our research, how can any particular solution work unless we also vote the right person into office. Therefore, we need to take greater leadership in the decision making process by entering into the uncomfortable world of politics, not as advisors, but as leaders of our society, if we are to make sure ethics prevail. Indeed, we truly believe that some people in our community would do a much greater service for the world running a country instead of a lab.


==> tex/z_prev_writing.tex <==
\textbf{MLPs as an Iterative Cyclic Transition. } We propose to model the MLP previously described as a cyclic transition between two spaces, i.e., Reproducing Kernel Hilbert Space (RKHS) and the image space of its dual  (IDS). The data is assumed to initially reside in RKHS. From there, our model views each column of $W_l$ as $q$ separate functions in RKHS that maps the data into its image space (IDS). From IDS, the activation function $\phi$ then maps the data in IDS back into RKHS, thereby completing a single cyclic. This cycle is our model's interpretation of a MLP layer, therefore, the composition of the layers consist of multiple cycles between these 2 spaces where the output of the last layer is then used to compute $\mathcal{E}$. The idea of modeling MLPs as transitions of states is analogous to a Markov Chain (MC), i.e., the behavior of the entire network is encapsulated by the transition matrix and its initial state. Inspired by MC's ability to model a complex system of transitions, we discovered that the behavior of the entire MLP also becomes predictable if the transitions satisfy certain properties.
   
    %Since the linear subspace is generated by applying $q$ functions in the RKHS to all input samples, following the Riesz representation theorem, we refer to the linear subspace as the \textit{images of the dual space} (IDS). 


Since each cyclic transition is equivalent to a network layer, we can model the network at incremental depths as a sequence of functions $(f_{1^\circ}, ..., f_{L^\circ})$. Since each function in this sequence can be interpreted as a feature map, we refer to this sequence as the \textit{kernel sequence}. By setting each element of the \textit{kernel sequence} as $f$ in Eq.~(\ref{eq:basic_empirical_risk}), it induces another sequence ($\mathcal{E}_1,...,\mathcal{E}_L$) of empirical risks denoted by Eq.~(\ref{eq:solve_incrementally}), which we will refer to as the \textit{risk sequence}. By interpreting the transitions as a sequence, it models the entire MLP while simplifying its representation. From this perspective, our goal is to discover a transition model that generates \textit{kernel sequences} capable of solving classification problems. To accomplish this, we first identify the principal properties necessary to guide its design.

\textbf{Properties of a Chain. }
Viewing the layers as a sequence of functions enables us to direct the transition model to exhibit certain properties. Specifically, we propose two properties which the \textit{risk sequence} must satisfy, and one property which the empirical risk $\mathcal{E}$ must satisfy.
\begin{property}
The \textit{risk sequence} must converge to a limit where $\lim_{l \rightarrow \infty} \mathcal{E}_l = \mathcal{E}^*$.
\label{prop:convergent_property}
\end{property}

\begin{property}
The network weights $W^*$ at $\mathcal{E}^*(W^*)$ must satisfy the First Order and Second Order Necessary local optimality Conditions as defined by \citet{bertsekas1997nonlinear} (App.~\ref{app:2nd_order}) for the empirical risk.
\label{prop:convergent_limit_property}
\end{property}

\begin{property}
The empirical risk must satisfy the \textit{affinity property} defined as
\begin{definition}
Given $\mathcal{S}$ and $\mathcal{S}^c$ as sets of all pairs of samples of $(x_i,x_j)$ from a dataset $X$ that belongs to the same and different classes respectively, let all $\mu_{i,j}$ values be non-negative scalars, and let $\kappa$ be a similarity measure between any pairs of $(x_i, x_j)$. An empirical risk satisfies the \textit{affinity property} if there exists a $\kappa$ such that its optimal solution $f^*$ is also the optimal solution for the $\textbf{affinity objective}$, which we define here as
    \begin{align}
    \underset{f}{\max} \hspace{0.05cm} 
    \sum_{i,j \in \mathcal{S}} \mu_{i,j} \mathcal{\kappa}(f(x_i), f(x_j)) - \sum_{i,j \in \mathcal{S}^c} 
    \mu_{i,j}
    \mathcal{\kappa}(f(x_i), f(x_j)).
     \label{eq:separability_property_definition}
    \end{align}
    \label{def:affinity_def}
\end{definition}
\label{prop:separability_prop}
\end{property}

While the first two properties place constraints on the transitional behavior of the \textit{risk sequence}, Property \ref{prop:separability_prop} is a constraint on $\mathcal{E}$. Notice how Properties 1 and 2 suggest an alternative strategy to optimize Eq.~(\ref{eq:basic_empirical_risk}). This observation leads directly to our proposal of incrementally solving Eq.~(\ref{eq:solve_incrementally}) in place of Eq.~(\ref{eq:basic_empirical_risk}). The addition of Property 3 is necessary to focus our attention to classification tasks. Namely, to perform classification, we wish to discover a mapping $\kappa \colon \mathbb{R}^m \times \mathbb{R}^m \rightarrow \mathbb{R}$ where sample pairs of the \textit{same/different} classes achieve a high/low score based on some notion of similarity. Since these three properties form the foundation of our work, we refer to them as the \textit{KNet properties}. By extension, we refer to MLPs with these properties as Kernel Chain Networks or KNets. While these properties do not arise naturally, our work demonstrates that they can be induced by appropriately choosing the activation function, empirical risk, and optimization strategy. 

\textbf{Satisfying the \textit{KNet Properties}. }  
%The ability of an MLP to satisfy the \textit{KNet properties} is inextricably related to the choice of $\mathcal{E}$ and $\Psi$. 

%We identified the incremental improvement of dependence between $\Psi(R_{l-1}W_l)$ and $Y$ as our central strategy to achieve classification. With this approach, we found the modeling of each layer via HSIC with RBF kernel feature map particularly advantageous for $\mathcal{E}$ and $\Psi$. This conclusion is supported by our theoretical work as presented below with their derivations and proofs in App.~\ref{app:proof_for_CCN_becomes_HSIC}, \ref{app:ccn_satisfies_dependence_property}. 

We propose to model each transition for Eq.~(\ref{eq:solve_incrementally}) as
    \begin{equation}
        %\underset{W_l}{\max} \quad \Tr( \Gamma K_{R_{l-1} W_l} )
        \underset{W_l}{\max} \quad \Tr( HK_Y H K_{R_{l-1} W_l} )
        %\underset{W_l}{\max} \quad \hsic(R_{l-1}W_l, Y)
        \hspace{0.3cm} \text{s.t} \hspace{0.3cm} W_l^TW_l = I.
         \label{eq:hsic_obj_pure}
    \end{equation}
    
%\begin{theorem}\label{thm:CCN_becomes_HSIC}
%    Each transition as Eq.~(\ref{eq:solve_incrementally}) can be modeled via HSIC to solve $W_l$ with
%    \begin{equation}
%        %\underset{W_l}{\max} \quad \Tr( \Gamma K_{R_{l-1} W_l} )
%        \underset{W_l}{\max} \quad \Tr( HK_Y H K_{R_{l-1} W_l} )
%        %\underset{W_l}{\max} \quad \hsic(R_{l-1}W_l, Y)
%        \hspace{0.3cm} \text{s.t} \hspace{0.3cm} W_l^TW_l = I.
%         \label{eq:hsic_obj_pure}
%    \end{equation}
%\end{theorem}


Eq.~(\ref{eq:hsic_obj_pure}) is chosen because it accurately models each step of a cycle, i.e., it multiplies the input $R_{l-1}$ by $W_l$, passes $R_{l-1}W_l$ through a kernel feature map, and then maximizes the dependence between $\Psi(R_{l-1}W_l)$ and $Y$. Therefore, the optimal $W_l$ maximizes the dependence between the layer output and its label. We emphasize that using kernel feature maps as the activation function generalizes its traditional mode of operation. If we let $r_l$ be a single sample at the output of the $l^{th}$ layer, then $\Psi$ traditionally operates \textit{separately} on each element of the vector $W_{l+1}^T r_l \in \mathbb{R}^m$ to produce another vector of $\mathbb{R}^m$. However, kernel feature maps extends this operation to $\Psi$s that can operate on the entire vector, e.g., $\Psi$ from RBF kernel operates on the entire vector to produce an output in $\mathbb{R}^{\infty}$. Therefore, by using a RBF kernel, each layer achieves the flexibility of approximating any function on a compact subset of $\mathbb{R}^n$ \cite{csaji2001approximation}. Additionally, modeling each MLP layer as Eq.~(\ref{eq:hsic_obj_pure}) is a highly attractive proposition because it can be effectively solved by the Iterative Spectral Method (ISM) recently proposed by \citet{wu2018iterative, wu2019solving}. ISM avoids Stochastic Gradient Descent (SGD) by solving Eq.~(\ref{eq:hsic_obj_pure}) spectrally, while theoretically guaranteeing the 1st and 2nd order optimality condition

\begin{theorem}\label{thm:ccn_satisfies_dependence_property}
    Eq.~(\ref{eq:hsic_obj_pure}) is an affinity objective.  
\end{theorem}

\begin{theorem}\label{thm:the_right_activation_function}
    Some statement about monotonic improvement proof (NOT DONE)
    %There exist a set of weights ${W_1, ..., W_L}$ such that Eq.~(\ref{eq:hsic_obj_pure}) (with a Gaussian kernel) generates a monotonically decreasing \textit{risk sequence} that converges.
\end{theorem}

Theorems \ref{thm:ccn_satisfies_dependence_property} and \ref{thm:the_right_activation_function} is aimed to satisfy Properties 1 and 3. By identifying Eq.~(\ref{eq:hsic_obj_pure}) as an \textit{affinity objective}, its solution also solves classification. Theorem \ref{thm:the_right_activation_function} further verifies that it is possible for Eq.~(\ref{eq:hsic_obj_pure}) to generate a converging sequence. Although there are many ways to generate converging sequences, here, we leverage the Monotone Convergence Theorem \cite{bibby1974axiomatisations} where a monotone sequence is guaranteed to have a limit if and only if the sequence is bounded. Therefore, if each transition generates an $\mathcal{E}_l$ lower than $\mathcal{E}_{l-1}$ in a bounded space, the \textit{risk sequence} is guaranteed to converge. Ideally, we wish to prove that ISM can can generate a sequence of weights $W_l$ that produces this convergence. Unfortunately, at this point, we are only able to prove the existence of a solution. Instead, we experimentally show that ISM generates a monotonically converging \textit{risk sequence}. Since ISM guarantees 1st and 2nd order optimality conditions, solving an MLP greedily guarantees each element of the \textit{risk sequence} to satisfy Property 2, thereby satisfying all 3 \textit{KNet Properties}.

\textbf{Relating HSIC to Traditional Empirical Risks. } Perhaps the most surprising result of our investigation is the discovery of HSIC's relationship to traditional empirical risks such as MSE and CE. The mapping between RKHS and IDS has tremendous effect on the orientation of the samples. Indeed, vastly different patterns can be induced by keeping or discarding the last activation function $\Psi$ after training. Specifically, we found that IDS and RKHS induce different results capable of solving MSE or CE, i.e., the same weights that optimizes HSIC also minimizes MSE and CE in their respective space. Namely, we propose the following two theorems with their proofs in App.~\ref{app:theorem_2_proof} and \ref{app:theorem_3_proof}. 
\begin{theorem}\label{thm:HSIC_as_cross_entropy}
    Given a change of basis, the argmax of the HSIC objective is equivalent to the argmin of the CE objective in RKHS.
\end{theorem}
\begin{theorem}\label{thm:HSIC_as_MSE}
    The MSE objective is minimized by the argmax of the HSIC objective in IDS. 
\end{theorem}

Theorems~\ref{thm:HSIC_as_cross_entropy} and \ref{thm:HSIC_as_MSE} suggests that by maximizing the dependence between $R_{l}$ and $Y$ to generate a converging \textit{risk sequence}, it has the same effect as minimizing both MSE and CE in different spaces.

\textbf{Interpretation of an MLP via HSIC. }  
While \citet{gretton2005measuring} provided a direct interpretation of HSIC that models a single layer, we investigated deeper into HSIC's effect on each sample within a transition. This allows us to study and interpret how layer-wise sample behaviors contribute to achieve classification. Is there a general pattern that characterizes the layer-to-layer interaction? Or, are the results of each layer randomly jumping until a local minimum is reached? Unexpectedly, we discovered that each transition is optimizing different notions of affinity in IDS and RKHS. Namely, we present the following two properties with their proofs in App.~\ref{app:optimizing_IDS} and \ref{app:optimizing_RKHS}.

\begin{property}
The global optimum of Eq.~(\ref{eq:hsic_obj_pure}) is achieved in IDS
when sample pairs from the same and different classes are mapped into Euclidean distances of 0 and maximal distance.
\label{prop:pulling_samples_together}
\end{property}
\begin{property}
The global optimum of Eq.~(\ref{eq:hsic_obj_pure}) is achieved in RKHS when sample pairs from the same and different classes are mapped into angular distances of 0 and $\frac{\pi}{2}$.
\label{prop:align_samples_together}
\end{property}
Properties~\ref{prop:pulling_samples_together} and \ref{prop:align_samples_together} suggest that as the network cycle through its layers, the HSIC objective iteratively improves the \textit{affinity property} in both IDS and RKHS with different similarity measures. Although these properties are specific to the Gaussian kernel, the interpretation can be easily extended. In fact, as a corollary to  Theorem~\ref{thm:ccn_satisfies_dependence_property}, we can propose the following property.
\begin{property}
The kernel function chosen for Eq.~(\ref{eq:hsic_obj_pure}) directly induces $\kappa$ in the \textit{affinity objective}.
\label{prop:kernel_in_RKHS}
\end{property}
Since kernels define relationships between samples, it is not surprising in hindsight that they define the $\kappa$ in the \textit{affinity objective}. However, these properties jointly offer an interpretation on how samples behave at each transition. The network is using $\kappa$ to define different similarities in different spaces; it then then compresses similar data into $c$ discernible points with different notions of distance.

From a network-level's perspective, although there are many layers stacked together, the entire network can still be interpreted as having a single highly flexible layer. Therefore, the cyclic transitions of the network is a way of identifying the optimal feature map $f^*$ at the limit of the \textit{kernel sequence}. This observation begins to bridge the connection between MLPs and the kernel discovery process: an important and under-explored topic proposed by \citet{belkin2003laplacian}. 



%\textbf{Relating HSIC Properties to Previous Work. } Interestingly, these three additional properties provide a consistent narrative supporting the experimental observations made by \citet{montavon2011kernel} as previously mentioned in the introduction. By applying Property~\ref{prop:align_samples_together}, we see that as $l$ increases in KNet, each $f_{l^\circ}$ maps the original data into orientations that are increasingly aligned or orthogonal, thereby compressing the data into fewer and fewer eigenvectors. Consequently, fewer dominant eigenvectors are required to minimize LSE as more layers are added to the network. Our finding on HSIC's ability to compress the data is also consistent with the observations made by \citet{ma2019hsic} where they related HSIC to Information Bottlenecks. Although this interesting connection is trivial to demonstrate, 
%a brief proof and further discussions are provided in App.~\ref{app:theorem_information_bottleneck}.




%\section{Design and Solving a HSIC based MLP}
\section{MLP Optimization with HSIC}

\textbf{ISM Algorithm. } 
Although ISM was originally proposed to solve Kernel Dimension Reduction problem \cite{wu2019solving}, it also perfectly models MLP layers. Besides the theoretical advantages of ISM, it is a fast algorithm that can be easily implemented. Based on ISM, there exists a family of kernels where each kernel is associated with its own $\Phi$ matrix. Once $\Phi$ is calculated, the solution of Eq.~(\ref{eq:hsic_obj_pure}) is simply its $q$ most dominant eigenvectors. For completeness, we include the equation for the Gaussian $\Phi$ matrix along with the ISM algorithm in App.~\ref{app:ISM Algorithm}: the theoretical guarantees can be found in the original work by \citet{wu2018iterative,wu2019solving}.

\textbf{Advantages of Using ISM. } By combining the \textit{KNet Properties} with ISM, MLPs can be solved without backpropagation, thereby avoiding the issues of vanishing/exploding gradients. Additionally, since ISM guarantees both the 1st and 2nd order conditions, saddle points can be avoided while ensuring the optimality of every element within the \textit{risk sequence}. Moreover, ISM has a closed-form solution to initialize the network weights, thereby removing the need to initialize the network via random values. Even the width and depth of the network can be automatically determined via ISM. Note that the width of the network is determined by the dimension of $W_l$. Since ISM is a spectral method, 
the dimension of $W_l$ can be guided by $\Phi$'s rank, i.e., the width at each layer can be dynamically determined by maintaining $\Phi$'s most dominant eigenvalues. As for the depth of the network, it is simply the length of the \textit{kernel sequence}.


\textbf{Solving MLP via ISM. } 
By using ISM to obtain $W_l$ at each layer for KNet, the width of the network can be determined by the rank of $\Phi$. Once $W_l$ is obtained, the layer can be simulated via $R_l = \Psi(R_{l-1}W_l)$. Of course, since the feature map, $\Psi$, of a Gaussian kernel has infinite dimensions, we use a low dimensional approximation of $\Psi$ via the Random Fourier Feature (RFF) \cite{rahimi2008random}. Hence, the output of RFF becomes the output of the layer; which is again fed into the next layer. This process is repeated until the \textit{affinity objective} meets a predefined threshold. For reasons we will clarify in a later section, the Silhouette Score $\tilde{S}$ \cite{rousseeuw1987silhouettes} is used as a surrogate to evaluate the \textit{affinity objective} in IDS. After training the model, the resulting cluster centers of each class can be used to label the test samples by matching them to the nearest center. The KNet algorithm is summarized in Algorithm 1.

%\begin{algorithm}[H]
%\footnotesize
% \textbf{Input :} Data $X$, Label $Y$\\ 
% \textbf{Output :} Network weights $W_1, ..., W_L$ \\
% \While{ $\tilde{S}$ < 0.95 }{
%    Use the output of last layer as input\\
%    Add a new layer \\
%    Solve $W_l$ via ISM
% }
% \caption{KNet Algorithm}
% \label{alg:MLP_via_ISM}
%\end{algorithm}    

